Natural orbitals for the no-core configuration interaction approach

Ab initio calculations face the challenge of describing a complex multiscale quantum many-body system. The nuclear wave function has both strong short-range correlations and long-range contributions. Natural orbitals provide a means of adapting the single-particle basis for ab initio no-core configuration interaction (NCCI) calculations to better match the many-body wave function. Natural orbitals are obtained by diagonalizing the one-body density matrix from a calculation using an initial single-particle reference basis, such as the traditional harmonic oscillator basis. The natural orbital basis builds in contributions from high-lying oscillator shells, thus accelerating convergence of wave functions, energies, and other observables. The convergence of the ground and excited state energies, radii, and electromagnetic observables of He, Li, and Be isotopes calculated using natural orbitals in ab initio NCCI calculations is discussed. It is found that electromagnetic observables involving the M1 operator fully converge, while the calculated energies, radii, and observables involving the E2 operator converge significantly faster with the natural orbital basis than with the harmonic oscillator basis. The use of infrared (IR) extrapolation schemes with the natural orbital calculations is also explored.

==> chapters/chapter2/chapter2_draft_170129.tex <==
\chapter{INTRODUCTION TO THE NO-CORE CONFIGURATION INTERACTION APPROACH}
\label{chap-chap2}


\section{Overview}
\label{sec-chap2-overview}


In this chapter a broad overview of quantum many-body theory is presented focusing on the tools necessary to work with the no-core configuration interaction (NCCI) approach. The NCCI approach utilizes second quantization to cast the nuclear Hamiltonian into a square matrix in terms of a many-body basis. Here we describe all the steps needed to build and diagonalize the Hamiltonian matrix in some detail. Moreover, example calculations are presented and extrapolated using the infrared extrapolation method.


The general nuclear Hamiltonian for a system of $A$ nucleons interacting via two and/or three-body interactions $V(\mathbf{r}_{i},\mathbf{r}_{j})$ and $V(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k})$ respectively is given by
\begin{equation}
H = \frac{1}{2m_{\mathrm{N}}} \sum\limits_{i = 1}^{A} p_{i}^{2} + \sum_{i \neq j}^{A} V(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i \neq j \neq k}^{A} V_{\mathrm{NNN}}(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k}).
\label{eqn-chap2-overview-full-hamiltonian}
\end{equation}
Although three nucleon interactions are needed to accurately reproduce experimental data~\citep{pieperqmc:2008}, two-body interactions  provide a simpler context in which to focus on the main goal of this thesis, which is to introduce an alternative single-particle basis (other than the traditional harmonic oscillator basis) for NCCI calculations. Thus for the purpose of this thesis, we omit three-body terms from the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}).


Moreover, for reasons that have to do with the center-of-mass degree of freedom (described in Sec.~\ref{sec-chap2-com-factorization}) in the NCCI approach we do not work with the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}). Instead, we work with the translationally invariant intrinsic Hamiltonian \citep{vanhees:1983,lipkin:1958}
\begin{equation}
H_{\mathrm{in}} = T_{\mathrm{rel}} + V = \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}} 
+ \sum_{i \neq j}^{A} V_{\mathrm{NN}}(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i \neq j}^{Z} V_{\mathrm{C}}(\mathbf{r}_{i},\mathbf{r}_{j}) ,
\label{eqn-chap2-overview-hamiltonian}
\end{equation}
where $m_{\mathrm{N}} c^{2} = 938.92$ MeV is the average nucleon mass, $V_{\mathrm{NN}}$ is the internucleon interaction, and $V_{\mathrm{C}}$ is the Coulomb interaction. 


We start with a brief summary of second quantization (Sec.~\ref{sec-chap2-second-quantization}) and use it to derive the two-body matrix elements of the NCCI Hamiltonian (Sec.~\ref{sec-chap2-tbme}). Consequently, we discuss the harmonic oscillator single-particle radial functions (Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}) and the nuclear many-body basis (Sec.~\ref{sec-chap2-many-body-basis}). The complete factorization of the center-of-mass and intrinsic portions of the many-body wave function (Sec.~\ref{sec-chap2-com-factorization}) and a description of the procedure followed to perform many-body calculations using the NCCI approach (Sec.~\ref{sec-chap2-many-body-calculations}) are then discussed. The one-body density matrix and its properties are reviewed (Sec.~\ref{sec-chap2-one-body-density-matrix}). Example calculations for the nuclei $\isotope[3]{He}$ and $\isotope[4]{He}$ are presented and the calculated results are extrapolated using the infrared extrapolation method (Sec.~\ref{sec-chap2-example-calculations}). We conclude this Chapter with an overview of the steps needed to perform an NCCI calculation using a general single-particle basis (Sec.~\ref{sec-chap2-general-basis}).


\section{Second quantization}
\label{sec-chap2-second-quantization}


Second quantization is used to describe systems of many identical particles. In what follows the notational conventions of Negele are used~\cite{negele1988:many-particle}.


The Hilbert space of $A$ distinguishable particles $ \mathcal{H}^{A}$ is spanned by the tensor product of $A$ distinguishable particles occupying single-particle states which belong to the single-particle Hilbert space $\mathcal{H}$ 
\begin{equation}
\mathcal{H}^{A} = \mathcal{H} \otimes \mathcal{H} \otimes \ldots \otimes \mathcal{H}.
\label{eqn-chap2-hilbert-space-product}
\end{equation}
If $\left\{ | a \rangle \right\}$ is an orthonormal basis for $\mathcal{H}$, an orthonormal basis for $\mathcal{H}^{A}$ can be constructed as the set of tensor product states
\begin{equation}
| a_{1} \ldots a_{A} ) \equiv |a_{1} \rangle \otimes |a_{2} \rangle \otimes \ldots \otimes |a_{A} \rangle,
\label{eqn-chap2-many-body-basis-product}
\end{equation}
where the curved parenthesis on the left hand side of (\ref{eqn-chap2-many-body-basis-product}) denotes that the many-body state is a simple product of single-particle states (i.e., no assumptions are made about the symmetry of the many-body state). 


The space of $A$ indistinguishable fermions $\mathcal{F}^{A}$ is spanned by fully antisymmetric many-body states constructed using the many-body states of $\mathcal{H}^{A}$  
\begin{equation}
| a_{1} \ldots a_{A} \rangle = \frac{1}{\sqrt{A!}} \sum_{P} (-1)^{P} | a_{P_{1}} \rangle \otimes | a_{P_{2}} \rangle \otimes \ldots \otimes | a_{P_{A}} \rangle.
\label{eqn-chap2-many-body-basis-antisymmetric}
\end{equation} 
The sum over $P$ is a sum over all possible permutations $(P_{1},\,P_{2},\ldots,P_{A})$ of the set $(a_{1},\,a_{2},\,\ldots, a_{A})$. Moreover, $(-1)^{P}$ is determined by counting the number of transpositions of two elements which brings a permutation to its original form $(a_{1},\,a_{2},\,\ldots, a_{A})$. 


The Fock space $F$ for fermions is the (Hilbert) direct sum of the fermion spaces $\mathcal{F}^{0}$, $\mathcal{F}^{1}$, $\mathcal{F}^{2}$, $\ldots$, $\mathcal{F}^{A}$, $\ldots$ for zero, one, two, etc particles
\begin{equation}
F = \mathcal{F}^{0} \oplus \mathcal{F}^{1} \oplus \mathcal{F}^{2} \oplus \ldots \oplus \mathcal{F}^{A} \oplus \ldots.
\label{eqn-chap2-fock-space}
\end{equation}
Here $\mathcal{F}^{0}$ is the space of no particles, $\mathcal{F}^{1}$ is identical to $\mathcal{H}$, and $\mathcal{F}^{A}$ with $A \geq 2$ is the space spanned by many-body states as given by (\ref{eqn-chap2-many-body-basis-antisymmetric}).


Creation and annihilation operators generate the entire Fock space $F$ by adding (removing) single-particle states to (from) many-body states. The fermionic creation operator $c_{a}^{\dagger}$ adds a particle in a single-particle state $| a \rangle$ to the many-body state $| a_{1} \ldots a_{A} \rangle$ as follows
\begin{equation}
c_{a}^{\dagger} | a_{1} a_{2} \ldots a_{A} \rangle = | a a_{1} a_{2} \ldots a_{A} \rangle,
\label{eqn-chap2-creation-operator}
\end{equation}
where the definition implies that the particle is added to the left of the initial many-body state. Now because of the antisymmetry requirement for fermions, we cannot act with the $c_{a}^{\dagger}$ operator on the state $| a a_{1} a_{2} \ldots a_{A} \rangle$ (and thus add the single-particle state $| a \rangle$ twice). This state is equal to zero by definition
\begin{equation}
c_{a}^{\dagger} |a a_{1} a_{2} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-creation-operator-2}
\end{equation}
Similarly an annihilation operator $c_{a}$ removes a particle occupying the single-particle state $|a\rangle$ from a many-body state
\begin{equation}
c_{a} |a a_{1} \ldots a_{A} \rangle = | a_{1} \ldots a_{A} \rangle.
\label{eqn-chap2-annihilation-operator}
\end{equation}
For completeness, note that in general $c_{a} | a_{1} a_{2} \ldots a \ldots a_{A} \rangle = (-1)^{P} | a_{1} a_{2} \ldots a_{A} \rangle$ where $P$ is the number of transpositions of two elements needed to bring the particle in the single-particle state $| a \rangle$ to the front of the many-body state. For example $c_{a_{2}} | a_{1} a_{2} a_{3} \rangle = - |a_{1} a_{3} \rangle$. If $c_{a}$ acts on a state $| a_{1} \ldots a_{A} \rangle$, i.e., a state which has no particle in the single-particle state $| a \rangle$, then the action of $c_{a}$ on the many-body state $| a_{1} \ldots a_{A} \rangle$ yields zero
\begin{equation}
c_{a} |a_{1} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-annihilation-operator-2}
\end{equation}
Following from~(\ref{eqn-chap2-creation-operator})~(\ref{eqn-chap2-annihilation-operator-2}), we conclude that the creation and annihilation operators obey the fermionic anticommutation relation
\begin{equation}
\lbrace c_{a} , c_{b} \rbrace = \delta_{ab}.
\label{eqn-chap2-anti-commutation}
\end{equation}


%Using creation and annihilation operators we can define the number operator 
%\begin{equation}
%\hat{N} = \sum_{a} c_{a}^{\dagger} c_{a},
%\label{eqn-chap2-number-operator}
%\end{equation}
%which counts the total number of particles in a many-body state
%\begin{equation}
%\hat{N} | a_{1} \ldots a_{A} \rangle = A | a_{1} \ldots a_{A} \rangle.
%\label{eqn-chap2-number-operator-2}
%\end{equation}
%The sum in \ref{eqn-chap2-number-operator} is over all single-particle states in the basis $\left\{ | a \rangle \right\}$.


One-body operators are operators which can be written as a sum of single-particle operators acting on one particle at a time. To be able to calculate the matrix elements of one-body operators with respect to many body states like (\ref{eqn-chap2-many-body-basis-antisymmetric}), it is useful to express one-body operators in terms of creation and annihilation operators. To arrive to this expression, let us first use the many-body states of $\mathcal{H}^{A}$ to calculate the matrix elements of a one-body operator $T = \sum_{i=1}^{A} t_{i}$. For the diagonal matrix elements (i.e., between the same many-body states) we have
\begin{multline}
( a_{1}a_{2} \ldots a_{A} | T | a_{1} a_{2} \ldots a_{A} ) = \\  
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2} \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \\
\langle a_{1} | t_{1} | a_{1} \rangle + \ldots + \langle a_{A} | t_{A} | a_{A} \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-identical-states}
\end{multline}
where we used the fact that the single-particle states are orthonormal hence $\langle a_{i} | a_{j} \rangle = \delta_{ij}$. Let us now evaluate the non-diagonal matrix elements of $T$ starting with the matrix elements between the many-body state $ | a_{1} a_{2} \ldots a_{A} )$ and the many-body state $ | a_{1} a_{2}' \ldots a_{A} )$, where $| a_{2} \rangle \neq | a_{2}' \rangle$. We have
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1} a_{2}' \ldots a_{A} ) = \langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \langle a_{1} | a_{1} \rangle \langle a_{2} | t_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle  = \langle a_{2} | t_{2} | a_{2}' \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-one-sp-state-different}
\end{multline}
since $\langle a_{2} | a_{2}' \rangle = 0 $. Finally, the matrix elements of $T$ between the many-body states $| a_{1} a_{2} \ldots a_{A} )$ and $| a_{1}' a_{2}' \ldots a_{A} )$, where $| a_{1} \rangle \neq | a_{1}' \rangle$ and $| a_{2} \rangle \neq | a_{2}' \rangle$, are
\begin{equation}
( a_{1} a_{2} \ldots a_{A} | T | a_{1}' a_{2}' \ldots a_{A} ) = \langle a_{1} | t_{1} | a_{1}' \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1}' \rangle \ldots \langle a_{A} | t_{A} | a_{A} \rangle = 0.
\label{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}
\end{equation}
Thus, the matrix elements of the one-body operator $T$ with respect to many-body states of $\mathcal{H}^{A}$ are fully defined by the sum of single-particle matrix elements of $\mathcal{H}$. If we now define the single-particle vacuum state $| - \rangle$ (i.e., a non-occupied single-particle state), then $c_{a}^{\dagger} | - \rangle = | a \rangle$. Using this definition and (\ref{eqn-chap2-one-body-operator-matrix-elements-identical-states})-(\ref{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}) we can write the one-body operator as
\begin{equation}
T = \sum_{ab} t_{ab} c_{a}^{\dagger} c_{b},
\label{eqn-chap2-one-body-operator-second-quantization}
\end{equation}
where $t_{ab} = \langle a | t | b \rangle$.

Similarly, the matrix elements of a two-body operator $V = \frac{1}{2} \sum_{i \neq j} u_{ij}$ with respect to the many-body states of $ \mathcal{H}^{A}$ are fully defined by the matrix elements $u_{abcd} = (ab | u | cd )$ calculated using the states of $\mathcal{H}^{2}$. Thus we can write $V$ as
\begin{equation}
V = \frac{1}{2} \sum_{abcd} u_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c}.
\label{eqn-chap2-interaction-second-quantized}
\end{equation}
However, it is more convenient to write the two-body operator as
\begin{equation}
V = \frac{1}{4} \sum_{abcd} \bar{u}_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c},
\label{eqn-chap2-interaction-second-quantized-antisymmetrized}
\end{equation}
where $\bar{u}_{abcd} = u_{abcd} - u_{abdc} = \langle ab | u | cd \rangle$ are normalized and antisymmetrized two-body matrix elements.


\section{Two-body matrix elements for the NCCI Hamiltonian}
\label{sec-chap2-tbme}

In the context of the NCCI approach, the most commonly used single-particle states are the harmonic oscillator single-particle basis states (which are reviewed in Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}). A harmonic oscillator single-particle state is labeled by the quantum numbers $| \alpha \rangle \equiv |n_{a}l_{a}j_{a}m_{a} \rangle$, where $n_{a}$ is the harmonic oscillator radial quantum number, $l_{a}$ is the angular momentum, $j_{a}$ is the total angular momentum, and $m_{a}$ is the $z$ projection of the total angular momentum. Using the harmonic oscillator single-particle states we can construct fully antisymmetric many-body basis states for the NCCI approach
\begin{equation}
| (n_{a}l_{a}j_{a}m_{a}) (n_{b}l_{b}j_{b}m_{b}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle.
\label{eqn-chap2-many-body-state-harmonic-oscillator}
\end{equation} 
The many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) have a total $z$ projection of the total angular momentum $M=\sum_{i=1}^{A} m_{i}$ and a total number of oscillator quanta $N=\sum_{i=1}^{A} (2n_{i} + l_{i}) = \sum_{i=1}^{A} N_{i}$. The harmonic oscillator single-particle states $| \alpha \rangle$ are given by 
\begin{equation}
| \alpha \rangle = \left[| R_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}},
\label{eqn-oscillator-orbitals-second-quantization}
\end{equation}
where $R_{n_{a}l_{a}}$ is a harmonic oscillator radial function, $Y_{l_{a}}$ is a spherical harmonic, and $|\frac{1}{2} \rangle$ is a spinor. The subscripts $j_{a}$ and $m_{a}$ indicate that the spherical tensor $| R_{n_{a} l_{a}} Y_{l_{a}} \rangle$ of rank $l_{a}$ and the spinor $| \frac{1}{2} \rangle$ are coupled to total angular momentum $j_{a}$~\cite{rose1957:am}. 


The Hilbert space of the NCCI Hamiltonian is spanned by the many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) which provide a basis for the representation of the Hamiltonian as a square matrix. To cast the Hamiltonian into a square matrix we must first calculate the two-body matrix elements of the relative kinetic energy and two-body interaction operators. The two-body matrix elements are calculated with respect to two-particle states, coupled to total angular momentum $J$. For distinguishable particles (e.g., one proton and one neutron states), angular momentum two-particle states are defined as 
\begin{equation}
| a b ; J ) = \sum_{m_{a}m_{b}} \langle j_{a} m_{a} j_{b} m_{b} | J M \rangle |a m_{a} \rangle | b m_{b} \rangle,
\label{eqn-chap2-two-particle-states-1}
\end{equation}
where $| a m_{a} \rangle = | n_{a} l_{a} j_{a} m_{a} \rangle$, $\langle j_{a} m_{a} j_{b} m_{b} | J M \rangle $ is a Clebsch-Gordan coefficient, and the parenthesis in implies that the two-particle state is not antisymmetrized. For two identical fermions we can obtain fully antisymmetrized states using the states $| a b ; J )$. We have
\begin{equation}
| a b ; J M \rangle_{\mathrm{AS}} = \frac{1}{\sqrt{2}} \left[ | a b ; J M ) - (-1)^{J - j_{a} - j_{b}} | b a ; J M \rangle \right].
\label{eqn-chap2-two-particle-states-2}
\end{equation}
These states have the symmetry property $| a b ; J M \rangle = - (-1)^{J -j_{a}-j_{b}} | b a ; J M \rangle$ which implies that if the states $| a \rangle$ and $| b \rangle$ are identical, then only two-body states with even $J$ are allowed. The states (\ref{eqn-chap2-two-particle-states-2}) are antisymmetrized but not strictly normalized. An extra factor of $1 / \sqrt{2}$ is required for normalization in the special case when the two particles occupy the same single-particle orbital $| n_{a} l_{a} j_{a} \rangle$. Hence, the appropriate two-particle states are
\begin{equation}
| a b ; J M \rangle_{\mathrm{NAS}} = (1 + \delta_{ab})^{-1/2} | a b ; J M \rangle_{\mathrm{AS}}.
\label{eqn-chap2-two-particle-states-3}
\end{equation}
Both the normalized antisymmetrized states and the antisymmetrized states are used to calculate the two-body matrix elements $\langle c d ; J | H_{\mathrm{in}} | a b ; J \rangle$ of the (scalar) intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}). The change of basis relation between two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-3}) and two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-2}) is
\begin{equation}
\langle c d ; J | H | a b ; J \rangle_{\mathrm{NAS}} = (1+\delta_{cd})^{-1/2} (1+\delta_{ab})^{-1/2} \langle c d ; J | H | a b ; J \rangle_{\mathrm{AS}}.
\label{eqn-chap2-nas-two-body-matrix-elements}
\end{equation}
A detailed discussion about the calculation of the two-body matrix elements of the intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) is given in Ref.~\cite{caprio2012:csbasis}. A brief overview is also given in Sec.~\ref{sec-chap2-general-basis}.
 

\section{The harmonic oscillator single-particle states}
\label{sec-chap2-harmonic-oscillator-radial-functions}


In this section we will review the basic properties of the harmonic oscillator single-particle states $| \alpha \rangle$ which are traditionally used in the NCCI approach~\cite{suhonen2007:nucleons-nucleus,moshinsky1996:oscillator,weniger1985:fourier-plane-wave} because their properties facilitate the many-body calculations. The harmonic oscillator single-particle states are also our starting basis for the construction of natural orbitals which are introduced in Chapter~\ref{chap-chap3}. 


The first important property of the harmonic oscillator single-particle basis is that it allows for the removal of spurious center-of-mass states from the low-lying spectrum of the NCCI Hamiltonian provided that an $\Nmax$ truncation is imposed on the many-body basis. The appearance of spurious center-of-mass states results from using the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) for the representation of the NCCI Hamiltonian as a square matrix. A detailed explanation of spurious center-of-mass states and the procedure followed for their removal from the low-lying spectrum is given in Sec.~\ref{sec-chap2-many-body-basis}.

The second important property of the harmonic oscillator single-particle states is that they simplify the calculation of two-body matrix elements for operators written in terms of relative coordinates using the Moshinsky transformation~\citep{moshinsky1996:oscillator}. According to  the transformation, products of harmonic oscillator states expressed in single-particle coordinates $R_{n_{1}l_{1}}(\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ transform into products of harmonic oscillator states expressed in terms of relative and center-of mass coordinates $R_{nl}(\mathbf{r}_{\mathrm{rel}})R_{NL}(\mathbf{R})$, where $2 n_{1} + l_{1} + 2 n_{2} + l_{2}= 2 n + l+ 2 N + L$, $\mathbf{r}_{\mathrm{rel}} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}-\mathbf{r}_{2})$, and $\mathbf{R} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}+\mathbf{r}_{2})$. (The factor of $1/\sqrt{2}$ in front of the center-of-mass vector is used instead of the traditional $1/2$ for normalization reasons). The calculation of two-body matrix elements for operators of the form $V(r_{1}-r_{2})$ with respect to two-particle states of the form $R_{n_{1}l_{1}} (\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ is then reduced to the calculation of the single-particle matrix element of the operator $V(\mathbf{r}_{\mathrm{rel}})$ with respect to single-particle states of the form $R_{nl}(\mathbf{r}_{\mathrm{rel}})$ and an overlap between single-particle states of the form $R_{NL}(\mathbf{R})$.

Let us now derive the harmonic oscillator radial wave functions. If we write $\Psi_{nlm}(\mathbf{r})=r^{-1} R_{nl}(b;r)Y_{lm}(\theta,\phi)$, where $R_{nl}(b;r)$ are radial functions and $Y_{lm}(\theta,\phi)$ are spherical harmonics, the harmonic oscillator wave functions are solutions to the familiar harmonic oscillator central force problem \cite{suhonen2007:nucleons-nucleus} 
\begin{equation}
h(\omega) = \frac{p^{2}}{2m_{\mathrm{N}}} + \frac{m_{\mathrm{N}} \omega^{2} r^{2}}{2}.
\label{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}
\end{equation} 
where $m_{\mathrm{N}}c^{2} \approx 938.92$ MeV is the average nucleon mass and $\omega$ is the oscillator frequency. The length scale of the radial functions $R_{nl}(b;r)$ is set by the oscillator length $b$ which depends on the parameters of the oscillator Hamiltonian (\ref{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}) as $b=\sqrt{\hbar / (m_{\mathrm{N}} \omega})$. The eigenvalues corresponding to the radial wave functions are given by $ (N + 3/2) \hw$, where $N = 2n + l$ is the oscillator quantum giving the number of oscillator quanta in an oscillator wave function. (Notice that the eigenvalues are evenly spaced by one unit of $\hw$). The radial functions $R_{nl}(b;r)$ are given by
\begin{equation}
R_{nl}(b;r) = b N_{nl} (r/b)^{l+1} L_{n}^{l+1/2}[(r/b)^{2}] e^{-(r/b)^{2}/2},
\label{eqn-chap2-harmonic-oscillator-radial-functions}
\end{equation} 
where $L_{n}^{l+1/2}[(r/b)^{2}]$ are generalized Laguerre polynomials, $n$ is the principal quantum number (which gives the number of nodes of the radial function), $l$ is the angular momentum, and $N_{nl}$ is a normalization factor given by
\begin{equation}
N_{nl} = \frac{1}{b^{3/2}} \left[ \frac{2n!}{(l+n+1/2)!} \right]^{1/2}.
\label{eqn-chap2-harmonic-oscillator-functions-normalization}
\end{equation}
For each $l$, the harmonic oscillator radial functions form a complete discrete basis for square integrable functions on $ \mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} R_{nl}(b;r) R_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-ho-orthonormal}
\end{equation}
 

\section{Symmetries of the NCCI Hamiltonian and the nuclear \\ many-body basis}
\label{sec-chap2-many-body-basis}


The selection of the nuclear many-body basis used in NCCI calculations is based on the symmetries of the NCCI Hamiltonian~(\ref{eqn-chap2-overview-hamiltonian}). The NCCI Hamiltonian is rotationally invariant, therefore it conserves the total angular momentum $J$ and the $z$ projection of total angular momentum $M$. Moreover, the Hamiltonian conserves parity. To diagonalize the Hamiltonian we can choose to use many-body states that have good $J$ (a $J$-scheme basis) or many-body states that have good $M$ (an $M$-scheme basis)~\cite{whitehead1977:shell-methods}. Although the $M$-scheme basis involves a larger number of many-body basis states compared to a $J$-scheme basis, constructing $M$-scheme many-body basis states is straightforward (i.e., we do not have to deal with angular momentum coupling as in the $J$-scheme basis). Therefore, for the NCCI calculations discussed here, an $M$-scheme basis is considered. However, the eigenstates of $H$ still have good $J$ which is recovered after diagonalization by calculating the expectation value of the $J^{2}$ operator with respect to the calculated many-body wave function.


To build many-body basis states we start from single-particle states $nljm$ and construct fully antisymmetric states (with good $M$) given by~(\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Calculations can be performed for any possible value of $M$ (which is supported by the single-particle states in the many-body basis). For example, for even nuclei $M=0, 1,\ldots$ and for odd nuclei $M=1/2, 3/2, \ldots$. However we usually use many-body states with $M=0$ for even nuclei and $M=1/2$ for odd nuclei. This is because for a given $M$ we can only obtain many-body wave functions with $J \geq M$. Thus, choosing the lowest possible $M$ allows us to study the ground and first few excited levels of a nucleus.


Commonly, for reasons involving the center-of-mass degree of freedom, as discussed below, the many-body basis is truncated using the $\Nmax$ truncation scheme~\cite{elliott1955:com-shell}. The scheme dictates that only many-body states with $\Ntot \leq N_{0} + \Nmax$ are permitted in the many-body basis, where $N_{0}$ is the number of quanta in the configuration where all the nucleons occupy the lowest permitted oscillator shells. For example, $N_{0}=2$ for $\isotope[6]{He}$ (in this configuration, the two protons occupy the $N=0$ proton shell, two neutrons occupy the $N=0$ neutron shell, and the last two neutrons occupy the $N=1$ shell) and $N_{0} =3$ for $\isotope[7]{Li}$ (because the extra proton compared to $\isotope[6]{He}$ goes into the $N=1$ proton shell). 


Finally, because the nuclear Hamiltonian conserves parity we want our many-body states to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. This means that the parity of a many-body state is obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the lowest possible configuration is given by $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity states of the nucleus $\Nmax$ must be even and proceed in steps of $2$, i.e., $\Nmax = 2, 4, 6, \ldots$. On the other hand, to obtain the unnatural parity states of the nucleus $\Nmax$ must be odd and also proceed in steps of $2$, i.e., $\Nmax = 1, 3, 5, \ldots$. 






\section{Spurious center-of-mass states removal}
\label{sec-chap2-com-factorization}


In this section we describe how spurious center-of-mass states result from the diagonalization of the NCCI Hamiltonian matrix built in terms of the set of the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Subsequently, we describe how these spurious states can be removed provided that the $\Nmax$ truncation scheme is used.

The many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) are defined with respect to a fixed point in space. However, physically there is no such point around which all the nucleons are orbiting. Rather we are interested in the internal motion of the nucleons relative to each other within the nucleus, a motion which defines the intrinsic structure of the nucleus.


In principle we can convert to relative coordinates. However, antisymmetrization in Jacobi coordinates (which define the relative motion) is cumbersome. Therefore, we are compelled to work in the full coordinate space which includes both the center of mass and relative degrees of freedom.


Our goal is to describe the relative motion as accurately as possible without unnecessary complications arising from the center of mass motion. In order to accomplish this it helps making certain choices regarding the basis and the Hamiltonian.


We want our eigenfunctions to factorize into center of mass and relative factors. We also want the center of mass factor to be simple and well understood so that it does not interfere with the calculation of energies and observables. In principle, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) is already separated into center of mass and relative coordinates. If we define the center-of-mass momentum as $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, the one-body kinetic energy operator in (\ref{eqn-chap2-overview-full-hamiltonian}) can be decomposed into a center-of-mass and a relative kinetic energy contributions~\cite{vanhees:1983}
\begin{equation}
T = T_{\mathrm{c.m.}} + T_{\mathrm{rel}} = \frac{1}{2Am_{\mathrm{N}}} \left(\sum\limits_{i=1}^{A}\mathbf{p}_{i}\right)^{2} + \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}}.
\label{eqn-chap2-kinetic-energy-decomposition}
\end{equation}
Therefore, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) also separates into center-of-mass and relative parts
\begin{equation}
H= T_{\mathrm{c.m.}} + T_{\mathrm{rel}} + V.
\label{eqn-chap2-full-separated-hamiltonian}
\end{equation}
Thus, in the full space our eigenfunctions would factorize into a center-of-mass and a relative wave function.

However, we are confined to work in a truncated space. Factorization can still be exact in an oscillator basis when the $\Nmax$ truncation is used. The truncated space then only contains a limited center-of-mass space spanned by center-of-mass harmonic oscillator states with $N_{\mathrm{c.m.}} = 0$, $2$, $\ldots, \Nmax$. We could attempt to diagonalize the Hamiltonian~(\ref{eqn-chap2-overview-full-hamiltonian}) in the truncated space. However, the $T_{\mathrm{c.m.}}$ operator in (\ref{eqn-chap2-full-separated-hamiltonian}) will mix contributions with different center-of-mass excitations $N_{\mathrm{c.m.}}$ and destroy factorization of the eigenfunctions. The Hamiltonian will force us towards states which attempt to diagonalize the center-of-mass kinetic energy operator $T_{\mathrm{c.m.}}$. Therefore, our NCCI calculations would end up approximating spherical waves in the center of mass coordinates, at the expense of accurately describing the intrinsic motion.

Thus, instead, we choose to work with the intrinsic Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V.
\end{equation} 
The resulting Hamiltonian is block diagonal with respect to the number of quanta $N_{\mathrm{c.m.}}$ for the center-of-mass motion. The resulting eigenfunctions will factorize into a center-of-mass factor of good $N_{\mathrm{c.m.}}$ and an intrinsic factor. The total number of quanta in a many-body state is shared between the center-of-mass motion and the intrinsic motion:
\begin{equation}
\Ntot = \sum_{i} N_{i} = N_{\mathrm{c.m.}} + N_{\mathrm{rel}}.
\label{eqn-chap2-number-of-quanta-com-quanta}
\end{equation}
Therefore, in eigenfunctions with $N_{\mathrm{c.m.}} = 0$, the full $\Nmax$ quanta are available to use in describing the intrinsic motion. The higher $N_{\mathrm{c.m.}}$ eigenfunctions produce spurious copies of the spectrum in which the intrinsic motion is described using fewer quanta $N_{\mathrm{rel}} \leq \Nmax - N_{\mathrm{c.m.}}$. 


It is convenient to push the spurious excited center-of-mass states out of the low lying spectrum. We do this by adding a term diagonal in the number of center-of-mass quanta. That is we add a ``Lawson term''~\cite{gloeckner1974:spurious-com} proportional to the $N_{\mathrm{c.m.}}$ operator. This is often equivalently described as adding a center-of-mass harmonic oscillator Hamiltonian. In terms of the center-of-mass coordinate $\mathbf{R} = (\sum_{i} \mathbf{r}_{i})/A$ and the center-of-mass momentum $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, 
\begin{equation}
H_{\mathrm{c.m.}} = \frac{P^{2}}{2Am_{\mathrm{N}}} + \frac{1}{2} A m_{\mathrm{N}} \omega^{2} R^{2}.
\label{eqn-chap2-harmonic-oscillator-many-body-hamiltonian-com}
\end{equation}
Then, $H_{\mathrm{c.m.}} = (N_{\mathrm{c.m.}} + 3/2)\hbar \omega$. Thus we actually diagonalize the Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V + \alpha N_{\mathrm{c.m.}},
\end{equation} 
where $\alpha$ is the Lawson term strength (typically a few MeV). This leads to the same eigenstates as the relative Hamiltonian but with the spurious states lifted out of the low-lying spectrum by an amount of $\alpha N_{\mathrm{c.m.}}$.




\section{Many-body calculations}
\label{sec-chap2-many-body-calculations}


In this section we will briefly describe the general procedure followed to obtain results using the NCCI approach.

The basic ingredient needed to build the Hamiltonian matrix are the matrix elements of the NCCI Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) with respect to many-body basis states like (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Thus, we need to evaluate matrix elements of the form
\begin{equation}
\langle \Phi_{n} | H | \Phi_{m} \rangle,
\label{eqn-chap2-two-body-matrix-elements}
\end{equation}
where $| \Phi_{n} \rangle = | (n_{1}l_{1}j_{1}m_{1}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle$ is a many-body basis state. [The matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) reduce to a sum over two-body matrix elements of the form $\langle c d ; J | H | a b ; J \rangle$ using Wick's theorem]. After calculating the matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) for all the many-body states in our basis we obtain the Hamiltonian matrix
\begin{equation}
  \begin{pmatrix}
    \langle \Phi_{1} | H | \Phi_{1} \rangle & \langle \Phi_{1} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{1} | H | \Phi_{m} \rangle \\
    \langle \Phi_{2} | H | \Phi_{1} \rangle & \langle \Phi_{2} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{2} | H | \Phi_{m} \rangle \\
    \vdots & \vdots & \ddots & \vdots \\
   \langle \Phi_{m} | H | \Phi_{1} \rangle & \langle \Phi_{m} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{m} | H | \Phi_{m} \rangle
  \end{pmatrix}
\label{eqn-chap2-ncci-hamiltonian-matrix}
\end{equation}
The dimension $d$ of the matrix (\ref{eqn-chap2-ncci-hamiltonian-matrix}) is equal to the number of many-body basis states for a given nucleus and $\Nmax$ truncation (see Fig.~\ref{fig-chap1-NNCI-dimension}). Diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}) yields the nuclear many-body wave functions  
\begin{equation}
| \Psi \rangle = \sum\limits_{n=1}^{d} c_{n} | \Phi_{n} \rangle,
\label{eqn-chap2-ncci-wave-functions}
\end{equation}
where $c_{n}$ are coefficients obtained from the diagonalization of (\ref{eqn-chap2-ncci-wave-functions}).


The diagonalization of the Hamiltonian matrix is performed using the Lanczos algorithm~\cite{komzsik2003:lanczos-method,lanczos1950:algorithm}. The algorithm transforms the generally large sparse matrix (\ref{eqn-chap2-ncci-wave-functions}) into a tridiagonal matrix (of lower dimension than the original matrix). The tridiagonal matrix is then diagonalized (using an appropriate algorithm) and the eigenvalues and eigenvectors are obtained. The eigenvectors of the tridiagonal matrix (Lanczos vectors) must then be converted from the Lanczos vector space to the original basis. The process established by Lanczos proceeds as follows: If $H$ is a Hamiltonian matrix of order $n$ (i.e., the matrix dimension is $n \times n$), then the process starts with a random initial vector $b_{0}$ which is used to construct $m$ vectors (orthogonal to each other) according to the algorithm
\begin{align}
b_{0} = \mathrm{random}, \nonumber \\
b_{1} = (H - \alpha_{0}) b_{0}, \nonumber \\
b_{2} = (H - \alpha_{1}) b_{1} - \beta_{0} b_{0}, \nonumber \\
b_{3} = (H - \alpha_{2}) b_{2} -\beta_{1} b_{1}, \nonumber \\
\vdots \nonumber \\
b_{m} = (H - \alpha_{m-1}) b_{m-1} - \beta_{m-2} b_{m-2},
\label{eqn-chap2-lanczos-algorithm}
\end{align}
where $m \leq n$. The equality to zero in the last step means the end of the process. The coefficients $\alpha_{m-1}$ and $\beta_{m-2}$ are determined by requiring that the norm of the vector $\parallel b_{m} \parallel$ is minimized. The coefficients are used to build the tridiagonal matrix $T$. We have
\begin{equation}
T =  \begin{pmatrix}
\alpha_{0} & \beta_{0} &   &   & 0\\ 
\beta_{0}  & \alpha_{1} & \beta_{1} & \\
                 & \ddots & \ddots & \ddots & \\
                 &  & \beta_{k-2} & \alpha_{k-1} &\beta_{k-1} \\
           0      & & & \beta_{k-1} & \alpha_{k}
  \end{pmatrix}
\label{eqn-chap2-tridiagonal-matrix}
\end{equation}
The eigenvalues of $T$ converge to the first $k$ eigenvalues of $H$ provided that a sufficient number of iterations $k$, where $k < n$, is performed. 


The generally large sizes of the NCCI Hamiltonian matrices require the use of parallel computing to handle both the storage and the Lanczos diagonalization of the Hamiltonian matrix. The parallel code Many Fermion Dynamics (MFD) \cite{maris2010:ncsm-mfdn-iccs10,vary2009:ncsm-mfdn-scidac09} developed by the Iowa State University group handles the construction of the many-body basis, the construction of the Hamiltonian matrix, the storage of the matrix, and the Lanczos diagonalization of the matrix. The input to the code includes the two-body matrix elements of the Hamiltonian, the $\Nmax$ truncation of the many-body basis, the number of protons ($Z$) and neutrons ($N$) of the nucleus we want to study, the number of Lanczos iterations we want to perform, and various other control parameters. The program outputs multiple output files containing the eigenvalues (which are the nuclear level energies), the one-body density matrices (described in Sec.~\ref{sec-chap2-one-body-density-matrix}), and other observables.


\section{The one-body density matrix}
\label{sec-chap2-one-body-density-matrix}


The one-body density matrix is a fundamental tool in many-body calculations, used for the calculation of the matrix elements of one-body operators~\cite{suhonen2007:nucleons-nucleus}. In second quantization, the matrix elements of the transition one-body density matrix are given by
\begin{equation}
\rho_{\alpha\beta}^{\mathrm{f\,i}} = \langle \Psi_{\mathrm{i}} | c_{\alpha}^{\dagger} c_{\beta} | \Psi_{\mathrm{f}} \rangle,
\label{eqn-chap2-one-body-density-operator}
\end{equation}
where $| \Psi_{\mathrm{i}} \rangle$ and $| \Psi_{\mathrm{f}} \rangle$ are the many-body wave functions of some initial and final nuclear state respectively. Using (\ref{eqn-chap2-one-body-density-operator}) we can calculate the matrix elements of a one-body operator $\mathcal{O}$ as follows
\begin{equation}
\langle \Psi_{\mathrm{i}} | \mathcal{O} | \Psi_{\mathrm{f}} \rangle =  \sum_{\alpha\beta} \langle \alpha | \mathcal{O} | \beta \rangle \langle \Psi_{\mathrm{i}} | c_{\alpha}^{\dagger}c_{\beta} | \Psi_{\mathrm{f}} \rangle.
\label{eqn-chap2-one-body-operator-matrix-elements}
\end{equation}
Typically, the many-body wave functions $| \Psi_{i} \rangle$ and $| \Psi_{f} \rangle$ carry some quantum numbers related to the nuclear state such as the total angular momentum $J$, the $z$ projection of the total angular momentum $M$, the total isospin of the state, etc. For example, the NCCI wave function is given by $| \Psi \rangle = | J^{\pi} M T \rangle$, where $\pi$ is the parity of the nuclear state.


The static one-body density matrix (i.e., the one-body density matrix obtained for the same initial and final many-body wave functions) contains information about correlations in the many-body wave function. By definition, an uncorrelated many-body wave function contains a single Slater determinant (a single many-body basis state). For example, $| \Psi \rangle = | a_{1} \ldots a_{A} \rangle$ is an uncorrelated many-body wave function. In the case of $| \Psi \rangle$, it is easy to see that all the diagonal matrix elements $\rho_{\alpha\alpha} = \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle $ are equal to $1$ (which reflects the fact that each single-particle state is occupied by exactly one nucleon), while all the off diagonal matrix elements $\rho_{\alpha\beta}$ are equal to zero. The sum of the diagonal matrix elements is equal to the total number of nucleons $A$ in the many-body wave function. In the case of a highly correlated many-body wave function, such as the ones calculated in an NCCI calculation, the one-body density matrix is not (in general) diagonal. The off diagonal matrix elements $\rho_{\alpha\beta}$ of the density matrix provide a measure of how correlated the many-body wave function is, while the diagonal matrix elements $\rho_{\alpha\alpha}$ provide the occupancies of each single-particle state $| a_{i} \rangle$ in the many-body wave function. The sum over the diagonal matrix elements is still equal to the total number of nucleons in the many-body wave function
\begin{equation}
\sum_{\alpha} \langle \Psi_{\mathrm{i}} | c_{\alpha}^{\dagger} c_{\alpha} | \Psi_{i} \rangle = A.
\label{eqn-chap2-density-matrix-number}
\end{equation}
It is important to stress here that a diagonal one-body density matrix does not necessarily indicate that a many-body wave function is uncorrelated unless the diagonal matrix elements $\rho_{\alpha \alpha}$ are exactly equal to $1$. The one-body density matrix is our starting point for the construction of natural orbitals in Chapter~\ref{chap-chap3}.


\section{Example calculations and infrared extrapolations}
\label{sec-chap2-example-calculations}


In this section we perform NCCI calculations to obtain the ground state energy and point proton rms radius of the isotopes $\isotope[3,4]{He}$. Our goal is to revisit the convergence properties of NCCI calculations using the harmonic oscillator basis and to extrapolate the calculated results to the full $\Nmax \rightarrow \infty$ space using the infrared extrapolation method which we present and discuss here.


Full convergence of observables calculated using the harmonic oscillator basis in NCCI calculations is rare for most nuclei~\cite{maris2009:ncfc,maris2012:mfdn-ccp11,maris2013:ncsm-pshell}. Here we consider the calculated results for $\isotope[3,4]{He}$, obtained using the JISP$16$ interaction and the Coulomb interaction between protons, shown in Fig.~\ref{fig-chap2-helium3-helium4}. Calculations were performed for even $\Nmax$ truncations up to $\Nmax = 16$ (in steps of $2$ starting from $\Nmax = 4$) which scan the $\hw$ range $10$-$40$ MeV. The solid lines correspond to the calculated results, the dashed horizontal lines correspond to the experimental results~\cite{npa-purcell-a-3-data:2010,npa-tilley-a-4-data:1992}, and the data points shown with crosses connected with dotted lines correspond to the extrapolated results discussed below. As we observe, the calculated results for both the ground state energy and the proton radius of $\isotope[4]{He}$ converge. On the other hand, the calculated ground state energy of $\isotope[3]{He}$ converges only approximately (the difference between the calculated ground state energy at the variational minimum of the $\Nmax = 14$ and $\Nmax = 16$ curves is about $\sim 0.01$ MeV) while the point proton rms radius does not converge . 


Comparisons of NCCI calculations with experimental results are only meaningful once full convergence is achieved. However, when the calculated results do not converge one can attempt to extrapolate results obtained in truncated spaces to the full $\Nmax \rightarrow \infty$ space. One such example was presented in Chapter~\ref{chap-chap1} where we used an empirical extrapolation method to extrapolate the ground state energy of $\isotope[6]{He}$. Here, we use the infrared extrapolation method to obtain predictions for the ground state energy and rms radius in the full space, based on the effective cutoffs imposed on the many-body wave function by the truncated many-body basis.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{\plotspath /ho_no_comparison/Z2-N1-Z2-N2-rp-e-HO-thesis-chapter1-170111.pdf}
\caption[NCCI calculations for the ground state energy and proton rms radius of {\protect $\isotope[3,4]{He}$}. The calculated results are extrapolated using the infrared extrapolation method.]{Calculated ground state energy (left) and point proton rms radius in the ground state (right) for $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom), obtained for various $\Nmax$ truncations of the many-body basis shown next to each successive curve and for $\hw$ strengths scanning the range $10$-$40$ MeV. The dashed horizontal lines show the experimental results. The crosses connected by dotted lines are obtained by extrapolating calculated results using the infrared extrapolation method as described in the text.}
\label{fig-chap2-helium3-helium4}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The infrared extrapolation method~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation, more2013:ir-extrapolation,furnstahl2014:ir-expansion, furnstahl2015:ir-extrapolations,odell-papenbrock-ir-extrapolation-quadruple:2016} starts with the assumption that the truncated many-body basis  induces both a short-range ultraviolet (UV) and a long-range infrared (IR) cutoff on the ability of the many-body basis to describe the many-body wave function. Quantitatively, if the highest occupied single-particle orbital in the many-body basis has $N$ oscillator quanta, then to a first approximation the momentum space (UV) cutoff is
\begin{equation}
\Lambda_{\mathrm{UV}} = \sqrt{2(N+3/2)} \,\, \hbar/b,
\label{eqn-chap2-uv-cutoff}
\end{equation}
and the coordinate space (IR) cutoff is
\begin{equation}
L = \sqrt{2(N+3/2)} \,\, b,
\label{eqn-chap2-ir-cutoff}
\end{equation}
where $b$ is the oscillator length.  Assuming that ultraviolet convergence of the calculated results has been achieved (this typically happens when the ultraviolet cutoff of the internucleon interaction $\lambda$ is smaller than the ultraviolet cutoff $\Lambda_{\mathrm{UV}}$ of the basis), then the bound state energies will converge exponentially with respect to $L$
\begin{equation}
E(N_{\mathrm{max}},\hbar\omega) = E_{\infty} +  a_{0} e^{-2 k_{\infty} L(N_{\mathrm{max}},\hbar\omega)},
\label{eqn-chap2-energy-extrapolation-theoretical}
\end{equation}
and the radii will converge as
\begin{equation}
r^{2}(L) = r_{\infty}^{2} [1 - (c_{0}+c_{1}\beta^{-2})\beta^{3}e^{-\beta}],
\label{eqn-chap2-rms-extrapolation}
\end{equation}
where $E_{\infty}$, $a_{0}$, $k_{\infty}$, $c_{0}$, $ c_{1}$, and $r_{\infty}^{2}$ are obtained by fitting calculated results and $\beta = 2k_{\infty} L$ (when fitting the rms radius, $k_{\infty}$ is taken from the energy fit). The infrared cutoff was later studied in more detail and a more precise expression for $L$ was obtained by finding the lowest eigenvalue of the operator $p^{2}$ in a finite oscillator basis~\cite{more2013:ir-extrapolation} 
\begin{equation}
L(N,\hbar\omega) = \sqrt{2(N+\Delta N + 3/2)} \,\, b(\hbar\omega),
\label{eqn-chap2-ir-length}
\end{equation}
where $\Delta N$ is an offset usually set equal to $2$.



The exponential convergence of the bound-state energies with respect to $L$ can be understood as follows~\cite{furnstahl2012:ho-extrapolation}. The finite extent $L$ of the oscillator basis in position space imposes a Dirichlet boundary condition on the bound state wave function at $r = L$. The exponential convergence with respect to $L$ is thus directly related to the exponential fall-off of the bound-state wave functions in position space. 


Let us now use the infrared extrapolation method with our calculated results. We extrapolate results calculated at the three highest $\Nmax$ truncations ($\Nmax=12$, $14$, and $16$) sharing the same $\hw$ strength (where $\hw \gtrsim 14$ MeV) which we deem as UV converged because their ultraviolet momentum $\Lambda_{UV}$ is comparable to the ultraviolet cutoff $\lambda$ of the JISP$16$ interaction~\cite{shirokov2007:nn-jisp16}. Specifically, the JISP$16$ interaction is obtained by fitting scattering data in a harmonic oscillator space with $N=8$ and $\hw = 40$ MeV, which means that $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16} \approx 800 \mathrm{MeV}/c$ according to (\ref{eqn-chap2-uv-cutoff}). Moreover, for the NCCI calculation with $\Nmax = 12$ and $\hw = 14$ MeV the same equation yields $\Lambda_{\mathrm{UV}} \approx 600 \mathrm{MeV}/c$.


The extrapolated results of both the ground state energy and proton radius of $\isotope[4]{He}$, shown in Fig.~\ref{fig-chap2-helium3-helium4}(c) and (d) respectively, converge. What we mean by using the term converge here, is that the extrapolated results do not depend on $\hw$ (however, a closer inspection reveals that there is a slight $\hw$ dependence of the extrapolated results, especially for the radius). The convergence of the extrapolated results for high $\hw$ values reassures us that the results we selected to extrapolate are UV converged. The extrapolated ground state energy of $\isotope[4]{He}$ (as well as the calculated energy at $\Nmax=16$ and $\hw$ around the variational minimum) is identical to the experimental result while the extrapolated proton radius is about $\sim 0.03$ fm short of the experimental result. This means that JISP$16$ fails to describe the proton radius, while it succeeds in the description of the ground state energy.


For $\isotope[3]{He}$, the extrapolated ground state energy [shown in Fig.~\ref{fig-chap2-helium3-helium4}(a)] converges, while the extrapolated proton radius [shown in Fig.~\ref{fig-chap2-helium3-helium4}(b)] does not (the extrapolated results depend on $\hw$). The converged result for the ground state energy implies that JISP$16$ underbinds $\isotope[3]{He}$ by $\sim 0.1$ MeV. The extrapolated proton radius results stagger around the experimental value. For $\hw > 25$ MeV, the extrapolated results are found on or around the experimental result (at the $\sim 0.1$ fm level). However, since full convergence is not achieved we cannot make a definite assessment as to whether JISP$16$ gives an accurate prediction of the proton radius of $\isotope[3]{He}$ based on Fig.~\ref{fig-chap2-helium3-helium4}(b). 


Overall, the infrared extrapolation method can be used to provide at least ``ballpark'' predictions for the value of observables in the full space. The infrared extrapolation method presented here will be used in Chapters~\ref{chap-chap3},~\ref{chap-chap4}, and~\ref{chap-chap5} to extrapolate NCCI results obtained with both the harmonic oscillator and natural orbital single-particle bases.






\section{Using a general single-particle basis in NCCI calculations}
\label{sec-chap2-general-basis}


In this section we review the procedure followed to derive the two-body matrix elements of the NCCI Hamiltonian in a general single-particle basis. The discussion follows closely the derivations discussed in Ref.~\cite{caprio2012:csbasis} where the two-body matrix elements of the NCCI Hamiltonian with respect to the Laguerre basis were derived. However, the discussion presented here is not limited to a particular single-particle basis. For example, we can use the methods presented here to derive the two-body matrix elements of the Hamiltonian in the harmonic oscillator basis (this is only possible if the interaction matrix elements with respect to the harmonic oscillator basis at a given $\hw$ are already known as discussed below). 


To aid the discussion, we will use the Laguerre basis~\cite{caprio2012:csbasis}. The Laguerre basis forms a complete, discrete, orthonormal set in the space of square integrable functions $\mathcal{L}^{2}(\mathbb{R}^{+})$. The Laguerre radial functions are given by
\begin{equation}
S_{nl}(b;r) \propto (2r/b)^{l+1} L_{n}^{2l+2} [2r/b] e^{-r/b},
\label{eqn-chap2-laguerre-radial-functions}
\end{equation}
where $n$ is the radial quantum number, $l$ is the angular momentum, and $b$ is the characteristic length of the Laguerre functions analogous to the oscillator length. For each $l$, the Laguerre functions are orthonormal in $\mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} S_{nl}(b;r) S_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-cs-orthonormal}
\end{equation}
By replacing the harmonic oscillator radial functions $R_{nl}$ in (\ref{eqn-oscillator-orbitals-second-quantization}) with $S_{nl}$ we can form Laguerre single-particle states $| \alpha \rangle$ for NCCI calculations
\begin{equation}
| \alpha \rangle = \left[| S_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}}.
\label{eqn-laguerre-orbitals-second-quantization}
\end{equation}


To build the Hamiltonian matrix using a general single-particle basis we need to calculate the two-body matrix elements of the interaction and the relative kinetic energy operators in the general basis. In the case where the two-body matrix elements of the interaction with respect to some single-particle basis are known, we can use a two-body transformation to obtain the two-body matrix elements in the general basis. For example, the JISP$16$ interaction is expressed in terms of the harmonic oscillator basis. Therefore, a two-body transformation from the harmonic oscillator to the general basis yields the two-body matrix elements in the general basis. Specifically, if $a = (n_{a}l_{a}j_{a})$ is a harmonic oscillator single-particle orbital and $\bar{a} = (\bar{n}_{a} \bar{l}_{a} \bar{j}_{a})$ is a Laguerre single-particle orbital then for antisymmetrized two-body states such as (\ref{eqn-chap2-two-particle-states-2}) the transformation is given by~\cite{hagen2006:gdm-realistic}
\begin{equation}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{AS}} = \sum_{abcd} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{AS}},
\label{eqn-chap2-two-body-interaction-transformation}
\end{equation}
where $\langle a | \bar{a} \rangle$ is an overlap bracket. For normalized antisymmetrized states such as (\ref{eqn-chap2-two-particle-states-3}) the transformation is given by
\begin{multline}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{NAS}} = (1+\delta_{\bar{a}\bar{b}})^{-1/2} (1+\delta_{\bar{c}\bar{d}})^{-1/2} \\  \sum_{abcd} (1+\delta_{ab})^{1/2} (1+\delta_{cd})^{1/2} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{NAS}}.
\label{eqn-chap2-two-body-interaction-transformation-nas}
\end{multline}
The overlap bracket is given by $\langle a | \bar{a} \rangle = \langle R_{n_{a}l_{a}} | S_{\bar{n}_{a} \bar{l}_{a}} \rangle \delta_{(l_{a}j_{a})(\bar{l}_{a}\bar{j}_{a})}$, where $\langle R_{nl} | S_{\bar{n}l} \rangle = \int_{0}^{\infty} dr R_{nl}(b_{\mathrm{HO}};r) S_{\bar{n}l}(b_{\mathrm{L}};r)$, and $b_{\mathrm{HO}}$ and $b_{\mathrm{L}}$ are the characteristic lengths of the harmonic oscillator basis and the Laguerre basis respectively. The transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) [or (\ref{eqn-chap2-two-body-interaction-transformation-nas})] involves an infinite quadruple sum over orbitals which needs to be truncated. The sum is truncated according to a one-body shell cutoff $\Ncut$ which must be selected in a way that ensures that NCCI calculations in the general basis are $\Ncut$-independent.


In principle, the two-body transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) can be used to obtain the two-body matrix elements of the relative kinetic energy operator in the general basis provided that the matrix elements in the harmonic oscillator basis are known. However, in Ref.~\cite{caprio2012:csbasis} the transformation was found to yield results which are highly sensitive to the $N_{\mathrm{cut}}$ truncation. Therefore, the two-body matrix elements of the relative kinetic energy operator were calculated directly in the general single-particle basis~\cite{caprio2012:csbasis}. Recall that the relative kinetic energy operator separates into one and two-body parts. Specifically, rearranging (\ref{eqn-chap2-kinetic-energy-decomposition}) we get
\begin{equation}
T_{\mathrm{rel}}  = \frac{1}{4 A m_{\mathrm{N}}} \sum_{i \neq j}^{A} (\mathbf{p}_{i}-\mathbf{p}_{j})^{2} = \frac{1}{2 A m_{\mathrm{N}}} \left[ (A-1) \sum_{i=1}^{A} p_{i}^{2} - \sum_{i \neq j}^{A} \mathbf{p}_{i} \cdot \mathbf{p}_{j} \right].
\label{eqn-chap2-kinetic-energy-decomposition-matrix-elements}
\end{equation}
The first term is a one-body operator the matrix elements of which can be calculated using the momentum space representation of the general single-particle basis. [For the Laguerre basis, the momentum space representation functions $\tilde{S}_{nl}(b;k)$ are given in terms of Jacobi polynomials, where $p = \hbar k$]. For the second term, the two-body matrix elements factorize according to Racah's reduction formula
\begin{equation}
\langle cd;J | \mathbf{p}_{1} \cdot \mathbf{p}_{2} | ab; J \rangle = (-1)^{j_{d}+j_{a}+J} \Gj{j_{c}}{j_{d}}{J}{j_{b}}{j_{a}}{1} \langle c || \mathbf{p}_{1} || a \rangle \langle d || \mathbf{p}_{2} || b \rangle,
\label{eqn-chap2-kinetic-energy-two-body-matrix-elements}
\end{equation}
where $\langle b || \mathbf{p} || a \rangle \propto [\int_{0}^{\infty} dk \tilde{S}_{n_{a}l_{a}}(b;k) k \tilde{S}_{n_{b}l_{b}}(b;k)] \langle l_{b} j_{b} || Y_{1} || l_{a} j_{a} \rangle$. Equation (\ref{eqn-chap2-kinetic-energy-two-body-matrix-elements}) then allows for the calculation of the two-body matrix elements of the kinetic energy operator.


The suite of computer programs h$2$utils~\cite{caprio2012:csbasis} can be used for the calculation of the two-body matrix elements of the Hamiltonian in a general single-particle basis. In the case of the harmonic oscillator basis, the two-body matrix elements can be also calculated by MFD.













==> chapters/chapter2/chapter2_draft_170222.tex <==
\chapter{INTRODUCTION TO THE NO-CORE CONFIGURATION INTERACTION APPROACH}
\label{chap-chap2}


\section{Overview}
\label{sec-chap2-overview}


In this chapter a broad overview of quantum many-body theory is presented focusing on the tools necessary to work with the no-core configuration interaction (NCCI) approach. The NCCI approach utilizes second quantization to cast the nuclear Hamiltonian into a square matrix in terms of a many-body basis. Here we describe all the steps needed to build and diagonalize the Hamiltonian matrix in some detail. Moreover, example calculations are presented and extrapolated using the infrared extrapolation method.


The general nuclear Hamiltonian for a system of $A$ nucleons interacting via two and/or three-body interactions $V(\mathbf{r}_{i},\mathbf{r}_{j})$ and $V(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k})$ respectively is given by
\begin{equation}
H = \frac{1}{2m_{\mathrm{N}}} \sum\limits_{i = 1}^{A} p_{i}^{2} + \sum_{i \neq j}^{A} V(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i \neq j \neq k}^{A} V_{\mathrm{NNN}}(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k}).
\label{eqn-chap2-overview-full-hamiltonian}
\end{equation}
Although three nucleon interactions are needed to accurately reproduce experimental data~\citep{pieperqmc:2008}, two-body interactions  provide a simpler context in which to focus on the main goal of this thesis, which is to introduce an alternative single-particle basis (other than the traditional harmonic oscillator basis) for NCCI calculations. Thus for the purpose of this thesis, we omit three-body terms from the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}).


Moreover, for reasons that have to do with the center-of-mass degree of freedom (described in Sec.~\ref{sec-chap2-com-factorization}) in the NCCI approach we do not work with the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}). Instead, we work with the translationally invariant intrinsic Hamiltonian \citep{vanhees:1983,lipkin:1958}
\begin{equation}
H_{\mathrm{in}} = T_{\mathrm{rel}} + V = \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}} 
+ \sum_{i \neq j}^{A} V_{\mathrm{NN}}(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i \neq j}^{Z} V_{\mathrm{C}}(\mathbf{r}_{i},\mathbf{r}_{j}) ,
\label{eqn-chap2-overview-hamiltonian}
\end{equation}
where $m_{\mathrm{N}} c^{2} = 938.92$ MeV is the average nucleon mass, $V_{\mathrm{NN}}$ is the internucleon interaction, and $V_{\mathrm{C}}$ is the Coulomb interaction. 


We start with a brief summary of second quantization (Sec.~\ref{sec-chap2-second-quantization}) which is then used to derive the two-body matrix elements of the NCCI Hamiltonian (Sec.~\ref{sec-chap2-tbme}). Consequently, we discuss the harmonic oscillator single-particle radial functions (Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}) and the nuclear many-body basis (Sec.~\ref{sec-chap2-many-body-basis}). The complete factorization of the center-of-mass and intrinsic portions of the many-body wave function (Sec.~\ref{sec-chap2-com-factorization}) and a description of the procedure followed to perform many-body calculations using the NCCI approach (Sec.~\ref{sec-chap2-many-body-calculations}) follow. The one-body density matrix and its properties are reviewed (Sec.~\ref{sec-chap2-one-body-density-matrix}). Example calculations for the nuclei $\isotope[3]{He}$ and $\isotope[4]{He}$ are presented, and the calculated results are extrapolated using the infrared extrapolation method (Sec.~\ref{sec-chap2-example-calculations}). We conclude this Chapter with an overview of the steps needed to perform an NCCI calculation using a general single-particle basis (Sec.~\ref{sec-chap2-general-basis}).


\section{Second quantization}
\label{sec-chap2-second-quantization}


Second quantization is used to describe systems of many identical particles. In what follows the notational conventions of Negele are used~\cite{negele1988:many-particle}.


The Hilbert space of $A$ distinguishable particles $ \mathcal{H}^{A}$ is spanned by the tensor product of $A$ distinguishable particles occupying single-particle states which belong to the single-particle Hilbert space $\mathcal{H}$ 
\begin{equation}
\mathcal{H}^{A} = \mathcal{H} \otimes \mathcal{H} \otimes \ldots \otimes \mathcal{H}.
\label{eqn-chap2-hilbert-space-product}
\end{equation}
If $\left\{ | a \rangle \right\}$ is an orthonormal basis for $\mathcal{H}$, an orthonormal basis for $\mathcal{H}^{A}$ can be constructed as the set of tensor product states
\begin{equation}
| a_{1} \ldots a_{A} ) \equiv |a_{1} \rangle \otimes |a_{2} \rangle \otimes \ldots \otimes |a_{A} \rangle,
\label{eqn-chap2-many-body-basis-product}
\end{equation}
where the curved parenthesis on the left hand side of (\ref{eqn-chap2-many-body-basis-product}) denotes that the many-body state is a simple product of single-particle states (i.e., no assumptions are made about the symmetry of the many-body state). 


The space of $A$ indistinguishable fermions $\mathcal{F}^{A}$ is spanned by fully antisymmetric many-body states constructed using the many-body states of $\mathcal{H}^{A}$  
\begin{equation}
| a_{1} \ldots a_{A} \rangle = \frac{1}{\sqrt{A!}} \sum_{P} (-1)^{P} | a_{P_{1}} \rangle \otimes | a_{P_{2}} \rangle \otimes \ldots \otimes | a_{P_{A}} \rangle.
\label{eqn-chap2-many-body-basis-antisymmetric}
\end{equation} 
The sum over $P$ is a sum over all possible permutations $(P_{1},\,P_{2},\ldots,P_{A})$ of the set $(a_{1},\,a_{2},\,\ldots, a_{A})$. Moreover, $(-1)^{P}$ is determined by counting the number of transpositions of two elements which brings a permutation to its original form $(a_{1},\,a_{2},\,\ldots, a_{A})$. 


The Fock space $F$ for fermions is the (Hilbert) direct sum of the fermion spaces $\mathcal{F}^{0}$, $\mathcal{F}^{1}$, $\mathcal{F}^{2}$, $\ldots$, $\mathcal{F}^{A}$, $\ldots$ for zero, one, two, etc particles
\begin{equation}
F = \mathcal{F}^{0} \oplus \mathcal{F}^{1} \oplus \mathcal{F}^{2} \oplus \ldots \oplus \mathcal{F}^{A} \oplus \ldots.
\label{eqn-chap2-fock-space}
\end{equation}
Here $\mathcal{F}^{0}$ is the space of no particles, $\mathcal{F}^{1}$ is identical to $\mathcal{H}$, and $\mathcal{F}^{A}$ with $A \geq 2$ is the space spanned by many-body states given by (\ref{eqn-chap2-many-body-basis-antisymmetric}).


Creation and annihilation operators generate the entire Fock space $F$ by adding (removing) single-particle states to (from) many-body states. The fermionic creation operator $c_{a}^{\dagger}$ adds a particle in a single-particle state $| a \rangle$ to the many-body state $| a_{1} \ldots a_{A} \rangle$ as follows
\begin{equation}
c_{a}^{\dagger} | a_{1} a_{2} \ldots a_{A} \rangle = | a a_{1} a_{2} \ldots a_{A} \rangle,
\label{eqn-chap2-creation-operator}
\end{equation}
where the definition implies that the particle is added to the left of the initial many-body state. Now, because of the antisymmetry requirement for fermions we cannot act with the $c_{a}^{\dagger}$ operator on the state $| a a_{1} a_{2} \ldots a_{A} \rangle$ (and thus add the single-particle state $| a \rangle$ twice). This state is equal to zero by definition
\begin{equation}
c_{a}^{\dagger} |a a_{1} a_{2} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-creation-operator-2}
\end{equation}
Similarly an annihilation operator $c_{a}$ removes a particle occupying the single-particle state $|a\rangle$ from a many-body state
\begin{equation}
c_{a} |a a_{1} \ldots a_{A} \rangle = | a_{1} \ldots a_{A} \rangle.
\label{eqn-chap2-annihilation-operator}
\end{equation}
For completeness, note that in general $c_{a} | a_{1} a_{2} \ldots a \ldots a_{A} \rangle = (-1)^{P} | a_{1} a_{2} \ldots a_{A} \rangle$ where $P$ is the number of transpositions of two elements needed to bring the particle in the single-particle state $| a \rangle$ to the front of the many-body state. For example $c_{a_{2}} | a_{1} a_{2} a_{3} \rangle = - |a_{1} a_{3} \rangle$. If $c_{a}$ acts on a state $| a_{1} \ldots a_{A} \rangle$, i.e., a state which has no particle in the single-particle state $| a \rangle$, then the action of $c_{a}$ on the many-body state $| a_{1} \ldots a_{A} \rangle$ yields zero
\begin{equation}
c_{a} |a_{1} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-annihilation-operator-2}
\end{equation}
Following from~(\ref{eqn-chap2-creation-operator})-(\ref{eqn-chap2-annihilation-operator-2}), we conclude that the creation and annihilation operators obey the fermionic anticommutation relation
\begin{equation}
\lbrace c_{a} , c_{b}^{\dagger} \rbrace = \delta_{ab}.
\label{eqn-chap2-anti-commutation}
\end{equation}


One-body operators are operators which can be written as a sum of single-particle operators acting on one particle at a time. To be able to calculate the matrix elements of one-body operators with respect to many body states like (\ref{eqn-chap2-many-body-basis-antisymmetric}), it is useful to express them in terms of creation and annihilation operators. To arrive at this expression, let us first use the many-body states of $\mathcal{H}^{A}$ to calculate the matrix elements of a one-body operator $T = \sum_{i=1}^{A} t_{i}$. For the diagonal matrix elements (i.e., between the same many-body states) we have
\begin{multline}
( a_{1}a_{2} \ldots a_{A} | T | a_{1} a_{2} \ldots a_{A} ) = \\  
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2} \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \\
\langle a_{1} | t_{1} | a_{1} \rangle + \ldots + \langle a_{A} | t_{A} | a_{A} \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-identical-states}
\end{multline}
where we used the fact that the single-particle states are orthonormal hence $\langle a_{i} | a_{j} \rangle = \delta_{ij}$. Let us now evaluate the non-diagonal matrix elements of $T$ starting with the matrix elements between the many-body state $ | a_{1} a_{2} \ldots a_{A} )$ and the many-body state $ | a_{1} a_{2}' \ldots a_{A} )$, where $| a_{2} \rangle \neq | a_{2}' \rangle$. We have
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1} a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \langle a_{1} | a_{1} \rangle \langle a_{2} | t_{2} | a_{2}' \rangle \langle a_{3} | a_{3} \rangle \ldots \langle a_{A} | a_{A} \rangle + \\
+ \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \langle a_{2} | t_{2} | a_{2}' \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-one-sp-state-different}
\end{multline}
since $\langle a_{2} | a_{2}' \rangle = 0 $. Finally, the matrix elements of $T$ between the many-body states $| a_{1} a_{2} \ldots a_{A} )$ and $| a_{1}' a_{2}' \ldots a_{A} )$, where $| a_{1} \rangle \neq | a_{1}' \rangle$ and $| a_{2} \rangle \neq | a_{2}' \rangle$, are
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1}' a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1}' \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1}' \rangle \ldots \langle a_{A} | t_{A} | a_{A} \rangle = 0.
\label{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}
\end{multline}
Thus, the matrix elements of the one-body operator $T$ with respect to many-body states of $\mathcal{H}^{A}$ are fully defined by the sum over single-particle matrix elements of $\mathcal{H}$. If we now define the single-particle vacuum state $| - \rangle$ (i.e., a non-occupied single-particle state), then $c_{a}^{\dagger} | - \rangle = | a \rangle$. Using this definition and (\ref{eqn-chap2-one-body-operator-matrix-elements-identical-states})-(\ref{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}) we can write a one-body operator as
\begin{equation}
T = \sum_{ab} t_{ab} c_{a}^{\dagger} c_{b},
\label{eqn-chap2-one-body-operator-second-quantization}
\end{equation}
where $t_{ab} = \langle a | t | b \rangle$.

Similarly, the matrix elements of a two-body operator $V = \frac{1}{2} \sum_{i \neq j} u_{ij}$ with respect to the many-body states of $ \mathcal{H}^{A}$ are fully defined by the matrix elements $u_{abcd} = (ab | u | cd )$ calculated using the states of $\mathcal{H}^{2}$. Thus we can write $V$ as
\begin{equation}
V = \frac{1}{2} \sum_{abcd} u_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c}.
\label{eqn-chap2-interaction-second-quantized}
\end{equation}
However, it is more convenient to write the two-body operator as
\begin{equation}
V = \frac{1}{4} \sum_{abcd} \bar{u}_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c},
\label{eqn-chap2-interaction-second-quantized-antisymmetrized}
\end{equation}
where $\bar{u}_{abcd} = u_{abcd} - u_{abdc} = \langle ab | u | cd \rangle$ are normalized and antisymmetrized two-body matrix elements.


\section{Two-body matrix elements for the NCCI Hamiltonian}
\label{sec-chap2-tbme}

In the context of the NCCI approach, the most commonly used single-particle states are the harmonic oscillator single-particle basis states (see Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}). A harmonic oscillator single-particle state is labeled by the quantum numbers $| \alpha \rangle \equiv |n_{a}l_{a}j_{a}m_{a} \rangle$, where $n_{a}$ is the harmonic oscillator radial quantum number, $l_{a}$ is the angular momentum, $j_{a}$ is the total angular momentum, and $m_{a}$ is the $z$ projection of the total angular momentum. Using the harmonic oscillator single-particle states we can construct fully antisymmetric many-body basis states for the NCCI approach
\begin{equation}
| (n_{a}l_{a}j_{a}m_{a}) (n_{b}l_{b}j_{b}m_{b}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle.
\label{eqn-chap2-many-body-state-harmonic-oscillator}
\end{equation} 
Many-body states such as (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) have a total $z$ projection of total angular momentum $M=\sum_{i=1}^{A} m_{i}$ and a total number of oscillator quanta $N_{\mathrm{tot}}=\sum_{i=1}^{A} (2n_{i} + l_{i}) = \sum_{i=1}^{A} N_{i}$. The harmonic oscillator single-particle states $| \alpha \rangle$ are given as the tensor product 
\begin{equation}
| \alpha \rangle = \left[| R_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}},
\label{eqn-oscillator-orbitals-second-quantization}
\end{equation}
where $R_{n_{a}l_{a}}$ is a harmonic oscillator radial function, $Y_{l_{a}}$ is a spherical harmonic, and $|\frac{1}{2} \rangle$ is a spinor. The subscripts $j_{a}$ and $m_{a}$ indicate that $| R_{n_{a} l_{a}} Y_{l_{a}} \rangle$ (a spherical tensor of rank $l_{a}$) and the spinor $| \frac{1}{2} \rangle$ are coupled to total angular momentum $j_{a}$ and $z$ projection of total angular momentum $m_{a}$~\cite{rose1957:am}. 


The Hilbert space of the NCCI Hamiltonian is spanned by the many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) which provide a basis for the representation of the Hamiltonian as a square matrix. To cast the Hamiltonian into a square matrix we must first calculate the two-body matrix elements of the relative kinetic energy and two-body $NN$ interaction operators. The two-body matrix elements are calculated with respect to two-particle states, coupled to total angular momentum $J$. For distinguishable particles (e.g., one proton and one neutron states), angular momentum coupled two-particle states are defined as 
\begin{equation}
| a b ; J ) = \sum_{m_{a}m_{b}} \langle j_{a} m_{a} j_{b} m_{b} | J M \rangle |a m_{a} \rangle | b m_{b} \rangle,
\label{eqn-chap2-two-particle-states-1}
\end{equation}
where $| a m_{a} \rangle = | n_{a} l_{a} j_{a} m_{a} \rangle$, $\langle j_{a} m_{a} j_{b} m_{b} | J M \rangle $ is a Clebsch-Gordan coefficient, and the parenthesis implies that the two-particle state is not antisymmetrized. For two identical fermions we can obtain fully antisymmetrized states using the states $| a b ; J )$. We have
\begin{equation}
| a b ; J M \rangle_{\mathrm{AS}} = \frac{1}{\sqrt{2}} \left[ | a b ; J M ) - (-1)^{J - j_{a} - j_{b}} | b a ; J M \rangle \right].
\label{eqn-chap2-two-particle-states-2}
\end{equation}
These states have the symmetry property $| a b ; J M \rangle = - (-1)^{J -j_{a}-j_{b}} | b a ; J M \rangle$ which implies that if the states $| a \rangle$ and $| b \rangle$ are identical, only two-body states with even $J$ are allowed. The states (\ref{eqn-chap2-two-particle-states-2}) are antisymmetrized but not strictly normalized. An extra factor of $1 / \sqrt{2}$ is required for normalization in the special case when the two particles occupy the same single-particle orbital $| n_{a} l_{a} j_{a} \rangle$. Hence, the appropriate two-particle states are
\begin{equation}
| a b ; J M \rangle_{\mathrm{NAS}} = (1 + \delta_{ab})^{-1/2} | a b ; J M \rangle_{\mathrm{AS}}.
\label{eqn-chap2-two-particle-states-3}
\end{equation}
Both the normalized antisymmetrized states and the antisymmetrized states are used to calculate the two-body matrix elements $\langle c d ; J | H_{\mathrm{in}} | a b ; J \rangle$ of the (scalar) intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}). The change of basis relation between two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-2}) and two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-3}) is
\begin{equation}
\langle c d ; J | H | a b ; J \rangle_{\mathrm{NAS}} = (1+\delta_{cd})^{-1/2} (1+\delta_{ab})^{-1/2} \langle c d ; J | H | a b ; J \rangle_{\mathrm{AS}}.
\label{eqn-chap2-nas-two-body-matrix-elements}
\end{equation}
A detailed discussion about the calculation of the two-body matrix elements of the intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) is given in Ref.~\cite{caprio2012:csbasis}. A brief overview is also given in Sec.~\ref{sec-chap2-general-basis}.
 

\section{The harmonic oscillator single-particle states}
\label{sec-chap2-harmonic-oscillator-radial-functions}


In this section we will review the basic properties of the harmonic oscillator single-particle states $| \alpha \rangle$~\cite{suhonen2007:nucleons-nucleus,moshinsky1996:oscillator,weniger1985:fourier-plane-wave} which are traditionally used in the NCCI approach because their properties facilitate the many-body calculations. The harmonic oscillator single-particle states are also our starting basis for the construction of natural orbitals which are introduced in Chapter~\ref{chap-chap3}. 


The first important property of the harmonic oscillator single-particle states (relevant to the NCCI approach) is that they allow for the complete removal of spurious center-of-mass states from the low-lying spectrum of the NCCI Hamiltonian provided that an $\Nmax$ truncation is imposed on the many-body basis. The appearance of spurious center-of-mass states results from using the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) for the representation of the NCCI Hamiltonian as a square matrix. A detailed discussion about the appearance of spurious center-of-mass states in an NCCI calculation and the procedure followed for their removal from the low-lying spectrum is given in Sec.~\ref{sec-chap2-many-body-basis}.

The second important property of the harmonic oscillator single-particle states (relevant to many-body calculations and consequently the NCCI approach) is that they simplify the calculation of two-body matrix elements for operators written in terms of relative coordinates, using the Moshinsky transformation~\citep{moshinsky1996:oscillator}. According to  the transformation, products of harmonic oscillator states expressed in single-particle coordinates $R_{n_{1}l_{1}}(\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ transform into products of harmonic oscillator states expressed in terms of relative and center-of mass coordinates $R_{nl}(\mathbf{r}_{\mathrm{rel}})R_{NL}(\mathbf{R})$, where $2 n_{1} + l_{1} + 2 n_{2} + l_{2}= 2 n + l+ 2 N + L$, $\mathbf{r}_{\mathrm{rel}} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}-\mathbf{r}_{2})$, and $\mathbf{R} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}+\mathbf{r}_{2})$. (The factor of $1/\sqrt{2}$ in front of the center-of-mass vector is used instead of the traditional $1/2$ for normalization reasons). The calculation of two-body matrix elements for operators of the form $V(r_{1}-r_{2})$ with respect to two-particle states of the form $R_{n_{1}l_{1}} (\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ is then reduced to the calculation of the single-particle matrix element of the operator $V(\mathbf{r}_{\mathrm{rel}})$ with respect to single-particle states of the form $R_{nl}(\mathbf{r}_{\mathrm{rel}})$ and an overlap between single-particle states of the form $R_{NL}(\mathbf{R})$.

Let us now derive the harmonic oscillator radial wave functions. If we write the single-particle wave function as $\Psi_{nlm}(\mathbf{r})=r^{-1} R_{nl}(b;r)Y_{lm}(\theta,\phi)$, where $R_{nl}(b;r)$ are radial functions and $Y_{lm}(\theta,\phi)$ are spherical harmonics, the harmonic oscillator single-particle wave functions are solutions to the familiar harmonic oscillator central force problem \cite{suhonen2007:nucleons-nucleus} 
\begin{equation}
h(\omega) = \frac{p^{2}}{2m_{\mathrm{N}}} + \frac{m_{\mathrm{N}} \omega^{2} r^{2}}{2}.
\label{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}
\end{equation} 
where $m_{\mathrm{N}}c^{2} \approx 938.92$ MeV is the average nucleon mass and $\omega$ is the oscillator frequency. The length scale of the radial functions $R_{nl}(b;r)$ is set by the oscillator length $b$ which depends on the parameters of the oscillator Hamiltonian (\ref{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}) as $b=\sqrt{\hbar / (m_{\mathrm{N}} \omega})$. The eigenvalues corresponding to each single-particle radial wave function are given by $ (N + 3/2) \hw$, where $N = 2n + l$ is the oscillator quantum (notice that the eigenvalues are evenly spaced by one unit of $\hw$). The radial functions $R_{nl}(b;r)$ are given by
\begin{equation}
R_{nl}(b;r) = b N_{nl} (r/b)^{l+1} L_{n}^{l+1/2}[(r/b)^{2}] e^{-(r/b)^{2}/2},
\label{eqn-chap2-harmonic-oscillator-radial-functions}
\end{equation} 
where $L_{n}^{l+1/2}[(r/b)^{2}]$ are generalized Laguerre polynomials, $n$ is the radial quantum number (which gives the number of nodes in the radial function), $l$ is the angular momentum, and $N_{nl}$ is a normalization factor given by
\begin{equation}
N_{nl} = \frac{1}{b^{3/2}} \left[ \frac{2n!}{(l+n+1/2)!} \right]^{1/2}.
\label{eqn-chap2-harmonic-oscillator-functions-normalization}
\end{equation}
For each $l$, the harmonic oscillator radial functions form a complete discrete basis for square integrable functions on $ \mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} R_{nl}(b;r) R_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-ho-orthonormal}
\end{equation}
 

\section{Symmetries of the NCCI Hamiltonian and the nuclear \\ many-body basis}
\label{sec-chap2-many-body-basis}


The selection of the nuclear many-body basis used in NCCI calculations is based on the symmetries of the NCCI Hamiltonian~(\ref{eqn-chap2-overview-hamiltonian}). The NCCI Hamiltonian is rotationally invariant, therefore it conserves the total angular momentum $J$ and the $z$ projection of total angular momentum $M$. Moreover, the Hamiltonian conserves parity. To diagonalize the Hamiltonian we can choose to use many-body states that have good $J$ (a $J$-scheme basis) or many-body states that have good $M$ (an $M$-scheme basis)~\cite{whitehead1977:shell-methods}. Although the $M$-scheme basis involves a larger number of many-body basis states compared to a $J$-scheme basis, constructing $M$-scheme many-body basis states is straightforward (i.e., we do not have to deal with angular momentum coupling as in the $J$-scheme basis). Therefore, for the NCCI calculations discussed here, an $M$-scheme basis is considered. However, the eigenstates of $H$ still have good $J$ which is recovered after diagonalization by calculating the expectation value of the $J^{2}$ operator with respect to the calculated many-body wave function.


To build many-body basis states we start from single-particle states $| nljm \rangle$ and construct fully antisymmetric states (with good $M$) given by~(\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Calculations can be performed for any possible value of $M$ (which is supported by the single-particle states in the many-body basis). For example, for even nuclei $M=0, 1,\ldots$ and for odd nuclei $M=1/2, 3/2, \ldots$ (we do not consider negative values for $M$ here). However, we usually use many-body states with $M=0$ for even nuclei and $M=1/2$ for odd nuclei. This is because for a given $M$ we can only obtain many-body wave functions with $J \geq | M |$. Thus, choosing the lowest possible $M$ allows us to study the ground and first few excited states of a nucleus.


Commonly, for reasons involving the center-of-mass degree of freedom, as discussed in Sec.~\ref{sec-chap2-com-factorization}, the many-body basis is truncated using the $\Nmax$ truncation scheme~\cite{elliott1955:com-shell}. The scheme dictates that only many-body states with $\Ntot \leq N_{0} + \Nmax$ are permitted in the many-body basis, where $N_{0}$ is the number of quanta in the configuration where all the nucleons occupy the lowest permitted oscillator shells. For example, $N_{0}=2$ for $\isotope[6]{He}$ (in this configuration, the two protons occupy the $N=0$ proton shell, two neutrons occupy the $N=0$ neutron shell, and the last two neutrons occupy the $N=1$ shell) and $N_{0} =3$ for $\isotope[7]{Li}$ (because the extra proton compared to $\isotope[6]{He}$ goes into the $N=1$ proton shell). 


Finally, because the nuclear Hamiltonian conserves parity we want our many-body states to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. This means that the parity of a many-body state is obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the lowest possible configuration is given by $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity states of the nucleus $\Nmax$ must be even and proceed in steps of $2$, i.e., $\Nmax = 2, 4, 6, \ldots$. On the other hand, to obtain the unnatural parity states of the nucleus $\Nmax$ must be odd and also proceed in steps of $2$, i.e., $\Nmax = 1, 3, 5, \ldots$. 






\section{Spurious center-of-mass states removal}
\label{sec-chap2-com-factorization}


In this section we describe how spurious center-of-mass states result from the diagonalization of the NCCI Hamiltonian matrix built in terms of the set of the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Subsequently, we describe how these spurious states can be removed provided that the $\Nmax$ truncation scheme is used.

The many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) are defined with respect to a fixed point in space. However, physically there is no such point around which all the nucleons are orbiting. Rather we are interested in the internal motion of the nucleons relative to each other within the nucleus, a motion which defines the intrinsic structure of the nucleus.


In principle we can convert to relative coordinates. However, antisymmetrization in Jacobi coordinates (which define the relative motion) is cumbersome. Therefore, we are compelled to work in the full coordinate space which includes both the center of mass and relative degrees of freedom.


Our goal is to describe the relative motion as accurately as possible without unnecessary complications arising from the center of mass motion. In order to accomplish this it helps making certain choices regarding the basis and the Hamiltonian.


We want our eigenfunctions to factorize into center of mass and relative factors. We also want the center of mass factor to be simple and well understood so that it does not interfere with the calculation of energies and observables. In principle, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) is already separated into center of mass and relative coordinates. If we define the center-of-mass momentum as $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, the one-body kinetic energy operator in (\ref{eqn-chap2-overview-full-hamiltonian}) can be decomposed into a center-of-mass and a relative kinetic energy contributions~\cite{vanhees:1983}
\begin{equation}
T = T_{\mathrm{c.m.}} + T_{\mathrm{rel}} = \frac{1}{2Am_{\mathrm{N}}} \left(\sum\limits_{i=1}^{A}\mathbf{p}_{i}\right)^{2} + \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}}.
\label{eqn-chap2-kinetic-energy-decomposition}
\end{equation}
Therefore, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) also separates into center-of-mass and relative parts
\begin{equation}
H= T_{\mathrm{c.m.}} + T_{\mathrm{rel}} + V.
\label{eqn-chap2-full-separated-hamiltonian}
\end{equation}
Thus, in the full space our eigenfunctions would factorize into a center-of-mass and a relative wave function.

However, we are confined to work in a truncated space. Factorization can still be exact in an oscillator basis when the $\Nmax$ truncation is used. The truncated space then only contains a limited center-of-mass space spanned by center-of-mass harmonic oscillator states with $N_{\mathrm{c.m.}} = 0$, $2$, $\ldots, \Nmax$. We could attempt to diagonalize the Hamiltonian~(\ref{eqn-chap2-full-separated-hamiltonian}) in the truncated space. However, the $T_{\mathrm{c.m.}}$ operator will mix contributions with different center-of-mass excitations $N_{\mathrm{c.m.}}$ and destroy factorization of the eigenfunctions. The Hamiltonian will force us towards states which attempt to diagonalize the center-of-mass kinetic energy operator $T_{\mathrm{c.m.}}$. Therefore, our NCCI calculations would end up approximating spherical waves in the center of mass coordinates, at the expense of accurately describing the intrinsic motion.

Thus, instead, we choose to work with the intrinsic Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V.
\end{equation} 
The resulting Hamiltonian is block diagonal with respect to the number of quanta $N_{\mathrm{c.m.}}$ for the center-of-mass motion. The resulting eigenfunctions will factorize into a center-of-mass factor of good $N_{\mathrm{c.m.}}$ and an intrinsic factor. The total number of quanta in a many-body state is shared between the center-of-mass motion and the intrinsic motion:
\begin{equation}
\Ntot = \sum_{i} N_{i} = N_{\mathrm{c.m.}} + N_{\mathrm{rel}}.
\label{eqn-chap2-number-of-quanta-com-quanta}
\end{equation}
Therefore, in eigenfunctions with $N_{\mathrm{c.m.}} = 0$, the full $\Nmax$ quanta are available to use in describing the intrinsic motion. The higher $N_{\mathrm{c.m.}}$ eigenfunctions produce spurious copies of the spectrum in which the intrinsic motion is described using fewer quanta $N_{\mathrm{rel}} \leq \Nmax - N_{\mathrm{c.m.}}$. 


It is convenient to push the spurious excited center-of-mass states out of the low lying spectrum. We do this by adding a term diagonal in the number of center-of-mass quanta. That is we add a ``Lawson term''~\cite{gloeckner1974:spurious-com} proportional to the $N_{\mathrm{c.m.}}$ operator. This is often equivalently described as adding a center-of-mass harmonic oscillator Hamiltonian. In terms of the center-of-mass coordinate $\mathbf{R} = (\sum_{i} \mathbf{r}_{i})/A$ and the center-of-mass momentum $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, 
\begin{equation}
H_{\mathrm{c.m.}} = \frac{P^{2}}{2Am_{\mathrm{N}}} + \frac{1}{2} A m_{\mathrm{N}} \omega^{2} R^{2}.
\label{eqn-chap2-harmonic-oscillator-many-body-hamiltonian-com}
\end{equation}
Then, $H_{\mathrm{c.m.}} = (N_{\mathrm{c.m.}} + 3/2)\hbar \omega$. Thus we actually diagonalize the Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V + \alpha N_{\mathrm{c.m.}},
\label{eqn-chap2-ncci-hamiltonian-with-lawson}
\end{equation} 
where $\alpha$ is the Lawson term strength (typically a few MeV). This leads to the same eigenstates as the relative Hamiltonian but with the spurious states lifted out of the low-lying spectrum by an amount of $\alpha N_{\mathrm{c.m.}}$.




\section{Many-body calculations}
\label{sec-chap2-many-body-calculations}


In this section we will briefly describe the general procedure followed to obtain results using the NCCI approach.

The basic ingredient needed to build the Hamiltonian matrix are the two-body matrix elements of the NCCI Hamiltonian (\ref{eqn-chap2-ncci-hamiltonian-with-lawson}) with respect to many-body basis states like (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Thus, we need to evaluate matrix elements of the form
\begin{equation}
\langle \Phi_{n} | H | \Phi_{m} \rangle,
\label{eqn-chap2-two-body-matrix-elements}
\end{equation}
where $| \Phi_{n} \rangle = | (n_{1}l_{1}j_{1}m_{1}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle$ is a many-body basis state. [The matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) reduce to a sum over two-body matrix elements of the form $\langle c d ; J | H | a b ; J \rangle$ using Wick's theorem]. After calculating the matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) for all the many-body states in our basis we obtain the Hamiltonian matrix
\begin{equation}
  \begin{pmatrix}
    \langle \Phi_{1} | H | \Phi_{1} \rangle & \langle \Phi_{1} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{1} | H | \Phi_{m} \rangle \\
    \langle \Phi_{2} | H | \Phi_{1} \rangle & \langle \Phi_{2} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{2} | H | \Phi_{m} \rangle \\
    \vdots & \vdots & \ddots & \vdots \\
   \langle \Phi_{m} | H | \Phi_{1} \rangle & \langle \Phi_{m} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{m} | H | \Phi_{m} \rangle
  \end{pmatrix}
\label{eqn-chap2-ncci-hamiltonian-matrix}
\end{equation}
The dimension $d$ of the matrix (\ref{eqn-chap2-ncci-hamiltonian-matrix}) is equal to the number of many-body basis states for a given nucleus and $\Nmax$ truncation (see Fig.~\ref{fig-chap1-NNCI-dimension}). Diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}) yields the nuclear many-body wave functions  
\begin{equation}
| \Psi \rangle = \sum\limits_{n=1}^{d} c_{n} | \Phi_{n} \rangle,
\label{eqn-chap2-ncci-wave-functions}
\end{equation}
where $c_{n}$ are coefficients obtained from the diagonalization of (\ref{eqn-chap2-ncci-wave-functions}).


The diagonalization of the Hamiltonian matrix is performed using the Lanczos algorithm~\cite{komzsik2003:lanczos-method,lanczos1950:algorithm}. The algorithm transforms the generally large sparse matrix (\ref{eqn-chap2-ncci-wave-functions}) into a tridiagonal matrix (of lower dimension than the original matrix). The tridiagonal matrix is then diagonalized (using an appropriate algorithm) and the eigenvalues and eigenvectors (of the tridiagonal matrix) are obtained. The eigenvectors of the tridiagonal matrix (Lanczos vectors) must then be converted from the Lanczos vector space to the original many-body basis. The process established by Lanczos proceeds as follows: If $H$ is a Hamiltonian matrix of order $n$ (i.e., the matrix dimension is $n \times n$), then we start with a random initial vector $b_{0}$ which is used to construct $m$ vectors (orthogonal to each other) according to the algorithm
\begin{align}
b_{0} & = \mathrm{random}, \nonumber & \\
b_{1} & = (H - \alpha_{0}) b_{0}, \nonumber \\
b_{2} & = (H - \alpha_{1}) b_{1} - \beta_{0} b_{0}, \nonumber \\
b_{3} & = (H - \alpha_{2}) b_{2} -\beta_{1} b_{1}, \nonumber \\
 \vdots  \nonumber & \\
b_{m} & = (H - \alpha_{m-1}) b_{m-1} - \beta_{m-2} b_{m-2},
\label{eqn-chap2-lanczos-algorithm}
\end{align}
where $m \leq n$. The equality to zero in the last step means the end of the process. The coefficients $\alpha_{m-1}$ and $\beta_{m-2}$ are determined by requiring that the norm of the vector $\parallel b_{m} \parallel$ is minimized and they are used to build the tridiagonal matrix 
\begin{equation}
T =  \begin{pmatrix}
\alpha_{0} & \beta_{0} &   &   & 0\\ 
\beta_{0}  & \alpha_{1} & \beta_{1} & \\
                 & \ddots & \ddots & \ddots & \\
                 &  & \beta_{k-2} & \alpha_{k-1} &\beta_{k-1} \\
           0      & & & \beta_{k-1} & \alpha_{k}
  \end{pmatrix}
\label{eqn-chap2-tridiagonal-matrix}
\end{equation}
The eigenvalues of $T$ converge to the first $k$ eigenvalues of $H$ provided that a sufficient number of iterations $k$, where $k < n$, is performed. 


The generally large sizes of the NCCI Hamiltonian matrices require the use of parallel computing which handles both the storage and the of the Hamiltonian matrix. The parallel code Many Fermion Dynamics (MFD) \cite{maris2010:ncsm-mfdn-iccs10,vary2009:ncsm-mfdn-scidac09} developed by the Iowa State University group handles the construction of the many-body basis, the construction of the Hamiltonian matrix, the storage of the matrix over multiple cores, and the Lanczos diagonalization of the matrix. The input to the code includes the two-body matrix elements of the Hamiltonian, the $\Nmax$ truncation of the many-body basis, the number of protons ($Z$) and neutrons ($N$) of the nucleus we want to study, the number of Lanczos iterations we want to perform, and various other control parameters. The program outputs multiple files containing the eigenvalues (which are the nuclear level energies), the one-body density matrices (described in Sec.~\ref{sec-chap2-one-body-density-matrix}), and other observables.


\section{The one-body density matrix}
\label{sec-chap2-one-body-density-matrix}


The one-body density matrix is a fundamental tool in many-body calculations which is used for the calculation of the matrix elements of one-body operators~\cite{suhonen2007:nucleons-nucleus}. In second quantization, the matrix elements of the transition one-body density matrix are given by
\begin{equation}
\rho_{\alpha\beta}^{\mathrm{f\,i}} = \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger} c_{\beta} | \Psi_{\mathrm{i}} \rangle,
\label{eqn-chap2-one-body-density-operator}
\end{equation}
where $| \Psi_{\mathrm{i}} \rangle$ and $| \Psi_{\mathrm{f}} \rangle$ are the many-body wave functions of an initial and a final nuclear state respectively. Using (\ref{eqn-chap2-one-body-density-operator}), the matrix elements of a one-body operator $\mathcal{O}$ are obtained as
\begin{equation}
\langle \Psi_{\mathrm{f}} | \mathcal{O} | \Psi_{\mathrm{i}} \rangle =  \sum_{\alpha\beta} \langle \alpha | \mathcal{O} | \beta \rangle \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger}c_{\beta} | \Psi_{\mathrm{i}} \rangle.
\label{eqn-chap2-one-body-operator-matrix-elements}
\end{equation}


The static one-body density matrix (i.e., the one-body density matrix obtained for the same initial and final many-body wave functions) contains information about correlations in the many-body wave function. By definition, an uncorrelated many-body wave function is written as a single Slater determinant, i.e., $| \Psi \rangle = | a_{1} \ldots a_{A} \rangle$. For an uncorrelated many-body wave function, it is easy to see that the diagonal matrix elements $\rho_{\alpha\alpha} = \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle $ are equal to $1$ (which reflects the fact that each single-particle state is occupied by exactly one nucleon), while all the off diagonal matrix elements $\rho_{\alpha\beta}$ are equal to zero. The sum of the diagonal matrix elements is equal to the total number of nucleons $A$ in the many-body wave function. In the case of a highly correlated many-body wave function, such as the ones calculated in an NCCI calculation, the one-body density matrix is not (in general) diagonal. The off diagonal matrix elements $\rho_{\alpha\beta}$ of the density matrix provide a measure of how correlated the many-body wave function is, while the diagonal matrix elements $\rho_{\alpha\alpha}$ provide the occupancies of each single-particle state $| a_{i} \rangle$ in the many-body wave function. The sum over the diagonal matrix elements is still equal to the total number of nucleons in the many-body wave function
\begin{equation}
\sum_{\alpha} \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle = A.
\label{eqn-chap2-density-matrix-number}
\end{equation}
It is important to stress here that a diagonal one-body density matrix does not necessarily indicate that a many-body wave function is uncorrelated unless the diagonal matrix elements $\rho_{\alpha \alpha}$ are exactly equal to $1$. The one-body density matrix is the starting point for the construction of natural orbitals in Chapter~\ref{chap-chap3}.


\section{Example calculations and infrared extrapolations}
\label{sec-chap2-example-calculations}


In this section we perform NCCI calculations to obtain the ground state energy and proton radius of the isotopes $\isotope[3,4]{He}$. Our goal is to revisit the convergence properties of NCCI calculations using the harmonic oscillator basis and to extrapolate the calculated results to the full $\Nmax \rightarrow \infty$ space using the infrared extrapolation method which we present and discuss here.


In Fig.~\ref{fig-chap2-helium3-helium4}, we plot the calculated ground state energy (left) and proton radius (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom). Calculations were performed for even truncations of the many-body basis up to $\Nmax = 16$ (in steps of $2$) which scan the $\hw$ range $10$-$40$ MeV. The solid lines correspond to the calculated results, the dashed horizontal lines correspond to the experimental results, and the dotted lines connect extrapolated results obtained using the infrared extrapolation method (discussed below). The experimental binding energies are taken from~\cite{npa-purcell-a-3-data:2010,npa-tilley-a-4-data:1992}, while the proton radii are deduced using the experimentally measured nuclear charge radii found in~\cite{angeli-marinova-nuclear-charge-radii:2013} and equation ($6$) in Ref.~\cite{bacca2012:6he-hyperspherical}. As we observe, the calculated ground state energy and proton radius of $\isotope[4]{He}$ converge. On the other hand, the calculated ground state energy of $\isotope[3]{He}$ approaches convergence (to the $\sim 0.01$ MeV level), while the proton radius does not converge.
 


Comparisons of NCCI calculations with experimental results are only meaningful once full convergence is achieved. However, when the calculated results do not converge we can attempt to extrapolate results obtained in truncated spaces to the full $\Nmax \rightarrow \infty$ space. One such example was presented in Chapter~\ref{chap-chap1}, where we used an empirical extrapolation method to extrapolate the calculated ground state energy of $\isotope[6]{He}$ to the full space. Here, we use the infrared extrapolation method to extrapolate the calculated ground state energy and proton radius of $\isotope[3,4]{He}$ to the full space. Extrapolating the converged $\isotope[4]{He}$ results serves as a test of the infrared method as we expect the extrapolated results to agree with the converged results.


The infrared extrapolation method~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation, more2013:ir-extrapolation,furnstahl2014:ir-expansion, furnstahl2015:ir-extrapolations,odell-papenbrock-ir-extrapolation-quadruple:2016} starts with the assumption that the truncated many-body basis  induces both a short-range ultraviolet (UV) and a long-range infrared (IR) cutoff on the ability of the many-body basis to describe the many-body wave function. Quantitatively, if the highest occupied single-particle orbital in the many-body basis has $N$ oscillator quanta, then to a first approximation the momentum space (UV) cutoff is~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation}
\begin{equation}
\Lambda_{\mathrm{UV}} = \sqrt{2(N+3/2)} \,\, \hbar/b,
\label{eqn-chap2-uv-cutoff}
\end{equation}
and the coordinate space (IR) cutoff is
\begin{equation}
L = \sqrt{2(N+3/2)} \,\, b,
\label{eqn-chap2-ir-cutoff}
\end{equation}
where $b$ is the oscillator length.  Assuming that ultraviolet convergence of the calculated results is reached (this typically happens when the ultraviolet cutoff of the internucleon interaction $\lambda$ is smaller than the ultraviolet cutoff $\Lambda_{\mathrm{UV}}$ of the basis), the bound state energies will converge exponentially with respect to $L$
\begin{equation}
E(N_{\mathrm{max}},\hbar\omega) = E_{\infty} +  a_{0} e^{-2 k_{\infty} L(N_{\mathrm{max}},\hbar\omega)},
\label{eqn-chap2-energy-extrapolation-theoretical}
\end{equation}
and the radii will converge as
\begin{equation}
r^{2}(L) = r_{\infty}^{2} [1 - (c_{0}+c_{1}\beta^{-2})\beta^{3}e^{-\beta}],
\label{eqn-chap2-rms-extrapolation}
\end{equation}
where $E_{\infty}$, $a_{0}$, $k_{\infty}$, $c_{0}$, $ c_{1}$, and $r_{\infty}^{2}$ are obtained by fitting (UV converged) calculated results and $\beta = 2k_{\infty} L$ [$k_{\infty}$ is taken from the energy fit in (\ref{eqn-chap2-rms-extrapolation})]. The infrared cutoff was later studied in more detail and a more precise expression for $L$ was obtained by finding the lowest eigenvalue of the operator $p^{2}$ in a finite oscillator basis~\cite{more2013:ir-extrapolation} 
\begin{equation}
L(N,\hbar\omega) = \sqrt{2(N+\Delta N + 3/2)} \,\, b(\hbar\omega),
\label{eqn-chap2-ir-length}
\end{equation}
where $\Delta N$ is an offset typically set equal to $2$.



The exponential convergence of the bound-state energies with respect to $L$ can be understood as follows~\cite{furnstahl2012:ho-extrapolation}. The finite extent $L$ of the oscillator basis in position space imposes a Dirichlet boundary condition on the bound state wave function at $r = L$. The exponential convergence with respect to $L$ is thus directly related to the exponential fall-off of the bound-state wave functions in position space. 


Let us now use the infrared extrapolation method with our calculated results. Here, we perform a three point extrapolation using the calculated results at $\Nmax=12$, $14$, and $16$ sharing the same $\hw$ parameter. We deem results obtained using $\hw$ parameters $\hw \gtrsim 14$ MeV UV converged because their ultraviolet momentum $\Lambda_{UV}$ is comparable to the ultraviolet cutoff $\lambda$ of the JISP$16$ interaction~\cite{shirokov2007:nn-jisp16}. Specifically, the JISP$16$ interaction is obtained by fitting scattering data in a harmonic oscillator space with $N=8$ and $\hw = 40$ MeV, which means that according to (\ref{eqn-chap2-uv-cutoff}) $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16} \approx 800$ $\mathrm{MeV}/c$. For the NCCI calculation with $\Nmax = 12$ and $\hw = 14$ MeV equation (\ref{eqn-chap2-uv-cutoff}) yields $\Lambda_{\mathrm{UV}} \approx 600$ $\mathrm{MeV}/c$.


In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (c)] and proton radius [panel (d)] of $\isotope[4]{He}$. As expected, the extrapolated results converge for both observables. A closer inspection reveals that a slight $\hw$ dependence persists which is however very small (at the $0.01$ MeV and $0.01$ fm for the extrapolated energy and proton radius respectively). For low $\hw$ parameters, the extrapolated energy does not converge which we expect since the calculated results used for the extrapolation are not fully UV converged. On the other hand, for high $\hw$ the extrapolated results converge since the calculated results used for the extrapolation are UV converged. The extrapolated ground state energy at $\hw \approx 20$ MeV ($-28.3$ MeV) agrees with the calculated result at the variational minimum of the $\Nmax = 16$ curve and the experimental result ($-28.3$ MeV). On the other hand, the extrapolated proton radius at $\hw \approx 20$ MeV ($1.44$ fm) agrees with the calculated result at $\Nmax = 16$ ($1.44$ fm) however it is about $\sim 0.03$ fm short of the experimental result. Thus, the NCCI calculation using the JISP$16$ interaction while predicting the binding energy correctly, it underestimates the proton radius.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{\plotspath /ho_no_comparison/Z2-N1-Z2-N2-rp-e-HO-thesis-chapter1-170111.pdf}
\caption[Calculated ground state energy and proton radius in the ground state of {\protect $\isotope[3]{He}$} and {\protect $\isotope[3]{He}$}, obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The calculated results are extrapolated to the full space using the infrared extrapolation method.]{Calculated ground state energy (left) and proton radius in the ground state (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom), obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The dashed horizontal lines show the experimental results. The crosses connected by dotted lines are obtained by extrapolating calculated results using the infrared extrapolation method as described in the text.}
\label{fig-chap2-helium3-helium4}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (a)] and proton radius [panel (b)] of $\isotope[4]{He}$. We observe that the calculated ground state energy converges (to the $0.01$ MeV level). The extrapolated result is about $\sim 0.1$ MeV short of the experimental result ($-7.72$ MeV). The extrapolated proton radius staggers around the experimental result (at the $0.1$ fm level). However, since full convergence is not achieved we cannot assess whether the calculation correctly predicts the proton radius.



\section{Using a general single-particle basis in NCCI calculations}
\label{sec-chap2-general-basis}


In this section we review the procedure followed to derive the two-body matrix elements of the NCCI Hamiltonian in a general single-particle basis. The discussion follows closely the derivations discussed in Ref.~\cite{caprio2012:csbasis} where the two-body matrix elements of the NCCI Hamiltonian with respect to the Laguerre basis were derived. However, the discussion presented here is not limited to a particular single-particle basis. 


However, to aid the discussion we will use the Laguerre basis~\cite{caprio2012:csbasis} in the derivations. The Laguerre basis forms a complete, discrete, orthonormal set in the space of square integrable functions $\mathcal{L}^{2}(\mathbb{R}^{+})$. The Laguerre radial functions are given by
\begin{equation}
S_{nl}(b;r) = (2/b)^{-1} N_{nl} (2r/b)^{l+1} L_{n}^{2l+2} [2r/b] e^{-r/b},
\label{eqn-chap2-laguerre-radial-functions}
\end{equation}
where $n$ is the radial quantum number, $l$ is the angular momentum, $b$ is the characteristic length of the Laguerre functions, and $N_{nl}$ is a normalization given by
\begin{equation}
N_{nl} = \left( \frac{2}{b} \right)^{3/2} \left[ \frac{n!}{(n+2l+2)!} \right]^{1/2}.
\label{eqn-chap2-laguerre-normalization-coefficient}
\end{equation}
For each $l$, the Laguerre functions are orthonormal in $\mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} S_{nl}(b;r) S_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-cs-orthonormal}
\end{equation}
By replacing the harmonic oscillator radial functions $R_{nl}$ in (\ref{eqn-oscillator-orbitals-second-quantization}) with $S_{nl}$ we can form Laguerre single-particle states $| \alpha \rangle$ given by
\begin{equation}
| \alpha \rangle = \left[| S_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}}.
\label{eqn-laguerre-orbitals-second-quantization}
\end{equation}


To build the Hamiltonian matrix using a general single-particle basis we need to calculate the two-body matrix elements of the interaction and relative kinetic energy operators in the general basis. In the case where the two-body matrix elements of the interaction with respect to some single-particle basis are known, we can use a two-body transformation to obtain the two-body matrix elements in the general basis. For example, the JISP$16$ interaction is expressed in terms of the harmonic oscillator basis. Therefore, we can use a two-body transformation which will yield the two-body matrix elements in the general basis. Specifically, if $a = (n_{a}l_{a}j_{a})$ is a harmonic oscillator single-particle orbital and $\bar{a} = (\bar{n}_{a} \bar{l}_{a} \bar{j}_{a})$ is a Laguerre single-particle orbital then for antisymmetrized two-body states such as (\ref{eqn-chap2-two-particle-states-2}) the transformation is given by~\cite{hagen2006:gdm-realistic}
\begin{equation}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{AS}} = \sum_{abcd} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{AS}},
\label{eqn-chap2-two-body-interaction-transformation}
\end{equation}
where $\langle a | \bar{a} \rangle$ is an overlap bracket. For normalized antisymmetrized states such as (\ref{eqn-chap2-two-particle-states-3}) the transformation is given by
\begin{multline}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{NAS}} = (1+\delta_{\bar{a}\bar{b}})^{-1/2} (1+\delta_{\bar{c}\bar{d}})^{-1/2} \\  \sum_{abcd} (1+\delta_{ab})^{1/2} (1+\delta_{cd})^{1/2} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{NAS}}.
\label{eqn-chap2-two-body-interaction-transformation-nas}
\end{multline}
The overlap bracket is given by 
\begin{equation}
\langle a | \bar{a} \rangle = \langle R_{n_{a}l_{a}} | S_{\bar{n}_{a} \bar{l}_{a}} \rangle \delta_{(l_{a}j_{a})(\bar{l}_{a}\bar{j}_{a})}, 
\label{eqn-chap2-overlap-bracket}
\end{equation}
where 
\begin{equation}
\langle R_{nl} | S_{\bar{n}l} \rangle = \int_{0}^{\infty} dr R_{nl}(b_{\mathrm{HO}};r) S_{\bar{n}l}(b_{\mathrm{L}};r), 
\label{eqn-chap2-overlap-integral}
\end{equation}
and $b_{\mathrm{HO}}$ and $b_{\mathrm{L}}$ are the characteristic lengths of the harmonic oscillator basis and the Laguerre basis respectively. The transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) [or (\ref{eqn-chap2-two-body-interaction-transformation-nas})] involves an infinite quadruple sum over orbitals. The sum is truncated according to a one-body shell cutoff $\Ncut$ which must be selected in a way which ensures that NCCI calculations in the general basis are $\Ncut$ independent.


In principle, the two-body transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) can be used to obtain the two-body matrix elements of the relative kinetic energy operator in the general basis (provided that the matrix elements in the harmonic oscillator or other basis are known). However, in Ref.~\cite{caprio2012:csbasis} the transformation was found to yield calculated results which are highly sensitive to the $N_{\mathrm{cut}}$ truncation. Therefore, the two-body matrix elements of the relative kinetic energy operator were calculated directly in the general single-particle basis~\cite{caprio2012:csbasis}. Recall that the relative kinetic energy operator separates into one and two-body parts. Specifically, rearranging (\ref{eqn-chap2-kinetic-energy-decomposition}) we get
\begin{equation}
T_{\mathrm{rel}}  = \frac{1}{4 A m_{\mathrm{N}}} \sum_{i \neq j}^{A} (\mathbf{p}_{i}-\mathbf{p}_{j})^{2} = \frac{1}{2 A m_{\mathrm{N}}} \left[ (A-1) \sum_{i=1}^{A} p_{i}^{2} - \sum_{i \neq j}^{A} \mathbf{p}_{i} \cdot \mathbf{p}_{j} \right].
\label{eqn-chap2-kinetic-energy-decomposition-matrix-elements}
\end{equation}
The first term is a one-body operator the matrix elements of which can be calculated using the momentum space representation of the general single-particle basis. [For the Laguerre basis, the momentum space representation functions $\tilde{S}_{nl}(b;k)$, where $p = \hbar k$, are given in terms of Jacobi polynomials]. The second term is a two-body operator the matrix elements of which factorize according to Racah's reduction formula~\cite{suhonen2007:nucleons-nucleus}
\begin{equation}
\langle cd;J | \mathbf{p}_{1} \cdot \mathbf{p}_{2} | ab; J \rangle = (-1)^{j_{d}+j_{a}+J} \Gj{j_{c}}{j_{d}}{J}{j_{b}}{j_{a}}{1} \langle c || \mathbf{p}_{1} || a \rangle \langle d || \mathbf{p}_{2} || b \rangle,
\label{eqn-chap2-kinetic-energy-two-body-matrix-elements}
\end{equation}
where $\langle b || \mathbf{p} || a \rangle \propto [\int_{0}^{\infty} dk \tilde{S}_{n_{a}l_{a}}(b;k) k \tilde{S}_{n_{b}l_{b}}(b;k)] \langle l_{b} j_{b} || Y_{1} || l_{a} j_{a} \rangle$.


The suite of computer programs h$2$utils~\cite{caprio2012:csbasis} can be used for the calculation of the two-body matrix elements of the Hamiltonian in a general single-particle basis. The program calculates the two-body matrix elements of the relative kinetic energy operator and the two-body matrix elements of the interaction as separate matrices. The two matrices are then added (allowing the user to select different length parameters $b_{p}$ and $b_{n}$ for the proton and neutron spaces respectively), thus resulting in a Hamiltonian matrix which can then be used as an input to MFD which performs the many-body calculation.













==> chapters/chapter2/chapter2_draft_170227.tex <==
\chapter{INTRODUCTION TO THE NO-CORE CONFIGURATION INTERACTION APPROACH}
\label{chap-chap2}


\section{Overview}
\label{sec-chap2-overview}


In this chapter a broad overview of quantum many-body theory is presented focusing on the tools necessary to work with the no-core configuration interaction (NCCI) approach. The NCCI approach utilizes second quantization to cast the nuclear Hamiltonian into a square matrix in terms of a many-body basis. Here we describe all the steps needed to build and diagonalize the Hamiltonian matrix in some detail. Moreover, example calculations are presented and extrapolated using the infrared extrapolation method.


The general nuclear Hamiltonian for a system of $A$ nucleons interacting via two and/or three-body interactions $V(\mathbf{r}_{i},\mathbf{r}_{j})$ and $V(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k})$ respectively is given by
\begin{equation}
H = \frac{1}{2m_{\mathrm{N}}} \sum\limits_{i = 1}^{A} p_{i}^{2} + \sum_{i \neq j}^{A} V(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i \neq j \neq k}^{A} V_{\mathrm{NNN}}(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k}).
\label{eqn-chap2-overview-full-hamiltonian}
\end{equation}
Although three nucleon interactions are needed to accurately reproduce experimental data~\citep{pieperqmc:2008}, two-body interactions  provide a simpler context in which to focus on the main goal of this thesis, which is to introduce an alternative single-particle basis (other than the traditional harmonic oscillator basis) for NCCI calculations. Thus for the purpose of this thesis, we omit three-body terms from the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}).


Moreover, for reasons that have to do with the center-of-mass degree of freedom (described in Sec.~\ref{sec-chap2-com-factorization}) in the NCCI approach we do not work with the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}). Instead, we work with the translationally invariant intrinsic Hamiltonian \citep{vanhees:1983,lipkin:1958}
\begin{equation}
H_{\mathrm{in}} = T_{\mathrm{rel}} + V = \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}} 
+ \sum_{i \neq j}^{A} V_{\mathrm{NN}}(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i \neq j}^{Z} V_{\mathrm{C}}(\mathbf{r}_{i},\mathbf{r}_{j}) ,
\label{eqn-chap2-overview-hamiltonian}
\end{equation}
where $m_{\mathrm{N}} c^{2} = 938.92$ MeV is the average nucleon mass, $V_{\mathrm{NN}}$ is the internucleon interaction, and $V_{\mathrm{C}}$ is the Coulomb interaction. 


We start with a brief summary of second quantization (Sec.~\ref{sec-chap2-second-quantization}) which is then used to derive the two-body matrix elements of the NCCI Hamiltonian (Sec.~\ref{sec-chap2-tbme}). Consequently, we discuss the harmonic oscillator single-particle radial functions (Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}) and the nuclear many-body basis (Sec.~\ref{sec-chap2-many-body-basis}). The complete factorization of the center-of-mass and intrinsic portions of the many-body wave function (Sec.~\ref{sec-chap2-com-factorization}) and a description of the procedure followed to perform many-body calculations using the NCCI approach (Sec.~\ref{sec-chap2-many-body-calculations}) follow. The one-body density matrix and its properties are reviewed (Sec.~\ref{sec-chap2-one-body-density-matrix}). Example calculations for the nuclei $\isotope[3]{He}$ and $\isotope[4]{He}$ are presented, and the calculated results are extrapolated using the infrared extrapolation method (Sec.~\ref{sec-chap2-example-calculations}). We conclude this Chapter with an overview of the steps needed to perform an NCCI calculation using a general single-particle basis (Sec.~\ref{sec-chap2-general-basis}).


\section{Second quantization}
\label{sec-chap2-second-quantization}


Second quantization is used to describe systems of many identical particles. In what follows the notational conventions of Negele are used~\cite{negele1988:many-particle}.


The Hilbert space of $A$ distinguishable particles $ \mathcal{H}^{A}$ is spanned by the tensor product of $A$ distinguishable particles occupying single-particle states which belong to the single-particle Hilbert space $\mathcal{H}$ 
\begin{equation}
\mathcal{H}^{A} = \mathcal{H} \otimes \mathcal{H} \otimes \ldots \otimes \mathcal{H}.
\label{eqn-chap2-hilbert-space-product}
\end{equation}
If $\left\{ | a \rangle \right\}$ is an orthonormal basis for $\mathcal{H}$, an orthonormal basis for $\mathcal{H}^{A}$ can be constructed as the set of tensor product states
\begin{equation}
| a_{1} \ldots a_{A} ) \equiv |a_{1} \rangle \otimes |a_{2} \rangle \otimes \ldots \otimes |a_{A} \rangle,
\label{eqn-chap2-many-body-basis-product}
\end{equation}
where the curved parenthesis on the left hand side of (\ref{eqn-chap2-many-body-basis-product}) denotes that the many-body state is a simple product of single-particle states (i.e., no assumptions are made about the symmetry of the many-body state). 


The space of $A$ indistinguishable fermions $\mathcal{F}^{A}$ is spanned by fully antisymmetric many-body states constructed using the many-body states of $\mathcal{H}^{A}$  
\begin{equation}
| a_{1} \ldots a_{A} \rangle = \frac{1}{\sqrt{A!}} \sum_{P} (-1)^{P} | a_{P_{1}} \rangle \otimes | a_{P_{2}} \rangle \otimes \ldots \otimes | a_{P_{A}} \rangle.
\label{eqn-chap2-many-body-basis-antisymmetric}
\end{equation} 
The sum over $P$ is a sum over all possible permutations $(P_{1},\,P_{2},\ldots,P_{A})$ of the set $(a_{1},\,a_{2},\,\ldots, a_{A})$. Moreover, $(-1)^{P}$ is determined by counting the number of transpositions of two elements which brings a permutation to its original form $(a_{1},\,a_{2},\,\ldots, a_{A})$. 


The Fock space $F$ for fermions is the (Hilbert) direct sum of the fermion spaces $\mathcal{F}^{0}$, $\mathcal{F}^{1}$, $\mathcal{F}^{2}$, $\ldots$, $\mathcal{F}^{A}$, $\ldots$ for zero, one, two, etc particles
\begin{equation}
F = \mathcal{F}^{0} \oplus \mathcal{F}^{1} \oplus \mathcal{F}^{2} \oplus \ldots \oplus \mathcal{F}^{A} \oplus \ldots.
\label{eqn-chap2-fock-space}
\end{equation}
Here $\mathcal{F}^{0}$ is the space of no particles, $\mathcal{F}^{1}$ is identical to $\mathcal{H}$, and $\mathcal{F}^{A}$ with $A \geq 2$ is the space spanned by many-body states given by (\ref{eqn-chap2-many-body-basis-antisymmetric}).


Creation and annihilation operators generate the entire Fock space $F$ by adding (removing) single-particle states to (from) many-body states. The fermionic creation operator $c_{a}^{\dagger}$ adds a particle in a single-particle state $| a \rangle$ to the many-body state $| a_{1} \ldots a_{A} \rangle$ as follows
\begin{equation}
c_{a}^{\dagger} | a_{1} a_{2} \ldots a_{A} \rangle = | a a_{1} a_{2} \ldots a_{A} \rangle,
\label{eqn-chap2-creation-operator}
\end{equation}
where the definition implies that the particle is added to the left of the initial many-body state. Now, because of the antisymmetry requirement for fermions we cannot act with the $c_{a}^{\dagger}$ operator on the state $| a a_{1} a_{2} \ldots a_{A} \rangle$ (and thus add the single-particle state $| a \rangle$ twice). This state is equal to zero by definition
\begin{equation}
c_{a}^{\dagger} |a a_{1} a_{2} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-creation-operator-2}
\end{equation}
Similarly an annihilation operator $c_{a}$ removes a particle occupying the single-particle state $|a\rangle$ from a many-body state
\begin{equation}
c_{a} |a a_{1} \ldots a_{A} \rangle = | a_{1} \ldots a_{A} \rangle.
\label{eqn-chap2-annihilation-operator}
\end{equation}
For completeness, note that in general $c_{a} | a_{1} a_{2} \ldots a \ldots a_{A} \rangle = (-1)^{P} | a_{1} a_{2} \ldots a_{A} \rangle$ where $P$ is the number of transpositions of two elements needed to bring the particle in the single-particle state $| a \rangle$ to the front of the many-body state. For example $c_{a_{2}} | a_{1} a_{2} a_{3} \rangle = - |a_{1} a_{3} \rangle$. If $c_{a}$ acts on a state $| a_{1} \ldots a_{A} \rangle$, i.e., a state which has no particle in the single-particle state $| a \rangle$, then the action of $c_{a}$ on the many-body state $| a_{1} \ldots a_{A} \rangle$ yields zero
\begin{equation}
c_{a} |a_{1} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-annihilation-operator-2}
\end{equation}
Following from~(\ref{eqn-chap2-creation-operator})-(\ref{eqn-chap2-annihilation-operator-2}), we conclude that the creation and annihilation operators obey the fermionic anticommutation relation
\begin{equation}
\lbrace c_{a} , c_{b}^{\dagger} \rbrace = \delta_{ab}.
\label{eqn-chap2-anti-commutation}
\end{equation}


One-body operators are operators which can be written as a sum of single-particle operators acting on one particle at a time. To be able to calculate the matrix elements of one-body operators with respect to many body states like (\ref{eqn-chap2-many-body-basis-antisymmetric}), it is useful to express them in terms of creation and annihilation operators. To arrive at this expression, let us first use the many-body states of $\mathcal{H}^{A}$ to calculate the matrix elements of a one-body operator $T = \sum_{i=1}^{A} t_{i}$. For the diagonal matrix elements (i.e., between the same many-body states) we have
\begin{multline}
( a_{1}a_{2} \ldots a_{A} | T | a_{1} a_{2} \ldots a_{A} ) = \\  
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2} \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \\
\langle a_{1} | t_{1} | a_{1} \rangle + \ldots + \langle a_{A} | t_{A} | a_{A} \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-identical-states}
\end{multline}
where we used the fact that the single-particle states are orthonormal hence $\langle a_{i} | a_{j} \rangle = \delta_{ij}$. Let us now evaluate the non-diagonal matrix elements of $T$ starting with the matrix elements between the many-body state $ | a_{1} a_{2} \ldots a_{A} )$ and the many-body state $ | a_{1} a_{2}' \ldots a_{A} )$, where $| a_{2} \rangle \neq | a_{2}' \rangle$. We have
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1} a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \langle a_{1} | a_{1} \rangle \langle a_{2} | t_{2} | a_{2}' \rangle \langle a_{3} | a_{3} \rangle \ldots \langle a_{A} | a_{A} \rangle + \\
+ \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \langle a_{2} | t_{2} | a_{2}' \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-one-sp-state-different}
\end{multline}
since $\langle a_{2} | a_{2}' \rangle = 0 $. Finally, the matrix elements of $T$ between the many-body states $| a_{1} a_{2} \ldots a_{A} )$ and $| a_{1}' a_{2}' \ldots a_{A} )$, where $| a_{1} \rangle \neq | a_{1}' \rangle$ and $| a_{2} \rangle \neq | a_{2}' \rangle$, are
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1}' a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1}' \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1}' \rangle \ldots \langle a_{A} | t_{A} | a_{A} \rangle = 0.
\label{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}
\end{multline}
Thus, the matrix elements of the one-body operator $T$ with respect to many-body states of $\mathcal{H}^{A}$ are fully defined by the sum over single-particle matrix elements of $\mathcal{H}$. If we now define the single-particle vacuum state $| - \rangle$ (i.e., a non-occupied single-particle state), then $c_{a}^{\dagger} | - \rangle = | a \rangle$. Using this definition and (\ref{eqn-chap2-one-body-operator-matrix-elements-identical-states})-(\ref{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}) we can write a one-body operator as
\begin{equation}
T = \sum_{ab} t_{ab} c_{a}^{\dagger} c_{b},
\label{eqn-chap2-one-body-operator-second-quantization}
\end{equation}
where $t_{ab} = \langle a | t | b \rangle$.

Similarly, the matrix elements of a two-body operator $V = \frac{1}{2} \sum_{i \neq j} u_{ij}$ with respect to the many-body states of $ \mathcal{H}^{A}$ are fully defined by the matrix elements $u_{abcd} = (ab | u | cd )$ calculated using the states of $\mathcal{H}^{2}$. Thus we can write $V$ as
\begin{equation}
V = \frac{1}{2} \sum_{abcd} u_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c}.
\label{eqn-chap2-interaction-second-quantized}
\end{equation}
However, it is more convenient to write the two-body operator as
\begin{equation}
V = \frac{1}{4} \sum_{abcd} \bar{u}_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c},
\label{eqn-chap2-interaction-second-quantized-antisymmetrized}
\end{equation}
where $\bar{u}_{abcd} = u_{abcd} - u_{abdc} = \langle ab | u | cd \rangle$ are normalized and antisymmetrized two-body matrix elements.


\section{Two-body matrix elements for the NCCI Hamiltonian}
\label{sec-chap2-tbme}

In the context of the NCCI approach, the most commonly used single-particle states are the harmonic oscillator single-particle basis states (see Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}). A harmonic oscillator single-particle state is labeled by the quantum numbers $| \alpha \rangle \equiv |n_{a}l_{a}j_{a}m_{a} \rangle$, where $n_{a}$ is the harmonic oscillator radial quantum number, $l_{a}$ is the angular momentum, $j_{a}$ is the total angular momentum, and $m_{a}$ is the $z$ projection of the total angular momentum. Using the harmonic oscillator single-particle states we can construct fully antisymmetric many-body basis states for the NCCI approach
\begin{equation}
| (n_{a}l_{a}j_{a}m_{a}) (n_{b}l_{b}j_{b}m_{b}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle.
\label{eqn-chap2-many-body-state-harmonic-oscillator}
\end{equation} 
Many-body states such as (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) have a total $z$ projection of total angular momentum $M=\sum_{i=1}^{A} m_{i}$ and a total number of oscillator quanta $N_{\mathrm{tot}}=\sum_{i=1}^{A} (2n_{i} + l_{i}) = \sum_{i=1}^{A} N_{i}$. The harmonic oscillator single-particle states $| \alpha \rangle$ are given as the tensor product 
\begin{equation}
| \alpha \rangle = \left[| R_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}},
\label{eqn-oscillator-orbitals-second-quantization}
\end{equation}
where $R_{n_{a}l_{a}}$ is a harmonic oscillator radial function, $Y_{l_{a}}$ is a spherical harmonic, and $|\frac{1}{2} \rangle$ is a spinor. The subscripts $j_{a}$ and $m_{a}$ indicate that $| R_{n_{a} l_{a}} Y_{l_{a}} \rangle$ (a spherical tensor of rank $l_{a}$) and the spinor $| \frac{1}{2} \rangle$ are coupled to total angular momentum $j_{a}$ and $z$ projection of total angular momentum $m_{a}$~\cite{rose1957:am}. 


The Hilbert space of the NCCI Hamiltonian is spanned by the many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) which provide a basis for the representation of the Hamiltonian as a square matrix. To cast the Hamiltonian into a square matrix we must first calculate the two-body matrix elements of the relative kinetic energy and two-body $NN$ interaction operators. The two-body matrix elements are calculated with respect to two-particle states, coupled to total angular momentum $J$. For distinguishable particles (e.g., one proton and one neutron states), angular momentum coupled two-particle states are defined as 
\begin{equation}
| a b ; J ) = \sum_{m_{a}m_{b}} \langle j_{a} m_{a} j_{b} m_{b} | J M \rangle |a m_{a} \rangle | b m_{b} \rangle,
\label{eqn-chap2-two-particle-states-1}
\end{equation}
where $| a m_{a} \rangle = | n_{a} l_{a} j_{a} m_{a} \rangle$, $\langle j_{a} m_{a} j_{b} m_{b} | J M \rangle $ is a Clebsch-Gordan coefficient, and the parenthesis implies that the two-particle state is not antisymmetrized. For two identical fermions we can obtain fully antisymmetrized states using the states $| a b ; J )$. We have
\begin{equation}
| a b ; J M \rangle_{\mathrm{AS}} = \frac{1}{\sqrt{2}} \left[ | a b ; J M ) - (-1)^{J - j_{a} - j_{b}} | b a ; J M \rangle \right].
\label{eqn-chap2-two-particle-states-2}
\end{equation}
These states have the symmetry property $| a b ; J M \rangle = - (-1)^{J -j_{a}-j_{b}} | b a ; J M \rangle$ which implies that if the states $| a \rangle$ and $| b \rangle$ are identical, only two-body states with even $J$ are allowed. The states (\ref{eqn-chap2-two-particle-states-2}) are antisymmetrized but not strictly normalized. An extra factor of $1 / \sqrt{2}$ is required for normalization in the special case when the two particles occupy the same single-particle orbital $| n_{a} l_{a} j_{a} \rangle$. Hence, the appropriate two-particle states are
\begin{equation}
| a b ; J M \rangle_{\mathrm{NAS}} = (1 + \delta_{ab})^{-1/2} | a b ; J M \rangle_{\mathrm{AS}}.
\label{eqn-chap2-two-particle-states-3}
\end{equation}
Both the normalized antisymmetrized states and the antisymmetrized states are used to calculate the two-body matrix elements $\langle c d ; J | H_{\mathrm{in}} | a b ; J \rangle$ of the (scalar) intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}). The change of basis relation between two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-2}) and two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-3}) is
\begin{equation}
\langle c d ; J | H | a b ; J \rangle_{\mathrm{NAS}} = (1+\delta_{cd})^{-1/2} (1+\delta_{ab})^{-1/2} \langle c d ; J | H | a b ; J \rangle_{\mathrm{AS}}.
\label{eqn-chap2-nas-two-body-matrix-elements}
\end{equation}
A detailed discussion about the calculation of the two-body matrix elements of the intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) is given in Ref.~\cite{caprio2012:csbasis}. A brief overview is also given in Sec.~\ref{sec-chap2-general-basis}.
 

\section{The harmonic oscillator single-particle states}
\label{sec-chap2-harmonic-oscillator-radial-functions}


In this section we will review the basic properties of the harmonic oscillator single-particle states $| \alpha \rangle$~\cite{suhonen2007:nucleons-nucleus,moshinsky1996:oscillator,weniger1985:fourier-plane-wave} which are traditionally used in the NCCI approach because their properties facilitate the many-body calculations. The harmonic oscillator single-particle states are also our starting basis for the construction of natural orbitals which are introduced in Chapter~\ref{chap-chap3}. 


The first important property of the harmonic oscillator single-particle states (relevant to the NCCI approach) is that they allow for the complete removal of spurious center-of-mass states from the low-lying spectrum of the NCCI Hamiltonian provided that an $\Nmax$ truncation is imposed on the many-body basis. The appearance of spurious center-of-mass states results from using the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) for the representation of the NCCI Hamiltonian as a square matrix. A detailed discussion about the appearance of spurious center-of-mass states in an NCCI calculation and the procedure followed for their removal from the low-lying spectrum is given in Sec.~\ref{sec-chap2-many-body-basis}.

The second important property of the harmonic oscillator single-particle states (relevant to many-body calculations and consequently the NCCI approach) is that they simplify the calculation of two-body matrix elements for operators written in terms of relative coordinates, using the Moshinsky transformation~\citep{moshinsky1996:oscillator}. According to  the transformation, products of harmonic oscillator states expressed in single-particle coordinates $R_{n_{1}l_{1}}(\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ transform into products of harmonic oscillator states expressed in terms of relative and center-of mass coordinates $R_{nl}(\mathbf{r}_{\mathrm{rel}})R_{NL}(\mathbf{R})$, where $2 n_{1} + l_{1} + 2 n_{2} + l_{2}= 2 n + l+ 2 N + L$, $\mathbf{r}_{\mathrm{rel}} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}-\mathbf{r}_{2})$, and $\mathbf{R} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}+\mathbf{r}_{2})$. (The factor of $1/\sqrt{2}$ in front of the center-of-mass vector is used instead of the traditional $1/2$ for normalization reasons). The calculation of two-body matrix elements for operators of the form $V(r_{1}-r_{2})$ with respect to two-particle states of the form $R_{n_{1}l_{1}} (\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ is then reduced to the calculation of the single-particle matrix element of the operator $V(\mathbf{r}_{\mathrm{rel}})$ with respect to single-particle states of the form $R_{nl}(\mathbf{r}_{\mathrm{rel}})$ and an overlap between single-particle states of the form $R_{NL}(\mathbf{R})$.

Let us now derive the harmonic oscillator radial wave functions. If we write the single-particle wave function as $\Psi_{nlm}(\mathbf{r})=r^{-1} R_{nl}(b;r)Y_{lm}(\theta,\phi)$, where $R_{nl}(b;r)$ are radial functions and $Y_{lm}(\theta,\phi)$ are spherical harmonics, the harmonic oscillator single-particle wave functions are solutions to the familiar harmonic oscillator central force problem \cite{suhonen2007:nucleons-nucleus} 
\begin{equation}
h(\omega) = \frac{p^{2}}{2m_{\mathrm{N}}} + \frac{m_{\mathrm{N}} \omega^{2} r^{2}}{2}.
\label{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}
\end{equation} 
where $m_{\mathrm{N}}c^{2} \approx 938.92$ MeV is the average nucleon mass and $\omega$ is the oscillator frequency. The length scale of the radial functions $R_{nl}(b;r)$ is set by the oscillator length $b$ which depends on the parameters of the oscillator Hamiltonian (\ref{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}) as $b=\sqrt{\hbar / (m_{\mathrm{N}} \omega})$. The eigenvalues corresponding to each single-particle radial wave function are given by $ (N + 3/2) \hw$, where $N = 2n + l$ is the oscillator quantum (notice that the eigenvalues are evenly spaced by one unit of $\hw$). The radial functions $R_{nl}(b;r)$ are given by
\begin{equation}
R_{nl}(b;r) = b N_{nl} (r/b)^{l+1} L_{n}^{l+1/2}[(r/b)^{2}] e^{-(r/b)^{2}/2},
\label{eqn-chap2-harmonic-oscillator-radial-functions}
\end{equation} 
where $L_{n}^{l+1/2}[(r/b)^{2}]$ are generalized Laguerre polynomials, $n$ is the radial quantum number (which gives the number of nodes in the radial function), $l$ is the angular momentum, and $N_{nl}$ is a normalization factor given by
\begin{equation}
N_{nl} = \frac{1}{b^{3/2}} \left[ \frac{2n!}{(l+n+1/2)!} \right]^{1/2}.
\label{eqn-chap2-harmonic-oscillator-functions-normalization}
\end{equation}
For each $l$, the harmonic oscillator radial functions form a complete discrete basis for square integrable functions on $ \mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} R_{nl}(b;r) R_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-ho-orthonormal}
\end{equation}
 

\section{Symmetries of the NCCI Hamiltonian and the nuclear \\ many-body basis}
\label{sec-chap2-many-body-basis}


The selection of the nuclear many-body basis used in NCCI calculations is based on the symmetries of the NCCI Hamiltonian~(\ref{eqn-chap2-overview-hamiltonian}). The NCCI Hamiltonian is rotationally invariant, therefore it conserves the total angular momentum $J$ and the $z$ projection of total angular momentum $M$. Moreover, the Hamiltonian conserves parity. To diagonalize the Hamiltonian we can choose to use many-body states that have good $J$ (a $J$-scheme basis) or many-body states that have good $M$ (an $M$-scheme basis)~\cite{whitehead1977:shell-methods}. Although the $M$-scheme basis involves a larger number of many-body basis states compared to a $J$-scheme basis, constructing $M$-scheme many-body basis states is straightforward (i.e., we do not have to deal with angular momentum coupling as in the $J$-scheme basis). Therefore, for the NCCI calculations discussed here, an $M$-scheme basis is considered. However, the eigenstates of $H$ still have good $J$ which is recovered after diagonalization by calculating the expectation value of the $J^{2}$ operator with respect to the calculated many-body wave function.


To build many-body basis states we start from single-particle states $| nljm \rangle$ and construct fully antisymmetric states (with good $M$) given by~(\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Calculations can be performed for any possible value of $M$ (which is supported by the single-particle states in the many-body basis). For example, for even nuclei $M=0, 1,\ldots$ and for odd nuclei $M=1/2, 3/2, \ldots$ (we do not consider negative values for $M$ here). However, we usually use many-body states with $M=0$ for even nuclei and $M=1/2$ for odd nuclei. This is because for a given $M$ we can only obtain many-body wave functions with $J \geq | M |$. Thus, choosing the lowest possible $M$ allows us to study the ground and first few excited states of a nucleus.


Commonly, for reasons involving the center-of-mass degree of freedom, as discussed in Sec.~\ref{sec-chap2-com-factorization}, the many-body basis is truncated using the $\Nmax$ truncation scheme~\cite{elliott1955:com-shell}. The scheme dictates that only many-body states with $\Ntot \leq N_{0} + \Nmax$ are permitted in the many-body basis, where $N_{0}$ is the number of quanta in the configuration where all the nucleons occupy the lowest permitted oscillator shells. For example, $N_{0}=2$ for $\isotope[6]{He}$ (in this configuration, the two protons occupy the $N=0$ proton shell, two neutrons occupy the $N=0$ neutron shell, and the last two neutrons occupy the $N=1$ shell) and $N_{0} =3$ for $\isotope[7]{Li}$ (because the extra proton compared to $\isotope[6]{He}$ goes into the $N=1$ proton shell). 


Finally, because the nuclear Hamiltonian conserves parity we want our many-body states to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. This means that the parity of a many-body state is obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the lowest possible configuration is given by $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity states of the nucleus $\Nmax$ must be even and proceed in steps of $2$, i.e., $\Nmax = 2, 4, 6, \ldots$. On the other hand, to obtain the unnatural parity states of the nucleus $\Nmax$ must be odd and also proceed in steps of $2$, i.e., $\Nmax = 1, 3, 5, \ldots$. 






\section{Spurious center-of-mass states removal}
\label{sec-chap2-com-factorization}


In this section we describe how spurious center-of-mass states result from the diagonalization of the NCCI Hamiltonian matrix built in terms of the set of the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Subsequently, we describe how these spurious states can be removed provided that the $\Nmax$ truncation scheme is used.

The many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) are defined with respect to a fixed point in space. However, physically there is no such point around which all the nucleons are orbiting. Rather we are interested in the internal motion of the nucleons relative to each other within the nucleus, a motion which defines the intrinsic structure of the nucleus.


In principle we can convert to relative coordinates. However, antisymmetrization in Jacobi coordinates (which define the relative motion) is cumbersome. Therefore, we are compelled to work in the full coordinate space which includes both the center of mass and relative degrees of freedom.


Our goal is to describe the relative motion as accurately as possible without unnecessary complications arising from the center of mass motion. In order to accomplish this it helps making certain choices regarding the basis and the Hamiltonian.


We want our eigenfunctions to factorize into center of mass and relative factors. We also want the center of mass factor to be simple and well understood so that it does not interfere with the calculation of energies and observables. In principle, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) is already separated into center of mass and relative coordinates. If we define the center-of-mass momentum as $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, the one-body kinetic energy operator in (\ref{eqn-chap2-overview-full-hamiltonian}) can be decomposed into a center-of-mass and a relative kinetic energy contributions~\cite{vanhees:1983}
\begin{equation}
T = T_{\mathrm{c.m.}} + T_{\mathrm{rel}} = \frac{1}{2Am_{\mathrm{N}}} \left(\sum\limits_{i=1}^{A}\mathbf{p}_{i}\right)^{2} + \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}}.
\label{eqn-chap2-kinetic-energy-decomposition}
\end{equation}
Therefore, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) also separates into center-of-mass and relative parts
\begin{equation}
H= T_{\mathrm{c.m.}} + T_{\mathrm{rel}} + V.
\label{eqn-chap2-full-separated-hamiltonian}
\end{equation}
Thus, in the full space our eigenfunctions would factorize into a center-of-mass and a relative wave function.

However, we are confined to work in a truncated space. Factorization can still be exact in an oscillator basis when the $\Nmax$ truncation is used. The truncated space then only contains a limited center-of-mass space spanned by center-of-mass harmonic oscillator states with $N_{\mathrm{c.m.}} = 0$, $2$, $\ldots, \Nmax$. We could attempt to diagonalize the Hamiltonian~(\ref{eqn-chap2-full-separated-hamiltonian}) in the truncated space. However, the $T_{\mathrm{c.m.}}$ operator will mix contributions with different center-of-mass excitations $N_{\mathrm{c.m.}}$ and destroy factorization of the eigenfunctions. The Hamiltonian will force us towards states which attempt to diagonalize the center-of-mass kinetic energy operator $T_{\mathrm{c.m.}}$. Therefore, our NCCI calculations would end up approximating spherical waves in the center of mass coordinates, at the expense of accurately describing the intrinsic motion.

Thus, instead, we choose to work with the intrinsic Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V.
\end{equation} 
The resulting Hamiltonian is block diagonal with respect to the number of quanta $N_{\mathrm{c.m.}}$ for the center-of-mass motion. The resulting eigenfunctions will factorize into a center-of-mass factor of good $N_{\mathrm{c.m.}}$ and an intrinsic factor. The total number of quanta in a many-body state is shared between the center-of-mass motion and the intrinsic motion:
\begin{equation}
\Ntot = \sum_{i} N_{i} = N_{\mathrm{c.m.}} + N_{\mathrm{rel}}.
\label{eqn-chap2-number-of-quanta-com-quanta}
\end{equation}
Therefore, in eigenfunctions with $N_{\mathrm{c.m.}} = 0$, the full $\Nmax$ quanta are available to use in describing the intrinsic motion. The higher $N_{\mathrm{c.m.}}$ eigenfunctions produce spurious copies of the spectrum in which the intrinsic motion is described using fewer quanta $N_{\mathrm{rel}} \leq \Nmax - N_{\mathrm{c.m.}}$. 


It is convenient to push the spurious excited center-of-mass states out of the low lying spectrum. We do this by adding a term diagonal in the number of center-of-mass quanta. That is we add a ``Lawson term''~\cite{gloeckner1974:spurious-com} proportional to the $N_{\mathrm{c.m.}}$ operator. This is often equivalently described as adding a center-of-mass harmonic oscillator Hamiltonian. In terms of the center-of-mass coordinate $\mathbf{R} = (\sum_{i} \mathbf{r}_{i})/A$ and the center-of-mass momentum $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, 
\begin{equation}
H_{\mathrm{c.m.}} = \frac{P^{2}}{2Am_{\mathrm{N}}} + \frac{1}{2} A m_{\mathrm{N}} \omega^{2} R^{2}.
\label{eqn-chap2-harmonic-oscillator-many-body-hamiltonian-com}
\end{equation}
Then, $H_{\mathrm{c.m.}} = (N_{\mathrm{c.m.}} + 3/2)\hbar \omega$. Thus we actually diagonalize the Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V + \alpha N_{\mathrm{c.m.}},
\label{eqn-chap2-ncci-hamiltonian-with-lawson}
\end{equation} 
where $\alpha$ is the Lawson term strength (typically a few MeV). This leads to the same eigenstates as the relative Hamiltonian but with the spurious states lifted out of the low-lying spectrum by an amount of $\alpha N_{\mathrm{c.m.}}$.




\section{Many-body calculations}
\label{sec-chap2-many-body-calculations}


In this section we will briefly describe the general procedure followed to obtain results using the NCCI approach.

The basic ingredient needed to build the Hamiltonian matrix are the two-body matrix elements of the NCCI Hamiltonian (\ref{eqn-chap2-ncci-hamiltonian-with-lawson}) with respect to many-body basis states like (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Thus, we need to evaluate matrix elements of the form
\begin{equation}
\langle \Phi_{n} | H | \Phi_{m} \rangle,
\label{eqn-chap2-two-body-matrix-elements}
\end{equation}
where $| \Phi_{n} \rangle = | (n_{1}l_{1}j_{1}m_{1}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle$ is a many-body basis state. [The matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) reduce to a sum over two-body matrix elements of the form $\langle c d ; J | H | a b ; J \rangle$ using Wick's theorem]. After calculating the matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) for all the many-body states in our basis we obtain the Hamiltonian matrix
\begin{equation}
  \begin{pmatrix}
    \langle \Phi_{1} | H | \Phi_{1} \rangle & \langle \Phi_{1} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{1} | H | \Phi_{m} \rangle \\
    \langle \Phi_{2} | H | \Phi_{1} \rangle & \langle \Phi_{2} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{2} | H | \Phi_{m} \rangle \\
    \vdots & \vdots & \ddots & \vdots \\
   \langle \Phi_{m} | H | \Phi_{1} \rangle & \langle \Phi_{m} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{m} | H | \Phi_{m} \rangle
  \end{pmatrix}
\label{eqn-chap2-ncci-hamiltonian-matrix}
\end{equation}
The dimension $d$ of the matrix (\ref{eqn-chap2-ncci-hamiltonian-matrix}) is equal to the number of many-body basis states for a given nucleus and $\Nmax$ truncation (see Fig.~\ref{fig-chap1-NNCI-dimension}). Diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}) yields the nuclear many-body wave functions  
\begin{equation}
| \Psi \rangle = \sum\limits_{n=1}^{d} c_{n} | \Phi_{n} \rangle,
\label{eqn-chap2-ncci-wave-functions}
\end{equation}
where $c_{n}$ are coefficients obtained from the diagonalization of (\ref{eqn-chap2-ncci-wave-functions}).


The diagonalization of the Hamiltonian matrix is performed using the Lanczos algorithm~\cite{komzsik2003:lanczos-method,lanczos1950:algorithm}. The algorithm transforms the generally large sparse matrix (\ref{eqn-chap2-ncci-wave-functions}) into a tridiagonal matrix (of lower dimension than the original matrix). The tridiagonal matrix is then diagonalized (using an appropriate algorithm) and the eigenvalues and eigenvectors (of the tridiagonal matrix) are obtained. The eigenvectors of the tridiagonal matrix (Lanczos vectors) must then be converted from the Lanczos vector space to the original many-body basis. The process established by Lanczos proceeds as follows: If $H$ is a Hamiltonian matrix of order $n$ (i.e., the matrix dimension is $n \times n$), then we start with a random initial vector $b_{0}$ which is used to construct $m$ vectors (orthogonal to each other) according to the algorithm
\begin{align}
b_{0} & = \mathrm{random}, \nonumber & \\
b_{1} & = (H - \alpha_{0}) b_{0}, \nonumber \\
b_{2} & = (H - \alpha_{1}) b_{1} - \beta_{0} b_{0}, \nonumber \\
b_{3} & = (H - \alpha_{2}) b_{2} -\beta_{1} b_{1}, \nonumber \\
 \vdots  \nonumber & \\
b_{m} & = (H - \alpha_{m-1}) b_{m-1} - \beta_{m-2} b_{m-2},
\label{eqn-chap2-lanczos-algorithm}
\end{align}
where $m \leq n$. The equality to zero in the last step means the end of the process. The coefficients $\alpha_{m-1}$ and $\beta_{m-2}$ are determined by requiring that the norm of the vector $\parallel b_{m} \parallel$ is minimized and they are used to build the tridiagonal matrix 
\begin{equation}
T =  \begin{pmatrix}
\alpha_{0} & \beta_{0} &   &   & 0\\ 
\beta_{0}  & \alpha_{1} & \beta_{1} & \\
                 & \ddots & \ddots & \ddots & \\
                 &  & \beta_{k-2} & \alpha_{k-1} &\beta_{k-1} \\
           0      & & & \beta_{k-1} & \alpha_{k}
  \end{pmatrix}
\label{eqn-chap2-tridiagonal-matrix}
\end{equation}
The eigenvalues of $T$ converge to the first $k$ eigenvalues of $H$ provided that a sufficient number of iterations $k$, where $k < n$, is performed. 


The generally large sizes of the NCCI Hamiltonian matrices require the use of parallel computing which handles both the storage and the of the Hamiltonian matrix. The parallel code Many Fermion Dynamics (MFD) \cite{maris2010:ncsm-mfdn-iccs10,vary2009:ncsm-mfdn-scidac09} developed by the Iowa State University group handles the construction of the many-body basis, the construction of the Hamiltonian matrix, the storage of the matrix over multiple cores, and the Lanczos diagonalization of the matrix. The input to the code includes the two-body matrix elements of the Hamiltonian, the $\Nmax$ truncation of the many-body basis, the number of protons ($Z$) and neutrons ($N$) of the nucleus we want to study, the number of Lanczos iterations we want to perform, and various other control parameters. The program outputs multiple files containing the eigenvalues (which are the nuclear level energies), the one-body density matrices (described in Sec.~\ref{sec-chap2-one-body-density-matrix}), and other observables.


\section{The one-body density matrix}
\label{sec-chap2-one-body-density-matrix}


The one-body density matrix is a fundamental tool in many-body calculations which is used for the calculation of the matrix elements of one-body operators~\cite{suhonen2007:nucleons-nucleus}. In second quantization, the matrix elements of the transition one-body density matrix are given by
\begin{equation}
\rho_{\alpha\beta}^{\mathrm{f\,i}} = \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger} c_{\beta} | \Psi_{\mathrm{i}} \rangle,
\label{eqn-chap2-one-body-density-operator}
\end{equation}
where $| \Psi_{\mathrm{i}} \rangle$ and $| \Psi_{\mathrm{f}} \rangle$ are the many-body wave functions of an initial and a final nuclear state respectively. Using (\ref{eqn-chap2-one-body-density-operator}), the matrix elements of a one-body operator $\mathcal{O}$ are obtained as
\begin{equation}
\langle \Psi_{\mathrm{f}} | \mathcal{O} | \Psi_{\mathrm{i}} \rangle =  \sum_{\alpha\beta} \langle \alpha | \mathcal{O} | \beta \rangle \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger}c_{\beta} | \Psi_{\mathrm{i}} \rangle.
\label{eqn-chap2-one-body-operator-matrix-elements}
\end{equation}


The static one-body density matrix (i.e., the one-body density matrix obtained for the same initial and final many-body wave functions) contains information about correlations in the many-body wave function. By definition, an uncorrelated many-body wave function is written as a single Slater determinant, i.e., $| \Psi \rangle = | a_{1} \ldots a_{A} \rangle$. For an uncorrelated many-body wave function, it is easy to see that the diagonal matrix elements $\rho_{\alpha\alpha} = \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle $ are equal to $1$ (which reflects the fact that each single-particle state is occupied by exactly one nucleon), while all the off diagonal matrix elements $\rho_{\alpha\beta}$ are equal to zero. The sum of the diagonal matrix elements is equal to the total number of nucleons $A$ in the many-body wave function. In the case of a highly correlated many-body wave function, such as the ones calculated in an NCCI calculation, the one-body density matrix is not (in general) diagonal. The off diagonal matrix elements $\rho_{\alpha\beta}$ of the density matrix provide a measure of how correlated the many-body wave function is, while the diagonal matrix elements $\rho_{\alpha\alpha}$ provide the occupancies of each single-particle state $| a_{i} \rangle$ in the many-body wave function. The sum over the diagonal matrix elements is still equal to the total number of nucleons in the many-body wave function
\begin{equation}
\sum_{\alpha} \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle = A.
\label{eqn-chap2-density-matrix-number}
\end{equation}
It is important to stress here that a diagonal one-body density matrix does not necessarily indicate that a many-body wave function is uncorrelated unless the diagonal matrix elements $\rho_{\alpha \alpha}$ are exactly equal to $1$. The one-body density matrix is the starting point for the construction of natural orbitals in Chapter~\ref{chap-chap3}.


\section{Example calculations and infrared extrapolations}
\label{sec-chap2-example-calculations}


In this section we perform NCCI calculations to obtain the ground state energy and proton radius of the isotopes $\isotope[3,4]{He}$. Our goal is to revisit the convergence properties of NCCI calculations using the harmonic oscillator basis and to extrapolate the calculated results to the full $\Nmax \rightarrow \infty$ space using the infrared extrapolation method which we present and discuss here.


In Fig.~\ref{fig-chap2-helium3-helium4}, we plot the calculated ground state energy (left) and proton radius (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom). Calculations were performed for even truncations of the many-body basis up to $\Nmax = 16$ (in steps of $2$) which scan the $\hw$ range $10$-$40$ MeV. The solid lines correspond to the calculated results, the dashed horizontal lines correspond to the experimental results, and the dotted lines connect extrapolated results obtained using the infrared extrapolation method (discussed below). The experimental binding energies are taken from~\cite{npa-purcell-a-3-data:2010,npa-tilley-a-4-data:1992}, while the proton radii are deduced using the experimentally measured nuclear charge radii found in~\cite{angeli-marinova-nuclear-charge-radii:2013} and equation ($6$) in Ref.~\cite{bacca2012:6he-hyperspherical}. As we observe, the calculated ground state energy and proton radius of $\isotope[4]{He}$ converge. On the other hand, the calculated ground state energy of $\isotope[3]{He}$ approaches convergence (to the $\sim 0.01$ MeV level), while the proton radius does not converge.
 


Comparisons of NCCI calculations with experimental results are only meaningful once full convergence is achieved. However, when the calculated results do not converge we can attempt to extrapolate results obtained in truncated spaces to the full $\Nmax \rightarrow \infty$ space. One such example was presented in Chapter~\ref{chap-chap1}, where we used an empirical extrapolation method to extrapolate the calculated ground state energy of $\isotope[6]{He}$ to the full space. Here, we use the infrared extrapolation method to extrapolate the calculated ground state energy and proton radius of $\isotope[3,4]{He}$ to the full space. Extrapolating the converged $\isotope[4]{He}$ results serves as a test of the infrared method as we expect the extrapolated results to agree with the converged results.


The infrared extrapolation method~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation, more2013:ir-extrapolation,furnstahl2014:ir-expansion, furnstahl2015:ir-extrapolations,odell-papenbrock-ir-extrapolation-quadruple:2016} starts with the assumption that the truncated many-body basis  induces both a short-range ultraviolet (UV) and a long-range infrared (IR) cutoff on the ability of the many-body basis to describe the many-body wave function. Quantitatively, if the highest occupied single-particle orbital in the many-body basis has $N$ oscillator quanta, then to a first approximation the momentum space (UV) cutoff is~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation}
\begin{equation}
\Lambda_{\mathrm{UV}} = \sqrt{2(N+3/2)} \,\, \hbar/b,
\label{eqn-chap2-uv-cutoff}
\end{equation}
and the coordinate space (IR) cutoff is
\begin{equation}
L = \sqrt{2(N+3/2)} \,\, b,
\label{eqn-chap2-ir-cutoff}
\end{equation}
where $b$ is the oscillator length.  Assuming that ultraviolet convergence of the calculated results is reached (this typically happens when the ultraviolet cutoff of the internucleon interaction $\lambda$ is smaller than the ultraviolet cutoff $\Lambda_{\mathrm{UV}}$ of the basis), the bound state energies will converge exponentially with respect to $L$
\begin{equation}
E(N_{\mathrm{max}},\hbar\omega) = E_{\infty} +  a_{0} e^{-2 k_{\infty} L(N_{\mathrm{max}},\hbar\omega)},
\label{eqn-chap2-energy-extrapolation-theoretical}
\end{equation}
and the radii will converge as
\begin{equation}
r^{2}(L) = r_{\infty}^{2} [1 - (c_{0}+c_{1}\beta^{-2})\beta^{3}e^{-\beta}],
\label{eqn-chap2-rms-extrapolation}
\end{equation}
where $E_{\infty}$, $a_{0}$, $k_{\infty}$, $c_{0}$, $ c_{1}$, and $r_{\infty}^{2}$ are obtained by fitting (UV converged) calculated results and $\beta = 2k_{\infty} L$ [$k_{\infty}$ is taken from the energy fit in (\ref{eqn-chap2-rms-extrapolation})]. The infrared cutoff was later studied in more detail and a more precise expression for $L$ was obtained by finding the lowest eigenvalue of the operator $p^{2}$ in a finite oscillator basis~\cite{more2013:ir-extrapolation} 
\begin{equation}
L(N,\hbar\omega) = \sqrt{2(N+\Delta N + 3/2)} \,\, b(\hbar\omega),
\label{eqn-chap2-ir-length}
\end{equation}
where $\Delta N$ is an offset typically set equal to $2$.



The exponential convergence of the bound-state energies with respect to $L$ can be understood as follows~\cite{furnstahl2012:ho-extrapolation}. The finite extent $L$ of the oscillator basis in position space imposes a Dirichlet boundary condition on the bound state wave function at $r = L$. The exponential convergence with respect to $L$ is thus directly related to the exponential fall-off of the bound-state wave functions in position space. 


Let us now use the infrared extrapolation method with our calculated results. Here, we perform a three point extrapolation using the calculated results at $\Nmax=12$, $14$, and $16$ sharing the same $\hw$ parameter. We deem results obtained using $\hw$ parameters $\hw \gtrsim 14$ MeV UV converged because their ultraviolet momentum $\Lambda_{UV}$ is comparable to the ultraviolet cutoff $\lambda$ of the JISP$16$ interaction~\cite{shirokov2007:nn-jisp16}. Specifically, the JISP$16$ interaction is obtained by fitting scattering data in a harmonic oscillator space with $N=8$ and $\hw = 40$ MeV, which means that according to (\ref{eqn-chap2-uv-cutoff}) $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16} \approx 800$ $\mathrm{MeV}/c$. For the NCCI calculation with $\Nmax = 12$ and $\hw = 14$ MeV equation (\ref{eqn-chap2-uv-cutoff}) yields $\Lambda_{\mathrm{UV}} \approx 600$ $\mathrm{MeV}/c$.


In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (c)] and proton radius [panel (d)] of $\isotope[4]{He}$. As expected, the extrapolated results converge for both observables. A closer inspection reveals that a slight $\hw$ dependence persists which is however very small (at the $0.01$ MeV and $0.01$ fm for the extrapolated energy and proton radius respectively). For low $\hw$ parameters, the extrapolated energy does not converge which we expect since the calculated results used for the extrapolation are not fully UV converged. On the other hand, for high $\hw$ the extrapolated results converge since the calculated results used for the extrapolation are UV converged. The extrapolated ground state energy at $\hw \approx 20$ MeV ($-28.3$ MeV) agrees with the calculated result at the variational minimum of the $\Nmax = 16$ curve and the experimental result ($-28.3$ MeV). On the other hand, the extrapolated proton radius at $\hw \approx 20$ MeV ($1.44$ fm) agrees with the calculated result at $\Nmax = 16$ ($1.44$ fm) however it is about $\sim 0.03$ fm short of the experimental result. Thus, the NCCI calculation using the JISP$16$ interaction while predicting the binding energy correctly, it underestimates the proton radius.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{\plotspath /ho_no_comparison/Z2-N1-Z2-N2-rp-e-HO-thesis-chapter1-170227.pdf}
\caption[Calculated ground state energy and proton radius in the ground state of {\protect $\isotope[3]{He}$} and {\protect $\isotope[4]{He}$}, obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The calculated results are extrapolated to the full space using the infrared extrapolation method.]{Calculated ground state energy (left) and proton radius in the ground state (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom), obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The dashed horizontal lines show the experimental results. The crosses connected by dotted lines are obtained by extrapolating calculated results using the infrared extrapolation method as described in the text.}
\label{fig-chap2-helium3-helium4}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (a)] and proton radius [panel (b)] of $\isotope[4]{He}$. We observe that the calculated ground state energy converges (to the $0.01$ MeV level). The extrapolated result is about $\sim 0.1$ MeV short of the experimental result ($-7.72$ MeV). The extrapolated proton radius staggers around the experimental result (at the $0.1$ fm level). However, since full convergence is not achieved we cannot assess whether the calculation correctly predicts the proton radius.



\section{Using a general single-particle basis in NCCI calculations}
\label{sec-chap2-general-basis}


In this section we review the procedure followed to derive the two-body matrix elements of the NCCI Hamiltonian in a general single-particle basis. The discussion follows closely the derivations discussed in Ref.~\cite{caprio2012:csbasis} where the two-body matrix elements of the NCCI Hamiltonian with respect to the Laguerre basis were derived. However, the discussion presented here is not limited to a particular single-particle basis. 


However, to aid the discussion we will use the Laguerre basis~\cite{caprio2012:csbasis} in the derivations. The Laguerre basis forms a complete, discrete, orthonormal set in the space of square integrable functions $\mathcal{L}^{2}(\mathbb{R}^{+})$. The Laguerre radial functions are given by
\begin{equation}
S_{nl}(b;r) = (2/b)^{-1} N_{nl} (2r/b)^{l+1} L_{n}^{2l+2} [2r/b] e^{-r/b},
\label{eqn-chap2-laguerre-radial-functions}
\end{equation}
where $n$ is the radial quantum number, $l$ is the angular momentum, $b$ is the characteristic length of the Laguerre functions, and $N_{nl}$ is a normalization given by
\begin{equation}
N_{nl} = \left( \frac{2}{b} \right)^{3/2} \left[ \frac{n!}{(n+2l+2)!} \right]^{1/2}.
\label{eqn-chap2-laguerre-normalization-coefficient}
\end{equation}
For each $l$, the Laguerre functions are orthonormal in $\mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} S_{nl}(b;r) S_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-cs-orthonormal}
\end{equation}
By replacing the harmonic oscillator radial functions $R_{nl}$ in (\ref{eqn-oscillator-orbitals-second-quantization}) with $S_{nl}$ we can form Laguerre single-particle states $| \alpha \rangle$ given by
\begin{equation}
| \alpha \rangle = \left[| S_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}}.
\label{eqn-laguerre-orbitals-second-quantization}
\end{equation}


To build the Hamiltonian matrix using a general single-particle basis we need to calculate the two-body matrix elements of the interaction and relative kinetic energy operators in the general basis. In the case where the two-body matrix elements of the interaction with respect to some single-particle basis are known, we can use a two-body transformation to obtain the two-body matrix elements in the general basis. For example, the JISP$16$ interaction is expressed in terms of the harmonic oscillator basis. Therefore, we can use a two-body transformation which will yield the two-body matrix elements in the general basis. Specifically, if $a = (n_{a}l_{a}j_{a})$ is a harmonic oscillator single-particle orbital and $\bar{a} = (\bar{n}_{a} \bar{l}_{a} \bar{j}_{a})$ is a Laguerre single-particle orbital then for antisymmetrized two-body states such as (\ref{eqn-chap2-two-particle-states-2}) the transformation is given by~\cite{hagen2006:gdm-realistic}
\begin{equation}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{AS}} = \sum_{abcd} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{AS}},
\label{eqn-chap2-two-body-interaction-transformation}
\end{equation}
where $\langle a | \bar{a} \rangle$ is an overlap bracket. For normalized antisymmetrized states such as (\ref{eqn-chap2-two-particle-states-3}) the transformation is given by
\begin{multline}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{NAS}} = (1+\delta_{\bar{a}\bar{b}})^{-1/2} (1+\delta_{\bar{c}\bar{d}})^{-1/2} \\  \sum_{abcd} (1+\delta_{ab})^{1/2} (1+\delta_{cd})^{1/2} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{NAS}}.
\label{eqn-chap2-two-body-interaction-transformation-nas}
\end{multline}
The overlap bracket is given by 
\begin{equation}
\langle a | \bar{a} \rangle = \langle R_{n_{a}l_{a}} | S_{\bar{n}_{a} \bar{l}_{a}} \rangle \delta_{(l_{a}j_{a})(\bar{l}_{a}\bar{j}_{a})}, 
\label{eqn-chap2-overlap-bracket}
\end{equation}
where 
\begin{equation}
\langle R_{nl} | S_{\bar{n}l} \rangle = \int_{0}^{\infty} dr R_{nl}(b_{\mathrm{HO}};r) S_{\bar{n}l}(b_{\mathrm{L}};r), 
\label{eqn-chap2-overlap-integral}
\end{equation}
and $b_{\mathrm{HO}}$ and $b_{\mathrm{L}}$ are the characteristic lengths of the harmonic oscillator basis and the Laguerre basis respectively. The transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) [or (\ref{eqn-chap2-two-body-interaction-transformation-nas})] involves an infinite quadruple sum over orbitals. The sum is truncated according to a one-body shell cutoff $\Ncut$ which must be selected in a way which ensures that NCCI calculations in the general basis are $\Ncut$ independent.


In principle, the two-body transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) can be used to obtain the two-body matrix elements of the relative kinetic energy operator in the general basis (provided that the matrix elements in the harmonic oscillator or other basis are known). However, in Ref.~\cite{caprio2012:csbasis} the transformation was found to yield calculated results which are highly sensitive to the $N_{\mathrm{cut}}$ truncation. Therefore, the two-body matrix elements of the relative kinetic energy operator were calculated directly in the general single-particle basis~\cite{caprio2012:csbasis}. Recall that the relative kinetic energy operator separates into one and two-body parts. Specifically, rearranging (\ref{eqn-chap2-kinetic-energy-decomposition}) we get
\begin{equation}
T_{\mathrm{rel}}  = \frac{1}{4 A m_{\mathrm{N}}} \sum_{i \neq j}^{A} (\mathbf{p}_{i}-\mathbf{p}_{j})^{2} = \frac{1}{2 A m_{\mathrm{N}}} \left[ (A-1) \sum_{i=1}^{A} p_{i}^{2} - \sum_{i \neq j}^{A} \mathbf{p}_{i} \cdot \mathbf{p}_{j} \right].
\label{eqn-chap2-kinetic-energy-decomposition-matrix-elements}
\end{equation}
The first term is a one-body operator the matrix elements of which can be calculated using the momentum space representation of the general single-particle basis. [For the Laguerre basis, the momentum space representation functions $\tilde{S}_{nl}(b;k)$, where $p = \hbar k$, are given in terms of Jacobi polynomials]. The second term is a two-body operator the matrix elements of which factorize according to Racah's reduction formula~\cite{suhonen2007:nucleons-nucleus}
\begin{equation}
\langle cd;J | \mathbf{p}_{1} \cdot \mathbf{p}_{2} | ab; J \rangle = (-1)^{j_{d}+j_{a}+J} \Gj{j_{c}}{j_{d}}{J}{j_{b}}{j_{a}}{1} \langle c || \mathbf{p}_{1} || a \rangle \langle d || \mathbf{p}_{2} || b \rangle,
\label{eqn-chap2-kinetic-energy-two-body-matrix-elements}
\end{equation}
where $\langle b || \mathbf{p} || a \rangle \propto [\int_{0}^{\infty} dk \tilde{S}_{n_{a}l_{a}}(b;k) k \tilde{S}_{n_{b}l_{b}}(b;k)] \langle l_{b} j_{b} || Y_{1} || l_{a} j_{a} \rangle$.


The suite of computer programs h$2$utils~\cite{caprio2012:csbasis} can be used for the calculation of the two-body matrix elements of the Hamiltonian in a general single-particle basis. The program calculates the two-body matrix elements of the relative kinetic energy operator and the two-body matrix elements of the interaction as separate matrices. The two matrices are then added (allowing the user to select different length parameters $b_{p}$ and $b_{n}$ for the proton and neutron spaces respectively), thus resulting in a Hamiltonian matrix which can then be used as an input to MFD which performs the many-body calculation.













==> chapters/chapter2/chapter2_draft_170307.tex <==
\chapter{INTRODUCTION TO THE NO-CORE CONFIGURATION INTERACTION APPROACH}
\label{chap-chap2}


\section{Overview}
\label{sec-chap2-overview}


In this chapter a broad overview of quantum many-body theory is presented focusing on the tools necessary to work with the no-core configuration interaction (NCCI) approach. The NCCI approach utilizes second quantization to cast the nuclear Hamiltonian into a square matrix in terms of a many-body basis. Here we describe all the steps needed to build and diagonalize the Hamiltonian matrix in some detail. Moreover, example calculations are presented and extrapolated using the infrared extrapolation method.


The general nuclear Hamiltonian for a system of $A$ nucleons interacting via two and/or three-body interactions $V(\mathbf{r}_{i},\mathbf{r}_{j})$ and $V(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k})$ respectively is given by
\begin{equation}
H = \frac{1}{2m_{\mathrm{N}}} \sum\limits_{i = 1}^{A} p_{i}^{2} + \sum_{i < j}^{A} V(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i < j < k}^{A} V_{\mathrm{NNN}}(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k}).
\label{eqn-chap2-overview-full-hamiltonian}
\end{equation}
Although three nucleon interactions are needed to accurately reproduce experimental data~\citep{pieperqmc:2008}, two-body interactions  provide a simpler context in which to focus on the main goal of this thesis, which is to introduce an alternative single-particle basis (other than the traditional harmonic oscillator basis) for NCCI calculations. Thus for the purpose of this thesis, we omit three-body terms from the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}).


Moreover, for reasons that have to do with the center-of-mass degree of freedom (described in Sec.~\ref{sec-chap2-com-factorization}) in the NCCI approach we do not work with the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}). Instead, we work with the translationally invariant intrinsic Hamiltonian \citep{vanhees:1983,lipkin:1958}
\begin{equation}
H_{\mathrm{in}} = T_{\mathrm{rel}} + V = \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}} 
+ \sum_{i < j}^{A} V_{\mathrm{NN}}(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i < j}^{Z} V_{\mathrm{C}}(\mathbf{r}_{i},\mathbf{r}_{j}) ,
\label{eqn-chap2-overview-hamiltonian}
\end{equation}
where $m_{\mathrm{N}} c^{2} = 938.92$ MeV is the average nucleon mass, $V_{\mathrm{NN}}$ is the internucleon interaction, and $V_{\mathrm{C}}$ is the Coulomb interaction. 


We start with a brief summary of second quantization (Sec.~\ref{sec-chap2-second-quantization}) which is then used to derive the two-body matrix elements of the NCCI Hamiltonian (Sec.~\ref{sec-chap2-tbme}). Consequently, we discuss the harmonic oscillator single-particle radial functions (Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}) and the nuclear many-body basis (Sec.~\ref{sec-chap2-many-body-basis}). The complete factorization of the center-of-mass and intrinsic portions of the many-body wave function (Sec.~\ref{sec-chap2-com-factorization}) and a description of the procedure followed to perform many-body calculations using the NCCI approach (Sec.~\ref{sec-chap2-many-body-calculations}) follow. The one-body density matrix and its properties are reviewed (Sec.~\ref{sec-chap2-one-body-density-matrix}). Example calculations for the nuclei $\isotope[3]{He}$ and $\isotope[4]{He}$ are presented, and the calculated results are extrapolated using the infrared extrapolation method (Sec.~\ref{sec-chap2-example-calculations}). We conclude this Chapter with an overview of the steps needed to perform an NCCI calculation using a general single-particle basis (Sec.~\ref{sec-chap2-general-basis}).


\section{Second quantization}
\label{sec-chap2-second-quantization}


Second quantization is used to describe systems of many identical particles. In what follows the notational conventions of Negele are used~\cite{negele1988:many-particle}.


The Hilbert space of $A$ distinguishable particles $ \mathcal{H}^{A}$ is spanned by the tensor product of $A$ distinguishable particles occupying single-particle states which belong to the single-particle Hilbert space $\mathcal{H}$ 
\begin{equation}
\mathcal{H}^{A} = \mathcal{H} \otimes \mathcal{H} \otimes \ldots \otimes \mathcal{H}.
\label{eqn-chap2-hilbert-space-product}
\end{equation}
If $\left\{ | a \rangle \right\}$ is an orthonormal basis for $\mathcal{H}$, an orthonormal basis for $\mathcal{H}^{A}$ can be constructed as the set of tensor product states
\begin{equation}
| a_{1} \ldots a_{A} ) \equiv |a_{1} \rangle \otimes |a_{2} \rangle \otimes \ldots \otimes |a_{A} \rangle,
\label{eqn-chap2-many-body-basis-product}
\end{equation}
where the curved parenthesis on the left hand side of (\ref{eqn-chap2-many-body-basis-product}) denotes that the many-body state is a simple product of single-particle states (i.e., no assumptions are made about the symmetry of the many-body state). 


The space of $A$ indistinguishable fermions $\mathcal{F}^{A}$ is spanned by fully antisymmetric many-body states constructed using the many-body states of $\mathcal{H}^{A}$  
\begin{equation}
| a_{1} \ldots a_{A} \rangle = \frac{1}{\sqrt{A!}} \sum_{P} (-1)^{P} | a_{P_{1}} \rangle \otimes | a_{P_{2}} \rangle \otimes \ldots \otimes | a_{P_{A}} \rangle.
\label{eqn-chap2-many-body-basis-antisymmetric}
\end{equation} 
The sum over $P$ is a sum over all possible permutations $(P_{1},\,P_{2},\ldots,P_{A})$ of the set $(a_{1},\,a_{2},\,\ldots, a_{A})$. Moreover, $(-1)^{P}$ is determined by counting the number of transpositions of two elements which brings a permutation to its original form $(a_{1},\,a_{2},\,\ldots, a_{A})$. 


The Fock space $F$ for fermions is the (Hilbert) direct sum of the fermion spaces $\mathcal{F}^{0}$, $\mathcal{F}^{1}$, $\mathcal{F}^{2}$, $\ldots$, $\mathcal{F}^{A}$, $\ldots$ for zero, one, two, etc particles
\begin{equation}
F = \mathcal{F}^{0} \oplus \mathcal{F}^{1} \oplus \mathcal{F}^{2} \oplus \ldots \oplus \mathcal{F}^{A} \oplus \ldots.
\label{eqn-chap2-fock-space}
\end{equation}
Here $\mathcal{F}^{0}$ is the space of no particles, $\mathcal{F}^{1}$ is identical to $\mathcal{H}$, and $\mathcal{F}^{A}$ with $A \geq 2$ is the space spanned by many-body states given by (\ref{eqn-chap2-many-body-basis-antisymmetric}).


Creation and annihilation operators generate the entire Fock space $F$ by adding (removing) single-particle states to (from) many-body states. The fermionic creation operator $c_{a}^{\dagger}$ adds a particle in a single-particle state $| a \rangle$ to the many-body state $| a_{1} \ldots a_{A} \rangle$ as follows
\begin{equation}
c_{a}^{\dagger} | a_{1} a_{2} \ldots a_{A} \rangle = | a a_{1} a_{2} \ldots a_{A} \rangle,
\label{eqn-chap2-creation-operator}
\end{equation}
where the definition implies that the particle is added to the left of the initial many-body state. Now, because of the antisymmetry requirement for fermions we cannot act with the $c_{a}^{\dagger}$ operator on the state $| a a_{1} a_{2} \ldots a_{A} \rangle$ (and thus add the single-particle state $| a \rangle$ twice). This state is equal to zero by definition
\begin{equation}
c_{a}^{\dagger} |a a_{1} a_{2} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-creation-operator-2}
\end{equation}
Similarly an annihilation operator $c_{a}$ removes a particle occupying the single-particle state $|a\rangle$ from a many-body state
\begin{equation}
c_{a} |a a_{1} \ldots a_{A} \rangle = | a_{1} \ldots a_{A} \rangle.
\label{eqn-chap2-annihilation-operator}
\end{equation}
For completeness, note that in general $c_{a} | a_{1} a_{2} \ldots a \ldots a_{A} \rangle = (-1)^{P} | a_{1} a_{2} \ldots a_{A} \rangle$ where $P$ is the number of transpositions of two elements needed to bring the particle in the single-particle state $| a \rangle$ to the front of the many-body state. For example $c_{a_{2}} | a_{1} a_{2} a_{3} \rangle = - |a_{1} a_{3} \rangle$. If $c_{a}$ acts on a state $| a_{1} \ldots a_{A} \rangle$, i.e., a state which has no particle in the single-particle state $| a \rangle$, then the action of $c_{a}$ on the many-body state $| a_{1} \ldots a_{A} \rangle$ yields zero
\begin{equation}
c_{a} |a_{1} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-annihilation-operator-2}
\end{equation}
Following from~(\ref{eqn-chap2-creation-operator})-(\ref{eqn-chap2-annihilation-operator-2}), we conclude that the creation and annihilation operators obey the fermionic anticommutation relation
\begin{equation}
\lbrace c_{a} , c_{b}^{\dagger} \rbrace = \delta_{ab}.
\label{eqn-chap2-anti-commutation}
\end{equation}


One-body operators are operators which can be written as a sum of single-particle operators acting on one particle at a time. To be able to calculate the matrix elements of one-body operators with respect to many body states like (\ref{eqn-chap2-many-body-basis-antisymmetric}), it is useful to express them in terms of creation and annihilation operators. To arrive at this expression, let us first use the many-body states of $\mathcal{H}^{A}$ to calculate the matrix elements of a one-body operator $T = \sum_{i=1}^{A} t_{i}$. For the diagonal matrix elements (i.e., between the same many-body states) we have
\begin{multline}
( a_{1}a_{2} \ldots a_{A} | T | a_{1} a_{2} \ldots a_{A} ) = \\  
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2} \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \\
\langle a_{1} | t_{1} | a_{1} \rangle + \ldots + \langle a_{A} | t_{A} | a_{A} \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-identical-states}
\end{multline}
where we used the fact that the single-particle states are orthonormal hence $\langle a_{i} | a_{j} \rangle = \delta_{ij}$. Let us now evaluate the non-diagonal matrix elements of $T$ starting with the matrix elements between the many-body state $ | a_{1} a_{2} \ldots a_{A} )$ and the many-body state $ | a_{1} a_{2}' \ldots a_{A} )$, where $| a_{2} \rangle \neq | a_{2}' \rangle$. We have
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1} a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \langle a_{1} | a_{1} \rangle \langle a_{2} | t_{2} | a_{2}' \rangle \langle a_{3} | a_{3} \rangle \ldots \langle a_{A} | a_{A} \rangle + \\
+ \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \langle a_{2} | t_{2} | a_{2}' \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-one-sp-state-different}
\end{multline}
since $\langle a_{2} | a_{2}' \rangle = 0 $. Finally, the matrix elements of $T$ between the many-body states $| a_{1} a_{2} \ldots a_{A} )$ and $| a_{1}' a_{2}' \ldots a_{A} )$, where $| a_{1} \rangle \neq | a_{1}' \rangle$ and $| a_{2} \rangle \neq | a_{2}' \rangle$, are
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1}' a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1}' \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1}' \rangle \ldots \langle a_{A} | t_{A} | a_{A} \rangle = 0.
\label{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}
\end{multline}
Thus, the matrix elements of the one-body operator $T$ with respect to many-body states of $\mathcal{H}^{A}$ are fully defined by the sum over single-particle matrix elements of $\mathcal{H}$. If we now define the single-particle vacuum state $| - \rangle$ (i.e., a non-occupied single-particle state), then $c_{a}^{\dagger} | - \rangle = | a \rangle$. Using this definition and (\ref{eqn-chap2-one-body-operator-matrix-elements-identical-states})-(\ref{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}) we can write a one-body operator as
\begin{equation}
T = \sum_{ab} t_{ab} c_{a}^{\dagger} c_{b},
\label{eqn-chap2-one-body-operator-second-quantization}
\end{equation}
where $t_{ab} = \langle a | t | b \rangle$.

Similarly, the matrix elements of a two-body operator $V = \frac{1}{2} \sum_{i \neq j} u_{ij}$ with respect to the many-body states of $ \mathcal{H}^{A}$ are fully defined by the matrix elements $u_{abcd} = (ab | u | cd )$ calculated using the states of $\mathcal{H}^{2}$. Thus we can write $V$ as
\begin{equation}
V = \frac{1}{2} \sum_{abcd} u_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c}.
\label{eqn-chap2-interaction-second-quantized}
\end{equation}
However, it is more convenient to write the two-body operator as
\begin{equation}
V = \frac{1}{4} \sum_{abcd} \bar{u}_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c},
\label{eqn-chap2-interaction-second-quantized-antisymmetrized}
\end{equation}
where $\bar{u}_{abcd} = u_{abcd} - u_{abdc} = \langle ab | u | cd \rangle$ are normalized and antisymmetrized two-body matrix elements.


\section{Two-body matrix elements for the NCCI Hamiltonian}
\label{sec-chap2-tbme}

In the context of the NCCI approach, the most commonly used single-particle states are the harmonic oscillator single-particle basis states (see Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}). A harmonic oscillator single-particle state is labeled by the quantum numbers $| \alpha \rangle \equiv |n_{a}l_{a}j_{a}m_{a} \rangle$, where $n_{a}$ is the harmonic oscillator radial quantum number, $l_{a}$ is the angular momentum, $j_{a}$ is the total angular momentum, and $m_{a}$ is the $z$ projection of the total angular momentum. Using the harmonic oscillator single-particle states we can construct fully antisymmetric many-body basis states for the NCCI approach
\begin{equation}
| (n_{a}l_{a}j_{a}m_{a}) (n_{b}l_{b}j_{b}m_{b}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle.
\label{eqn-chap2-many-body-state-harmonic-oscillator}
\end{equation} 
Many-body states such as (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) have a total $z$ projection of total angular momentum $M=\sum_{i=1}^{A} m_{i}$ and a total number of oscillator quanta $N_{\mathrm{tot}}=\sum_{i=1}^{A} (2n_{i} + l_{i}) = \sum_{i=1}^{A} N_{i}$. The harmonic oscillator single-particle states $| \alpha \rangle$ are given as the tensor product 
\begin{equation}
| \alpha \rangle = \left[| R_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}},
\label{eqn-oscillator-orbitals-second-quantization}
\end{equation}
where $R_{n_{a}l_{a}}$ is a harmonic oscillator radial function, $Y_{l_{a}}$ is a spherical harmonic, and $|\frac{1}{2} \rangle$ is a spinor. The subscripts $j_{a}$ and $m_{a}$ indicate that $| R_{n_{a} l_{a}} Y_{l_{a}} \rangle$ (a spherical tensor of rank $l_{a}$) and the spinor $| \frac{1}{2} \rangle$ are coupled to total angular momentum $j_{a}$ and $z$ projection of total angular momentum $m_{a}$~\cite{rose1957:am}. 


The Hilbert space of the NCCI Hamiltonian is spanned by the many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) which provide a basis for the representation of the Hamiltonian as a square matrix. To cast the Hamiltonian into a square matrix we must first calculate the two-body matrix elements of the relative kinetic energy and two-body $NN$ interaction operators. The two-body matrix elements are calculated with respect to two-particle states, coupled to total angular momentum $J$. For distinguishable particles (e.g., one proton and one neutron states), angular momentum coupled two-particle states are defined as 
\begin{equation}
| a b ; J ) = \sum_{m_{a}m_{b}} \langle j_{a} m_{a} j_{b} m_{b} | J M \rangle |a m_{a} \rangle | b m_{b} \rangle,
\label{eqn-chap2-two-particle-states-1}
\end{equation}
where $| a m_{a} \rangle = | n_{a} l_{a} j_{a} m_{a} \rangle$, $\langle j_{a} m_{a} j_{b} m_{b} | J M \rangle $ is a Clebsch-Gordan coefficient, and the parenthesis implies that the two-particle state is not antisymmetrized. For two identical fermions we can obtain fully antisymmetrized states using the states $| a b ; J )$. We have
\begin{equation}
| a b ; J M \rangle_{\mathrm{AS}} = \frac{1}{\sqrt{2}} \left[ | a b ; J M ) - (-1)^{J - j_{a} - j_{b}} | b a ; J M \rangle \right].
\label{eqn-chap2-two-particle-states-2}
\end{equation}
These states have the symmetry property $| a b ; J M \rangle = - (-1)^{J -j_{a}-j_{b}} | b a ; J M \rangle$ which implies that if the states $| a \rangle$ and $| b \rangle$ are identical, only two-body states with even $J$ are allowed. The states (\ref{eqn-chap2-two-particle-states-2}) are antisymmetrized but not strictly normalized. An extra factor of $1 / \sqrt{2}$ is required for normalization in the special case when the two particles occupy the same single-particle orbital $| n_{a} l_{a} j_{a} \rangle$. Hence, the appropriate two-particle states are
\begin{equation}
| a b ; J M \rangle_{\mathrm{NAS}} = (1 + \delta_{ab})^{-1/2} | a b ; J M \rangle_{\mathrm{AS}}.
\label{eqn-chap2-two-particle-states-3}
\end{equation}
Both the normalized antisymmetrized states and the antisymmetrized states are used to calculate the two-body matrix elements $\langle c d ; J | H_{\mathrm{in}} | a b ; J \rangle$ of the (scalar) intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}). The change of basis relation between two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-2}) and two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-3}) is
\begin{equation}
\langle c d ; J | H | a b ; J \rangle_{\mathrm{NAS}} = (1+\delta_{cd})^{-1/2} (1+\delta_{ab})^{-1/2} \langle c d ; J | H | a b ; J \rangle_{\mathrm{AS}}.
\label{eqn-chap2-nas-two-body-matrix-elements}
\end{equation}
A detailed discussion about the calculation of the two-body matrix elements of the intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) is given in Ref.~\cite{caprio2012:csbasis}. A brief overview is also given in Sec.~\ref{sec-chap2-general-basis}.
 

\section{The harmonic oscillator single-particle states}
\label{sec-chap2-harmonic-oscillator-radial-functions}


In this section we will review the basic properties of the harmonic oscillator single-particle states $| \alpha \rangle$~\cite{suhonen2007:nucleons-nucleus,moshinsky1996:oscillator,weniger1985:fourier-plane-wave} which are traditionally used in the NCCI approach because their properties facilitate the many-body calculations. The harmonic oscillator single-particle states are also our starting basis for the construction of natural orbitals which are introduced in Chapter~\ref{chap-chap3}. 


The first important property of the harmonic oscillator single-particle states (relevant to the NCCI approach) is that they allow for the complete removal of spurious center-of-mass states from the low-lying spectrum of the NCCI Hamiltonian provided that an $\Nmax$ truncation is imposed on the many-body basis. The appearance of spurious center-of-mass states results from using the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) for the representation of the NCCI Hamiltonian as a square matrix. A detailed discussion about the appearance of spurious center-of-mass states in an NCCI calculation and the procedure followed for their removal from the low-lying spectrum is given in Sec.~\ref{sec-chap2-many-body-basis}.

The second important property of the harmonic oscillator single-particle states (relevant to many-body calculations and consequently the NCCI approach) is that they simplify the calculation of two-body matrix elements for operators written in terms of relative coordinates, using the Moshinsky transformation~\citep{moshinsky1996:oscillator}. According to  the transformation, products of harmonic oscillator states expressed in single-particle coordinates $R_{n_{1}l_{1}}(\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ transform into products of harmonic oscillator states expressed in terms of relative and center-of mass coordinates $R_{nl}(\mathbf{r}_{\mathrm{rel}})R_{NL}(\mathbf{R})$, where $2 n_{1} + l_{1} + 2 n_{2} + l_{2}= 2 n + l+ 2 N + L$, $\mathbf{r}_{\mathrm{rel}} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}-\mathbf{r}_{2})$, and $\mathbf{R} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}+\mathbf{r}_{2})$. (The factor of $1/\sqrt{2}$ in front of the center-of-mass vector is used instead of the traditional $1/2$ for normalization reasons). The calculation of two-body matrix elements for operators of the form $V(\mathbf{r}_{1}-\mathbf{r}_{2})$ with respect to two-particle states of the form $R_{n_{1}l_{1}} (\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ is then reduced to the calculation of the single-particle matrix element of the operator $V(\mathbf{r}_{\mathrm{rel}})$ with respect to single-particle states of the form $R_{nl}(\mathbf{r}_{\mathrm{rel}})$ and an overlap between single-particle states of the form $R_{NL}(\mathbf{R})$.

Let us now review the harmonic oscillator radial wave functions. If we write the single-particle wave function as $\Psi_{nlm}(\mathbf{r})=r^{-1} R_{nl}(b;r)Y_{lm}(\theta,\phi)$, where $R_{nl}(b;r)$ are radial wave functions and $Y_{lm}(\theta,\phi)$ are spherical harmonics, then $\Psi_{nlm}(\mathbf{r})$ are solutions to the familiar harmonic oscillator central force problem \cite{suhonen2007:nucleons-nucleus} 
\begin{equation}
h(\omega) = \frac{p^{2}}{2m_{\mathrm{N}}} + \frac{m_{\mathrm{N}} \omega^{2} r^{2}}{2}.
\label{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}
\end{equation} 
where $m_{\mathrm{N}}c^{2} \approx 938.92$ MeV is the average nucleon mass and $\omega$ is the oscillator frequency. The length scale of the radial functions $R_{nl}(b;r)$ is set by the oscillator length $b$ which depends on the parameters of the oscillator Hamiltonian (\ref{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}) as $b=\sqrt{\hbar / (m_{\mathrm{N}} \omega})$. The eigenvalues corresponding to each single-particle radial wave function are given by $ (N + 3/2) \hw$, where $N = 2n + l$ is the oscillator quantum (notice that the eigenvalues are evenly spaced by one unit of $\hw$). The radial functions $R_{nl}(b;r)$ are given by
\begin{equation}
R_{nl}(b;r) = b N_{nl} (r/b)^{l+1} L_{n}^{l+1/2}[(r/b)^{2}] e^{-(r/b)^{2}/2},
\label{eqn-chap2-harmonic-oscillator-radial-functions}
\end{equation} 
where $L_{n}^{l+1/2}[(r/b)^{2}]$ are generalized Laguerre polynomials, $n$ is the radial quantum number (which gives the number of nodes in the radial function), $l$ is the angular momentum, and $N_{nl}$ is a normalization factor given by
\begin{equation}
N_{nl} = \frac{1}{b^{3/2}} \left[ \frac{2n!}{(l+n+1/2)!} \right]^{1/2}.
\label{eqn-chap2-harmonic-oscillator-functions-normalization}
\end{equation}
For each $l$, the harmonic oscillator radial functions form a complete discrete basis for square integrable functions on $ \mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} R_{nl}(b;r) R_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-ho-orthonormal}
\end{equation}
 

\section{Symmetries of the NCCI Hamiltonian and the nuclear \\ many-body basis}
\label{sec-chap2-many-body-basis}


The selection of the nuclear many-body basis used in NCCI calculations is based on the symmetries of the NCCI Hamiltonian~(\ref{eqn-chap2-overview-hamiltonian}). The NCCI Hamiltonian is rotationally invariant therefore it conserves the total angular momentum $J$ and the $z$ projection of total angular momentum $M$. Moreover, the Hamiltonian conserves parity. To diagonalize the Hamiltonian we can choose to use many-body states that have good $J$ (a $J$-scheme basis) or many-body states that have good $M$ (an $M$-scheme basis)~\cite{whitehead1977:shell-methods}. Although the $M$-scheme basis involves a larger number of many-body basis states compared to a $J$-scheme basis, constructing $M$-scheme many-body basis states is straightforward (i.e., we do not have to deal with angular momentum coupling as in the $J$-scheme basis). Therefore, for the NCCI calculations discussed here, an $M$-scheme basis is considered. However, the eigenstates of $H$ still have good $J$ which is recovered after diagonalization by calculating the expectation value of the $J^{2}$ operator with respect to the calculated many-body wave function.


To build many-body basis states we start from single-particle states $| nljm \rangle$ and construct fully antisymmetric states (with good $M$) given by~(\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Calculations can be performed for any possible value of $M$ (which is supported by the single-particle states in the many-body basis). For example, for even nuclei $M=0, 1,\ldots$ and for odd nuclei $M=1/2, 3/2, \ldots$ (we do not consider negative values for $M$ here). However, we usually use many-body states with $M=0$ for even nuclei and $M=1/2$ for odd nuclei. This is because for a given $M$ we can only obtain many-body wave functions with $J \geq | M |$. Thus, choosing the lowest possible $M$ allows us to study the ground and first few excited states of a nucleus.


Commonly, for reasons involving the center-of-mass degree of freedom, as discussed in Sec.~\ref{sec-chap2-com-factorization}, the many-body basis is truncated using the $\Nmax$ truncation scheme~\cite{elliott1955:com-shell}. The scheme dictates that only many-body states with $\Ntot \leq N_{0} + \Nmax$ are permitted in the many-body basis, where $N_{0}$ is the number of quanta in the configuration where all the nucleons occupy the lowest permitted oscillator shells. For example, $N_{0}=2$ for $\isotope[6]{He}$ (in this configuration, the two protons occupy the $N=0$ proton shell, two neutrons occupy the $N=0$ neutron shell, and the last two neutrons occupy the $N=1$ shell) and $N_{0} =3$ for $\isotope[7]{Li}$ (because the extra proton compared to $\isotope[6]{He}$ goes into the $N=1$ proton shell). 




Finally, because the nuclear Hamiltonian conserves parity we want our many-body basis to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. A many-body basis truncated at a given $\Nmax$ contains (many-body) states with $N_{\mathrm{tot}} \leq N_{0} + \Nmax$, where $N_{\mathrm{tot}} = \sum_{i} N_{i} = N_{1} + \ldots + N_{A}$, and $N_{i}$ is the oscillator quantum of a nucleon $i$ in its single-particle state. Hence, many-body basis states which belong to this (many-body) basis have parity which is obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the many-body states of the lowest allowed configuration is $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity eigenstates of the nucleus we must build many-body bases with even $\Nmax$ truncations, i.e., $\Nmax = 0, 2, 4, ldots$. On the other hand, to obtain the unnatural parity eigenstates of the nucleus we must construct many-body bases with odd $\Nmax$ truncations, i.e., $\Nmax = 1, 3, 5, \ldots$. 

%Finally, because the nuclear Hamiltonian conserves parity we want our many-body basis to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. This means that the parity of a many-body state which belongs to the many-body basis can be obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the lowest possible configuration is given by $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity states of the nucleus $\Nmax$ must be even and proceed in steps of $2$, i.e., $\Nmax = 2, 4, 6, \ldots$. On the other hand, to obtain the unnatural parity states of the nucleus $\Nmax$ must be odd and also proceed in steps of $2$, i.e., $\Nmax = 1, 3, 5, \ldots$. 






\section{Spurious center-of-mass states removal}
\label{sec-chap2-com-factorization}


In this section we describe how spurious center-of-mass states result from the diagonalization of the NCCI Hamiltonian matrix built in terms of the set of the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Subsequently, we describe how these spurious states can be removed provided that the $\Nmax$ truncation scheme is used.

The many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) are defined with respect to a fixed point in space. However, physically there is no such point around which all the nucleons are orbiting. Rather we are interested in the internal motion of the nucleons relative to each other within the nucleus, a motion which defines the intrinsic structure of the nucleus.


In principle we can convert to relative coordinates. However, antisymmetrization in Jacobi coordinates (which define the relative motion) is cumbersome. Therefore, we are compelled to work in the full coordinate space which includes both the center of mass and relative degrees of freedom.


Our goal is to describe the relative motion as accurately as possible without unnecessary complications arising from the center of mass motion. In order to accomplish this it helps making certain choices regarding the basis and the Hamiltonian.


We want our eigenfunctions to factorize into center of mass and relative factors. We also want the center of mass factor to be simple and well understood so that it does not interfere with the calculation of energies and observables. In principle, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) is already separated into center of mass and relative coordinates. If we define the center-of-mass momentum as $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, the one-body kinetic energy operator in (\ref{eqn-chap2-overview-full-hamiltonian}) can be decomposed into a center-of-mass and a relative kinetic energy contributions~\cite{vanhees:1983}
\begin{equation}
T = T_{\mathrm{c.m.}} + T_{\mathrm{rel}} = \frac{\left(\sum\limits_{i=1}^{A}\mathbf{p}_{i}\right)^{2}}{2Am_{\mathrm{N}}}  + \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}}.
\label{eqn-chap2-kinetic-energy-decomposition}
\end{equation}
Therefore, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) also separates into center-of-mass and relative parts
\begin{equation}
H= T_{\mathrm{c.m.}} + (T_{\mathrm{rel}} + V).
\label{eqn-chap2-full-separated-hamiltonian}
\end{equation}
Thus, in the full space our eigenfunctions would factorize into a center-of-mass and a relative wave function.

However, we are confined to work in a truncated space. Factorization can still be exact in an oscillator basis when the $\Nmax$ truncation is used. The truncated space then only contains a limited center-of-mass space spanned by center-of-mass harmonic oscillator states with $N_{\mathrm{c.m.}} = 0$, $2$, $\ldots, \Nmax$. We could attempt to diagonalize the Hamiltonian~(\ref{eqn-chap2-full-separated-hamiltonian}) in the truncated space. However, the $T_{\mathrm{c.m.}}$ operator will mix contributions with different center-of-mass excitations $N_{\mathrm{c.m.}}$ and destroy factorization of the eigenfunctions. The Hamiltonian will force us towards states which attempt to diagonalize the center-of-mass kinetic energy operator $T_{\mathrm{c.m.}}$. Therefore, our NCCI calculations would end up approximating spherical waves in the center of mass coordinates, at the expense of accurately describing the intrinsic motion.

Thus, instead, we choose to work with the intrinsic Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V.
\end{equation} 
The resulting Hamiltonian is block diagonal with respect to the number of quanta $N_{\mathrm{c.m.}}$ for the center-of-mass motion. The resulting eigenfunctions will factorize into a center-of-mass factor of good $N_{\mathrm{c.m.}}$ and an intrinsic factor. The total number of quanta in a many-body state is shared between the center-of-mass motion and the intrinsic motion:
\begin{equation}
\Ntot = \sum_{i} N_{i} = N_{\mathrm{c.m.}} + N_{\mathrm{rel}}.
\label{eqn-chap2-number-of-quanta-com-quanta}
\end{equation}
Therefore, in eigenfunctions with $N_{\mathrm{c.m.}} = 0$, the full $\Nmax$ quanta are available to use in describing the intrinsic motion. The higher $N_{\mathrm{c.m.}}$ eigenfunctions produce spurious copies of the spectrum in which the intrinsic motion is described using fewer quanta $N_{\mathrm{rel}} \leq \Nmax - N_{\mathrm{c.m.}}$. 


It is convenient to push the spurious excited center-of-mass states out of the low lying spectrum. We do this by adding a term diagonal in the number of center-of-mass quanta. That is we add a ``Lawson term''~\cite{gloeckner1974:spurious-com} proportional to the $N_{\mathrm{c.m.}}$ operator. This is often equivalently described as adding a center-of-mass harmonic oscillator Hamiltonian. In terms of the center-of-mass coordinate $\mathbf{R} = (\sum_{i} \mathbf{r}_{i})/A$ and the center-of-mass momentum $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, 
\begin{equation}
H_{\mathrm{c.m.}} = \frac{P^{2}}{2Am_{\mathrm{N}}} + \frac{1}{2} A m_{\mathrm{N}} \omega^{2} R^{2}.
\label{eqn-chap2-harmonic-oscillator-many-body-hamiltonian-com}
\end{equation}
Then, $H_{\mathrm{c.m.}} = (N_{\mathrm{c.m.}} + 3/2)\hbar \omega$. Thus we actually diagonalize the Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V + \alpha N_{\mathrm{c.m.}},
\label{eqn-chap2-ncci-hamiltonian-with-lawson}
\end{equation} 
where $\alpha$ is the Lawson term strength (typically a few MeV). This leads to the same eigenstates as the relative Hamiltonian but with the spurious states lifted out of the low-lying spectrum by an amount $\alpha N_{\mathrm{c.m.}}$.




\section{Many-body calculations}
\label{sec-chap2-many-body-calculations}


In this section we will briefly describe the general procedure followed to obtain results using the NCCI approach.

The basic ingredient needed to build the Hamiltonian matrix is the two-body matrix elements of the NCCI Hamiltonian (\ref{eqn-chap2-ncci-hamiltonian-with-lawson}) with respect to many-body basis states like (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Thus, we need to evaluate matrix elements of the form
\begin{equation}
\langle \Phi_{n} | H | \Phi_{m} \rangle,
\label{eqn-chap2-two-body-matrix-elements}
\end{equation}
where $| \Phi_{n} \rangle = | (n_{1}l_{1}j_{1}m_{1}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle$ is a many-body basis state. [The matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) reduce to a sum over two-body matrix elements of the form $\langle c d ; J | H | a b ; J \rangle$ using Wick's theorem]. After calculating the matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) for all the many-body states in our basis we obtain the Hamiltonian matrix
\begin{equation}
  \begin{pmatrix}
    \langle \Phi_{1} | H | \Phi_{1} \rangle & \langle \Phi_{1} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{1} | H | \Phi_{m} \rangle \\
    \langle \Phi_{2} | H | \Phi_{1} \rangle & \langle \Phi_{2} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{2} | H | \Phi_{m} \rangle \\
    \vdots & \vdots & \ddots & \vdots \\
   \langle \Phi_{d} | H | \Phi_{1} \rangle & \langle \Phi_{d} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{d} | H | \Phi_{d} \rangle
  \end{pmatrix}
\label{eqn-chap2-ncci-hamiltonian-matrix}
\end{equation}
The dimension $d$ of the matrix (\ref{eqn-chap2-ncci-hamiltonian-matrix}) is equal to the number of many-body basis states for a given nucleus and $\Nmax$ truncation (see Fig.~\ref{fig-chap1-NNCI-dimension}). Diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}) yields the nuclear many-body wave function
\begin{equation}
| \Psi \rangle = \sum\limits_{n=1}^{d} c_{n} | \Phi_{n} \rangle.
\label{eqn-chap2-ncci-wave-functions}
\end{equation}
%where $c_{n}$ are coefficients obtained from the diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}).


The diagonalization of the Hamiltonian matrix is commonly performed using the Lanczos algorithm~\cite{komzsik2003:lanczos-method,lanczos1950:algorithm}. The algorithm transforms the generally large sparse matrix (\ref{eqn-chap2-ncci-wave-functions}) into a tridiagonal matrix (of lower dimension than the original matrix). The tridiagonal matrix is then diagonalized (using an appropriate algorithm) and the eigenvalues and eigenvectors (of the tridiagonal matrix) are obtained. The eigenvectors of the tridiagonal matrix (Lanczos vectors) must then be converted from the Lanczos vector space to the original many-body basis. The process established by Lanczos proceeds as follows: If $H$ is a Hamiltonian matrix of order $n$ (i.e., the matrix dimension is $n \times n$), then we start with a random initial vector $b_{0}$ which is used to construct $m$ vectors (orthogonal to each other) according to the algorithm
\begin{align}
b_{0} & = \mathrm{random}, \nonumber & \\
b_{1} & = (H - \alpha_{0}) b_{0}, \nonumber \\
b_{2} & = (H - \alpha_{1}) b_{1} - \beta_{0} b_{0}, \nonumber \\
b_{3} & = (H - \alpha_{2}) b_{2} -\beta_{1} b_{1}, \nonumber \\
 \vdots  \nonumber & \\
b_{m} & = (H - \alpha_{m-1}) b_{m-1} - \beta_{m-2} b_{m-2} = 0,
\label{eqn-chap2-lanczos-algorithm}
\end{align}
where $m \leq n$. The equality to zero in the last step means the end of the process. The coefficients $\alpha_{m-1}$ and $\beta_{m-2}$ are determined by requiring that the norm of the vector $\parallel b_{m} \parallel$ is minimized. The coefficients are then used to build the tridiagonal matrix 
\begin{equation}
T =  \begin{pmatrix}
\alpha_{0} & \beta_{0} &   &   & 0\\ 
\beta_{0}  & \alpha_{1} & \beta_{1} & \\
                 & \ddots & \ddots & \ddots & \\
                 &  & \beta_{k-2} & \alpha_{k-1} &\beta_{k-1} \\
           0      & & & \beta_{k-1} & \alpha_{k}
  \end{pmatrix}
\label{eqn-chap2-tridiagonal-matrix}
\end{equation}
The eigenvalues of $T$ converge to the eigenvalues of $H$ provided that a sufficient number of iterations $k$, where $k < n$, is performed. 


The generally large sizes of the NCCI Hamiltonian matrices require the use of parallel computing which handles both the storage and the diagonalization of the Hamiltonian matrix. For the calculations presented in this thesis, we use the parallel code Many Fermion Dynamics-Nuclear (MFDn) \cite{maris2010:ncsm-mfdn-iccs10,vary2009:ncsm-mfdn-scidac09} developed by the Iowa State University group handles the construction of the many-body basis, the construction of the Hamiltonian matrix, the storage of the matrix over multiple cores, and the Lanczos diagonalization of the matrix. The input to the code includes the two-body matrix elements of the Hamiltonian, the $\Nmax$ truncation of the many-body basis, the number of protons ($Z$) and neutrons ($N$) of the nucleus we want to study, the number of Lanczos iterations we want to perform, and various other control parameters. The program outputs the eigenvalues (which are the nuclear level energies), the one-body density matrices (described in Sec.~\ref{sec-chap2-one-body-density-matrix}), and other observables.


\section{The one-body density matrix}
\label{sec-chap2-one-body-density-matrix}


The one-body density matrix can be calculated using the many-body wave functions obtained in a many-body calculation. It is more frequently used for the calculation of the matrix elements of one-body operators~\cite{suhonen2007:nucleons-nucleus}. Moreover, the static one-body density matrix contains information about correlations in the many-body wave function as described below. In second quantization, the transition one-body density matrix is given by
\begin{equation}
\rho_{\alpha\beta}^{\mathrm{f\,i}} = \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger} c_{\beta} | \Psi_{\mathrm{i}} \rangle,
\label{eqn-chap2-one-body-density-operator}
\end{equation}
where $| \Psi_{\mathrm{i}} \rangle$ and $| \Psi_{\mathrm{f}} \rangle$ are the many-body wave functions of an initial and a final nuclear state respectively. Using (\ref{eqn-chap2-one-body-density-operator}), the matrix elements of a one-body operator $\mathcal{O}$ are obtained as
\begin{equation}
\langle \Psi_{\mathrm{f}} | \mathcal{O} | \Psi_{\mathrm{i}} \rangle =  \sum_{\alpha\beta} \langle \alpha | \mathcal{O} | \beta \rangle \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger}c_{\beta} | \Psi_{\mathrm{i}} \rangle.
\label{eqn-chap2-one-body-operator-matrix-elements}
\end{equation}


The static one-body density matrix (i.e., the one-body density matrix obtained for the same initial and final many-body wave functions) contains information about correlations in the many-body wave function. By definition, an uncorrelated many-body wave function can be written as a single Slater determinant, i.e., $| \Psi \rangle = | a_{1} \ldots a_{A} \rangle$. For an uncorrelated many-body wave function, it is easy to see that the diagonal matrix elements $\rho_{\alpha\alpha} = \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle $ are equal to $1$ (which reflects the fact that each single-particle state is occupied by exactly one nucleon), while all the off diagonal matrix elements $\rho_{\alpha\beta}$ are equal to $0$. The sum of the diagonal matrix elements is equal to the total number of nucleons $A$ in the many-body wave function. In the case of a correlated many-body wave function, such as the ones calculated in an NCCI calculation, the one-body density matrix is not (in general) diagonal. The off diagonal matrix elements $\rho_{\alpha\beta}$ of the density matrix provide a measure of how correlated the many-body wave function is, while the diagonal matrix elements $\rho_{\alpha\alpha}$ provide the occupancies of each single-particle state $| a_{i} \rangle$ in the many-body wave function. The sum over the diagonal matrix elements is still equal to the total number of nucleons in the many-body wave function
\begin{equation}
\sum_{\alpha} \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle = A.
\label{eqn-chap2-density-matrix-number}
\end{equation}
It is important to stress here that a diagonal one-body density matrix does not necessarily indicate that a many-body wave function is uncorrelated unless the diagonal matrix elements $\rho_{\alpha \alpha}$ are exactly equal to $1$. The one-body density matrix is the starting point for the construction of natural orbitals in Chapter~\ref{chap-chap3}.


\section{Example calculations and infrared extrapolations}
\label{sec-chap2-example-calculations}


In this section we perform NCCI calculations to obtain the ground state energy and proton radius of the isotopes $\isotope[3,4]{He}$. Our goal is to revisit the convergence properties of NCCI calculations using the harmonic oscillator basis and to extrapolate the calculated results to the full $\Nmax \rightarrow \infty$ space using the infrared extrapolation method which we present and discuss here.


In Fig.~\ref{fig-chap2-helium3-helium4}, we plot the calculated ground state energy (left) and proton radius (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom). Calculations were performed for even truncations of the many-body basis up to $\Nmax = 16$ (in steps of $2$) which scan the $\hw$ range $10$-$40$ MeV. The solid lines correspond to the calculated results, the dashed horizontal lines correspond to the experimental results, and the dotted lines connect extrapolated results obtained using the infrared extrapolation method (discussed below). The experimental binding energies are taken from~\cite{npa-purcell-a-3-data:2010,npa-tilley-a-4-data:1992}, while the proton radii are deduced using the experimentally measured nuclear charge radii reported in~\cite{angeli-marinova-nuclear-charge-radii:2013} and equation ($6$) in Ref.~\cite{bacca2012:6he-hyperspherical}. As we observe, the calculated ground state energy and proton radius of $\isotope[4]{He}$ converge. On the other hand, the calculated ground state energy of $\isotope[3]{He}$ approaches convergence (to the $\sim 0.01$ MeV level), while the proton radius does not converge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{\plotspath /ho_no_comparison/Z2-N1-Z2-N2-rp-e-HO-thesis-chapter1-170227.pdf}
\caption[Calculated ground state energy and proton radius in the ground state of {\protect $\isotope[3]{He}$} and {\protect $\isotope[4]{He}$}, obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The calculated results are extrapolated to the full space using the infrared extrapolation method.]{Calculated ground state energy (left) and proton radius in the ground state (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom), obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The dashed horizontal lines show the experimental results. The crosses connected by dotted lines are obtained by extrapolating calculated results using the infrared extrapolation method as described in the text.}
\label{fig-chap2-helium3-helium4}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 


Comparisons of NCCI calculations with experimental results are only meaningful once full convergence is achieved. However, when the calculated results do not converge we can attempt to extrapolate results obtained in truncated spaces to the full $\Nmax \rightarrow \infty$ space. One such example was presented in Chapter~\ref{chap-chap1}, where we used an empirical extrapolation method to extrapolate the calculated ground state energy of $\isotope[6]{He}$ to the full space. Here, we use the infrared extrapolation method to extrapolate the calculated ground state energy and proton radius of $\isotope[3,4]{He}$ to the full space. Extrapolating the converged $\isotope[4]{He}$ results serves as a test of the infrared method as we expect the extrapolated results to agree with the converged results.


The infrared extrapolation method~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation, more2013:ir-extrapolation,furnstahl2014:ir-expansion, furnstahl2015:ir-extrapolations,odell-papenbrock-ir-extrapolation-quadruple:2016} starts with the assumption that the truncated many-body basis  induces both a short-range ultraviolet (UV) and a long-range infrared (IR) cutoff on the ability of the many-body basis to describe the many-body wave function. Quantitatively, if the highest occupied single-particle orbital in the many-body basis has $N$ oscillator quanta, then to a first approximation the momentum space (UV) cutoff is~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation}
\begin{equation}
\Lambda_{\mathrm{UV}} = \sqrt{2(N+3/2)} \,\, \hbar/b,
\label{eqn-chap2-uv-cutoff}
\end{equation}
and the coordinate space (IR) cutoff is
\begin{equation}
L = \sqrt{2(N+3/2)} \,\, b,
\label{eqn-chap2-ir-cutoff}
\end{equation}
where $b$ is the oscillator length.  Assuming that ultraviolet convergence of the calculated results is reached (this typically happens when the ultraviolet cutoff of the internucleon interaction $\lambda$ is smaller than the ultraviolet cutoff $\Lambda_{\mathrm{UV}}$ of the basis), the bound state energies will converge exponentially with respect to $L$
\begin{equation}
E(N_{\mathrm{max}},\hbar\omega) = E_{\infty} +  a_{0} e^{-2 k_{\infty} L(N_{\mathrm{max}},\hbar\omega)},
\label{eqn-chap2-energy-extrapolation-theoretical}
\end{equation}
and the radii will converge as
\begin{equation}
r^{2}(L) = r_{\infty}^{2} [1 - (c_{0}+c_{1}\beta^{-2})\beta^{3}e^{-\beta}],
\label{eqn-chap2-rms-extrapolation}
\end{equation}
where $E_{\infty}$, $a_{0}$, $k_{\infty}$, $c_{0}$, $ c_{1}$, and $r_{\infty}^{2}$ are obtained by fitting (UV converged) calculated results and $\beta = 2k_{\infty} L$ [$k_{\infty}$ is taken from the energy fit in (\ref{eqn-chap2-energy-extrapolation-theoretical})]. The infrared cutoff was later studied in more detail and a more precise expression for $L$ was obtained by finding the lowest eigenvalue of the operator $p^{2}$ in a finite oscillator basis~\cite{more2013:ir-extrapolation} 
\begin{equation}
L(N,\hbar\omega) = \sqrt{2(N+\Delta N + 3/2)} \,\, b(\hbar\omega),
\label{eqn-chap2-ir-length}
\end{equation}
where $\Delta N = 2$ is an offset determined from the diagonalization of $p^{2}$.



The exponential convergence of the bound-state energies with respect to $L$ can be understood as follows~\cite{furnstahl2012:ho-extrapolation}. The finite extent $L$ of the oscillator basis in position space effectively imposes a Dirichlet boundary condition on the bound state wave function at $r = L$. The exponential convergence with respect to $L$ is thus directly related to the exponential fall-off of the bound-state wave functions in position space. 


Let us now use the infrared extrapolation method with our calculated results. Here, we perform a three point extrapolation using the calculated results at $\Nmax=12$, $14$, and $16$ sharing the same $\hw$ parameter. We deem results obtained using $\hw$ parameters $\hw \gtrsim 14$ MeV UV converged because their ultraviolet momentum $\Lambda_{UV}$ is comparable to the ultraviolet cutoff $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16}$ of the JISP$16$ interaction~\cite{shirokov2007:nn-jisp16}. Specifically, the JISP$16$ interaction is obtained by fitting scattering data in a harmonic oscillator space with $N=8$ and $\hw = 40$ MeV, which means that according to (\ref{eqn-chap2-uv-cutoff}) $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16} \approx 800$ $\mathrm{MeV}/c$. For the NCCI calculation with $\Nmax = 12$ and $\hw \approx 14$ MeV equation (\ref{eqn-chap2-uv-cutoff}) yields $\Lambda_{\mathrm{UV}} \approx 600$ $\mathrm{MeV}/c$ which is perhaps too low compared to the UV cutoff of JISP$16$.


In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (c)] and proton radius [panel (d)] of $\isotope[4]{He}$. As expected, the extrapolated results converge for both observables. A closer inspection reveals that a slight $\hw$ dependence persists which is however very small (at the $0.01$ MeV level and $0.01$ fm level for the extrapolated energy and proton radius respectively). For low $\hw$ parameters, the extrapolated energy does not converge which we expect since the calculated results used for the extrapolation are not fully UV converged. On the other hand, for high $\hw$ the extrapolated results converge since the calculated results used for the extrapolation are UV converged. The extrapolated ground state energy at $\hw \approx 20$ MeV ($-28.3$ MeV) agrees with the calculated result at the variational minimum of the $\Nmax = 16$ curve and the experimental result ($-28.3$ MeV). On the other hand, the extrapolated proton radius at $\hw \approx 20$ MeV ($1.44$ fm) agrees with the calculated result at $\Nmax = 16$ ($1.44$ fm) however it is about $\sim 0.03$ fm short of the experimental result. Thus, the NCCI calculation using the JISP$16$ interaction while predicting the binding energy correctly, it underestimates the proton radius.



In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (a)] and proton radius [panel (b)] of $\isotope[4]{He}$. We observe that the calculated ground state energy converges (to the $0.01$ MeV level). The extrapolated result is about $\sim 0.1$ MeV short of the experimental result ($-7.72$ MeV). The extrapolated proton radius staggers around the experimental result (at the $0.1$ fm level). However, since full convergence is not achieved we cannot assess whether the calculation correctly predicts the proton radius.



\section{Using a general single-particle basis in NCCI calculations}
\label{sec-chap2-general-basis}


In this section we review the procedure followed to derive the two-body matrix elements of the NCCI Hamiltonian in a general single-particle basis. The discussion follows closely the derivations discussed in Ref.~\cite{caprio2012:csbasis} where the two-body matrix elements of the NCCI Hamiltonian with respect to the Laguerre basis were derived. However, the discussion presented here is not limited to a particular single-particle basis. 


However, to aid the discussion we will use the Laguerre basis~\cite{caprio2012:csbasis} in the derivations. The Laguerre basis forms a complete, discrete, orthonormal set in the space of square integrable functions $\mathcal{L}^{2}(\mathbb{R}^{+})$. The Laguerre radial functions are given by
\begin{equation}
S_{nl}(b;r) = (2/b)^{-1} N_{nl} (2r/b)^{l+1} L_{n}^{2l+2} [2r/b] e^{-r/b},
\label{eqn-chap2-laguerre-radial-functions}
\end{equation}
where $n$ is the radial quantum number, $l$ is the angular momentum, $b$ is the characteristic length of the Laguerre functions, and $N_{nl}$ is a normalization given by
\begin{equation}
N_{nl} = \left( \frac{2}{b} \right)^{3/2} \left[ \frac{n!}{(n+2l+2)!} \right]^{1/2}.
\label{eqn-chap2-laguerre-normalization-coefficient}
\end{equation}
For each $l$, the Laguerre functions are orthonormal in $\mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} S_{nl}(b;r) S_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-cs-orthonormal}
\end{equation}
By replacing the harmonic oscillator radial functions $R_{nl}$ in (\ref{eqn-oscillator-orbitals-second-quantization}) with $S_{nl}$ we can form Laguerre single-particle states $| \alpha \rangle$ given by
\begin{equation}
| \alpha \rangle = \left[| S_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}}.
\label{eqn-laguerre-orbitals-second-quantization}
\end{equation}


To build the Hamiltonian matrix using a general single-particle basis we need to calculate the two-body matrix elements of the interaction and relative kinetic energy operators in the general basis. In the case where the two-body matrix elements of the interaction with respect to some single-particle basis are known, we can use a two-body transformation to obtain the two-body matrix elements in the general basis. For example, the JISP$16$ interaction is expressed in terms of the harmonic oscillator basis. Therefore, we can use a two-body transformation which will yield the two-body matrix elements in the general basis. Specifically, if $a = (n_{a}l_{a}j_{a})$ is a harmonic oscillator single-particle orbital and $\bar{a} = (\bar{n}_{a} \bar{l}_{a} \bar{j}_{a})$ is a Laguerre single-particle orbital then for antisymmetrized two-body states such as (\ref{eqn-chap2-two-particle-states-2}) the transformation is given by~\cite{hagen2006:gdm-realistic}
\begin{equation}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{AS}} = \sum_{abcd} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{AS}},
\label{eqn-chap2-two-body-interaction-transformation}
\end{equation}
where $\langle a | \bar{a} \rangle$ is an overlap bracket. For normalized antisymmetrized states such as (\ref{eqn-chap2-two-particle-states-3}) the transformation is given by
\begin{multline}
\langle \bar{c} \bar{d}; J | V | \bar{a} \bar{b}; J \rangle_{\mathrm{NAS}} = (1+\delta_{\bar{a}\bar{b}})^{-1/2} (1+\delta_{\bar{c}\bar{d}})^{-1/2} \\  \sum_{abcd} (1+\delta_{ab})^{1/2} (1+\delta_{cd})^{1/2} \langle a | \bar{a} \rangle \langle b | \bar{b} \rangle \langle c | \bar{c} \rangle \langle d | \bar{d} \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{NAS}}.
\label{eqn-chap2-two-body-interaction-transformation-nas}
\end{multline}
The overlap bracket is given by 
\begin{equation}
\langle a | \bar{a} \rangle = \langle R_{n_{a}l_{a}} | S_{\bar{n}_{a} \bar{l}_{a}} \rangle \delta_{(l_{a}j_{a})(\bar{l}_{a}\bar{j}_{a})}, 
\label{eqn-chap2-overlap-bracket}
\end{equation}
where 
\begin{equation}
\langle R_{nl} | S_{\bar{n}l} \rangle = \int_{0}^{\infty} dr R_{nl}(b_{\mathrm{HO}};r) S_{\bar{n}l}(b_{\mathrm{L}};r), 
\label{eqn-chap2-overlap-integral}
\end{equation}
and $b_{\mathrm{HO}}$ and $b_{\mathrm{L}}$ are the characteristic lengths of the harmonic oscillator basis and the Laguerre basis respectively. The transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) [or (\ref{eqn-chap2-two-body-interaction-transformation-nas})] involves an infinite quadruple sum over orbitals. The sum is truncated according to a one-body shell cutoff $\Ncut$ which must be selected in a way which ensures that NCCI calculations in the general basis are $\Ncut$ independent.


In principle, the two-body transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) can be used to obtain the two-body matrix elements of the relative kinetic energy operator in the general basis (provided that the matrix elements in the harmonic oscillator or other basis are known). However, in Ref.~\cite{caprio2012:csbasis} the transformation was found to yield calculated results which are highly sensitive to the $N_{\mathrm{cut}}$ truncation. Therefore, the two-body matrix elements of the relative kinetic energy operator were calculated directly in the general single-particle basis~\cite{caprio2012:csbasis}. Recall that the relative kinetic energy operator separates into one and two-body parts. Specifically, rearranging (\ref{eqn-chap2-kinetic-energy-decomposition}) we get
\begin{equation}
T_{\mathrm{rel}}  = \frac{1}{4 A m_{\mathrm{N}}} \sum_{i \neq j}^{A} (\mathbf{p}_{i}-\mathbf{p}_{j})^{2} = \frac{1}{2 A m_{\mathrm{N}}} \left[ (A-1) \sum_{i=1}^{A} p_{i}^{2} - \sum_{i \neq j}^{A} \mathbf{p}_{i} \cdot \mathbf{p}_{j} \right].
\label{eqn-chap2-kinetic-energy-decomposition-matrix-elements}
\end{equation}
The first term is a one-body operator the matrix elements of which can be calculated using the momentum space representation of the general single-particle basis. [For the Laguerre basis, the momentum space representation functions $\tilde{S}_{nl}(b;k)$, where $p = \hbar k$, are given in terms of Jacobi polynomials]. The second term is a two-body operator the matrix elements of which factorize according to Racah's reduction formula~\cite{suhonen2007:nucleons-nucleus}
\begin{equation}
\langle cd;J | \mathbf{p}_{1} \cdot \mathbf{p}_{2} | ab; J \rangle = (-1)^{j_{d}+j_{a}+J} \Gj{j_{c}}{j_{d}}{J}{j_{b}}{j_{a}}{1} \langle c || \mathbf{p}_{1} || a \rangle \langle d || \mathbf{p}_{2} || b \rangle,
\label{eqn-chap2-kinetic-energy-two-body-matrix-elements}
\end{equation}
where $\langle b || \mathbf{p} || a \rangle \propto [\int_{0}^{\infty} dk \tilde{S}_{n_{a}l_{a}}(b;k) k \tilde{S}_{n_{b}l_{b}}(b;k)] \langle l_{b} j_{b} || Y_{1} || l_{a} j_{a} \rangle$.


The suite of computer programs h$2$utils~\cite{caprio2012:csbasis} can be used for the calculation of the two-body matrix elements of the Hamiltonian in a general single-particle basis. The program calculates the two-body matrix elements of the relative kinetic energy operator and the two-body matrix elements of the interaction as separate matrices. The two matrices are then added (allowing the user to select different length parameters $b_{p}$ and $b_{n}$ for the proton and neutron spaces respectively), thus resulting in a Hamiltonian matrix which can then be used as an input to MFD which performs the many-body calculation.













==> chapters/chapter2/chapter2_draft_170309.tex <==
\chapter{INTRODUCTION TO THE NO-CORE CONFIGURATION INTERACTION APPROACH}
\label{chap-chap2}


\section{Overview}
\label{sec-chap2-overview}


In this chapter a broad overview of quantum many-body theory is presented focusing on the tools necessary to work with the no-core configuration interaction (NCCI) approach. The NCCI approach utilizes second quantization to cast the nuclear Hamiltonian into a square matrix in terms of a many-body basis. Here we describe all the steps needed to build and diagonalize the Hamiltonian matrix in some detail. Moreover, example calculations are presented and extrapolated using the infrared extrapolation method.


The general nuclear Hamiltonian for a system of $A$ nucleons interacting via two and/or three-body interactions $V(\mathbf{r}_{i},\mathbf{r}_{j})$ and $V(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k})$ respectively is given by
\begin{equation}
H = \frac{1}{2m_{\mathrm{N}}} \sum\limits_{i = 1}^{A} p_{i}^{2} + \sum_{i < j}^{A} V(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i < j < k}^{A} V_{\mathrm{NNN}}(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k}).
\label{eqn-chap2-overview-full-hamiltonian}
\end{equation}
Although three nucleon interactions are needed to accurately reproduce experimental data~\citep{pieperqmc:2008}, two-body interactions  provide a simpler context in which to focus on the main goal of this thesis, which is to introduce an alternative single-particle basis (other than the traditional harmonic oscillator basis) for NCCI calculations. Thus for the purpose of this thesis, we omit three-body terms from the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}).


Moreover, for reasons that have to do with the center-of-mass degree of freedom (described in Sec.~\ref{sec-chap2-com-factorization}) in the NCCI approach we do not work with the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}). Instead, we work with the translationally invariant intrinsic Hamiltonian \citep{vanhees:1983,lipkin:1958}
\begin{equation}
H_{\mathrm{in}} = T_{\mathrm{rel}} + V = \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}} 
+ \sum_{i < j}^{A} V_{\mathrm{NN}}(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i < j}^{Z} V_{\mathrm{C}}(\mathbf{r}_{i},\mathbf{r}_{j}) ,
\label{eqn-chap2-overview-hamiltonian}
\end{equation}
where $m_{\mathrm{N}} c^{2} = 938.92$ MeV is the average nucleon mass, $V_{\mathrm{NN}}$ is the internucleon interaction, and $V_{\mathrm{C}}$ is the Coulomb interaction. 


We start with a brief summary of second quantization (Sec.~\ref{sec-chap2-second-quantization}) which is then used to derive the two-body matrix elements of the NCCI Hamiltonian (Sec.~\ref{sec-chap2-tbme}). Consequently, we discuss the harmonic oscillator single-particle radial functions (Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}) and the nuclear many-body basis (Sec.~\ref{sec-chap2-many-body-basis}). The complete factorization of the center-of-mass and intrinsic portions of the many-body wave function (Sec.~\ref{sec-chap2-com-factorization}) and a description of the procedure followed to perform many-body calculations using the NCCI approach (Sec.~\ref{sec-chap2-many-body-calculations}) follow. The one-body density matrix and its properties are reviewed (Sec.~\ref{sec-chap2-one-body-density-matrix}). Example calculations for the nuclei $\isotope[3]{He}$ and $\isotope[4]{He}$ are presented, and the calculated results are extrapolated using the infrared extrapolation method (Sec.~\ref{sec-chap2-example-calculations}). We conclude this Chapter with an overview of the steps needed to perform an NCCI calculation using a general single-particle basis (Sec.~\ref{sec-chap2-general-basis}).


\section{Second quantization}
\label{sec-chap2-second-quantization}


Second quantization is used to describe systems of many identical particles. In what follows the notational conventions of Negele are used~\cite{negele1988:many-particle}.


The Hilbert space of $A$ distinguishable particles $ \mathcal{H}^{A}$ is spanned by the tensor product of $A$ distinguishable particles occupying single-particle states which belong to the single-particle Hilbert space $\mathcal{H}$ 
\begin{equation}
\mathcal{H}^{A} = \mathcal{H} \otimes \mathcal{H} \otimes \ldots \otimes \mathcal{H}.
\label{eqn-chap2-hilbert-space-product}
\end{equation}
If $\left\{ | a \rangle \right\}$ is an orthonormal basis for $\mathcal{H}$, an orthonormal basis for $\mathcal{H}^{A}$ can be constructed as the set of tensor product states
\begin{equation}
| a_{1} \ldots a_{A} ) \equiv |a_{1} \rangle \otimes |a_{2} \rangle \otimes \ldots \otimes |a_{A} \rangle,
\label{eqn-chap2-many-body-basis-product}
\end{equation}
where the curved parenthesis on the left hand side of (\ref{eqn-chap2-many-body-basis-product}) denotes that the many-body state is a simple product of single-particle states (i.e., no assumptions are made about the symmetry of the many-body state). 


The space of $A$ indistinguishable fermions $\mathcal{F}^{A}$ is spanned by fully antisymmetric many-body states constructed using the many-body states of $\mathcal{H}^{A}$  
\begin{equation}
| a_{1} \ldots a_{A} \rangle = \frac{1}{\sqrt{A!}} \sum_{P} (-1)^{P} | a_{P_{1}} \rangle \otimes | a_{P_{2}} \rangle \otimes \ldots \otimes | a_{P_{A}} \rangle.
\label{eqn-chap2-many-body-basis-antisymmetric}
\end{equation} 
The sum over $P$ is a sum over all possible permutations $(P_{1},\,P_{2},\ldots,P_{A})$ of the set $(a_{1},\,a_{2},\,\ldots, a_{A})$. Moreover, $(-1)^{P}$ is determined by counting the number of transpositions of two elements which brings a permutation to its original form $(a_{1},\,a_{2},\,\ldots, a_{A})$. 


The Fock space $F$ for fermions is the (Hilbert) direct sum of the fermion spaces $\mathcal{F}^{0}$, $\mathcal{F}^{1}$, $\mathcal{F}^{2}$, $\ldots$, $\mathcal{F}^{A}$, $\ldots$ for zero, one, two, etc particles
\begin{equation}
F = \mathcal{F}^{0} \oplus \mathcal{F}^{1} \oplus \mathcal{F}^{2} \oplus \ldots \oplus \mathcal{F}^{A} \oplus \ldots.
\label{eqn-chap2-fock-space}
\end{equation}
Here $\mathcal{F}^{0}$ is the space of no particles, $\mathcal{F}^{1}$ is identical to $\mathcal{H}$, and $\mathcal{F}^{A}$ with $A \geq 2$ is the space spanned by many-body states given by (\ref{eqn-chap2-many-body-basis-antisymmetric}).


Creation and annihilation operators generate the entire Fock space $F$ by adding (removing) single-particle states to (from) many-body states. The fermionic creation operator $c_{a}^{\dagger}$ adds a particle in a single-particle state $| a \rangle$ to the many-body state $| a_{1} \ldots a_{A} \rangle$ as follows
\begin{equation}
c_{a}^{\dagger} | a_{1} a_{2} \ldots a_{A} \rangle = | a a_{1} a_{2} \ldots a_{A} \rangle,
\label{eqn-chap2-creation-operator}
\end{equation}
where the definition implies that the particle is added to the left of the initial many-body state. Now, because of the antisymmetry requirement for fermions we cannot act with the $c_{a}^{\dagger}$ operator on the state $| a a_{1} a_{2} \ldots a_{A} \rangle$ (and thus add the single-particle state $| a \rangle$ twice). This state is equal to zero by definition
\begin{equation}
c_{a}^{\dagger} |a a_{1} a_{2} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-creation-operator-2}
\end{equation}
Similarly an annihilation operator $c_{a}$ removes a particle occupying the single-particle state $|a\rangle$ from a many-body state
\begin{equation}
c_{a} |a a_{1} \ldots a_{A} \rangle = | a_{1} \ldots a_{A} \rangle.
\label{eqn-chap2-annihilation-operator}
\end{equation}
For completeness, note that in general $c_{a} | a_{1} a_{2} \ldots a \ldots a_{A} \rangle = (-1)^{P} | a_{1} a_{2} \ldots a_{A} \rangle$ where $P$ is the number of transpositions of two elements needed to bring the particle in the single-particle state $| a \rangle$ to the front of the many-body state. For example $c_{a_{2}} | a_{1} a_{2} a_{3} \rangle = - |a_{1} a_{3} \rangle$. If $c_{a}$ acts on a state $| a_{1} \ldots a_{A} \rangle$, i.e., a state which has no particle in the single-particle state $| a \rangle$, then the action of $c_{a}$ on the many-body state $| a_{1} \ldots a_{A} \rangle$ yields zero
\begin{equation}
c_{a} |a_{1} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-annihilation-operator-2}
\end{equation}
Following from~(\ref{eqn-chap2-creation-operator})-(\ref{eqn-chap2-annihilation-operator-2}), we conclude that the creation and annihilation operators obey the fermionic anticommutation relation
\begin{equation}
\lbrace c_{a} , c_{b}^{\dagger} \rbrace = \delta_{ab}.
\label{eqn-chap2-anti-commutation}
\end{equation}


One-body operators are operators which can be written as a sum of single-particle operators acting on one particle at a time. To be able to calculate the matrix elements of one-body operators with respect to many body states like (\ref{eqn-chap2-many-body-basis-antisymmetric}), it is useful to express them in terms of creation and annihilation operators. To arrive at this expression, let us first use the many-body states of $\mathcal{H}^{A}$ to calculate the matrix elements of a one-body operator $T = \sum_{i=1}^{A} t_{i}$. For the diagonal matrix elements (i.e., between the same many-body states) we have
\begin{multline}
( a_{1}a_{2} \ldots a_{A} | T | a_{1} a_{2} \ldots a_{A} ) = \\  
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2} \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \\
\langle a_{1} | t_{1} | a_{1} \rangle + \ldots + \langle a_{A} | t_{A} | a_{A} \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-identical-states}
\end{multline}
where we used the fact that the single-particle states are orthonormal hence $\langle a_{i} | a_{j} \rangle = \delta_{a_{i}a_{j}}$. Let us now evaluate the non-diagonal matrix elements of $T$ starting with the matrix elements between the many-body state $ | a_{1} a_{2} \ldots a_{A} )$ and the many-body state $ | a_{1} a_{2}' \ldots a_{A} )$, where $| a_{2} \rangle \neq | a_{2}' \rangle$. We have
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1} a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \langle a_{1} | a_{1} \rangle \langle a_{2} | t_{2} | a_{2}' \rangle \langle a_{3} | a_{3} \rangle \ldots \langle a_{A} | a_{A} \rangle + \\
+ \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \langle a_{2} | t_{2} | a_{2}' \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-one-sp-state-different}
\end{multline}
since $\langle a_{2} | a_{2}' \rangle = 0 $. Finally, the matrix elements of $T$ between the many-body states $| a_{1} a_{2} \ldots a_{A} )$ and $| a_{1}' a_{2}' \ldots a_{A} )$, where $| a_{1} \rangle \neq | a_{1}' \rangle$ and $| a_{2} \rangle \neq | a_{2}' \rangle$, are
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1}' a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1}' \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1}' \rangle \ldots \langle a_{A} | t_{A} | a_{A} \rangle = 0.
\label{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}
\end{multline}
Thus, the matrix elements of the one-body operator $T$ with respect to many-body states of $\mathcal{H}^{A}$ are fully defined by the sum over single-particle matrix elements of $\mathcal{H}$. If we now define the single-particle vacuum state $| - \rangle$ (i.e., a non-occupied single-particle state), then $c_{a}^{\dagger} | - \rangle = | a \rangle$. Using this definition and (\ref{eqn-chap2-one-body-operator-matrix-elements-identical-states})-(\ref{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}) we can write a one-body operator as
\begin{equation}
T = \sum_{ab} t_{ab} c_{a}^{\dagger} c_{b},
\label{eqn-chap2-one-body-operator-second-quantization}
\end{equation}
where $t_{ab} = \langle a | t | b \rangle$.

Similarly, the matrix elements of a two-body operator $V = \frac{1}{2} \sum_{i \neq j} u_{ij}$ with respect to the many-body states of $ \mathcal{H}^{A}$ are fully defined by the matrix elements $u_{abcd} = (ab | u | cd )$ calculated using the states of $\mathcal{H}^{2}$. Thus we can write $V$ as
\begin{equation}
V = \frac{1}{2} \sum_{abcd} u_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c}.
\label{eqn-chap2-interaction-second-quantized}
\end{equation}
However, it is more convenient to write the two-body operator as
\begin{equation}
V = \frac{1}{4} \sum_{abcd} \bar{u}_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c},
\label{eqn-chap2-interaction-second-quantized-antisymmetrized}
\end{equation}
where $\bar{u}_{abcd} = u_{abcd} - u_{abdc} = \langle ab | u | cd \rangle$ are normalized and antisymmetrized two-body matrix elements.


\section{Two-body matrix elements for the NCCI Hamiltonian}
\label{sec-chap2-tbme}

In the context of the NCCI approach, the most commonly used single-particle states are the harmonic oscillator single-particle basis states (see Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}). A harmonic oscillator single-particle state is labeled by the quantum numbers $| \alpha \rangle \equiv |n_{a}l_{a}j_{a}m_{a} \rangle$, where $n_{a}$ is the harmonic oscillator radial quantum number, $l_{a}$ is the angular momentum, $j_{a}$ is the total angular momentum, and $m_{a}$ is the $z$ projection of the total angular momentum. Using the harmonic oscillator single-particle states we can construct fully antisymmetric many-body basis states for the NCCI approach
\begin{equation}
| (n_{a}l_{a}j_{a}m_{a}) (n_{b}l_{b}j_{b}m_{b}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle.
\label{eqn-chap2-many-body-state-harmonic-oscillator}
\end{equation} 
Many-body states such as (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) have a total $z$ projection of total angular momentum $M=\sum_{i=1}^{A} m_{i}$ and a total number of oscillator quanta $N_{\mathrm{tot}}=\sum_{i=1}^{A} (2n_{i} + l_{i}) = \sum_{i=1}^{A} N_{i}$. The harmonic oscillator single-particle states $| \alpha \rangle$ are given as the tensor product 
\begin{equation}
| \alpha \rangle = \left[| R_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}},
\label{eqn-oscillator-orbitals-second-quantization}
\end{equation}
where $R_{n_{a}l_{a}}$ is a harmonic oscillator radial function, $Y_{l_{a}}$ is a spherical harmonic, and $|\frac{1}{2} \rangle$ is a spinor. The subscripts $j_{a}$ and $m_{a}$ indicate that $| R_{n_{a} l_{a}} Y_{l_{a}} \rangle$ (a spherical tensor of rank $l_{a}$) and the spinor $| \frac{1}{2} \rangle$ are coupled to total angular momentum $j_{a}$ and $z$ projection of total angular momentum $m_{a}$~\cite{rose1957:am}. 


The Hilbert space of the NCCI Hamiltonian is spanned by the many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) which provide a basis for the representation of the Hamiltonian as a square matrix. To cast the Hamiltonian into a square matrix we must first calculate the two-body matrix elements of the relative kinetic energy and two-body $NN$ interaction operators. The two-body matrix elements are calculated with respect to two-particle states, coupled to total angular momentum $J$. For distinguishable particles (e.g., one proton and one neutron states), angular momentum coupled two-particle states are defined as 
\begin{equation}
| a b ; J ) = \sum_{m_{a}m_{b}} \langle j_{a} m_{a} j_{b} m_{b} | J M \rangle |a m_{a} \rangle | b m_{b} \rangle,
\label{eqn-chap2-two-particle-states-1}
\end{equation}
where $| a m_{a} \rangle = | n_{a} l_{a} j_{a} m_{a} \rangle$, $\langle j_{a} m_{a} j_{b} m_{b} | J M \rangle $ is a Clebsch-Gordan coefficient, and the parenthesis implies that the two-particle state is not antisymmetrized. For two identical fermions we can obtain fully antisymmetrized states using the states $| a b ; J )$. We have
\begin{equation}
| a b ; J M \rangle_{\mathrm{AS}} = \frac{1}{\sqrt{2}} \left[ | a b ; J M ) - (-1)^{J - j_{a} - j_{b}} | b a ; J M \rangle \right].
\label{eqn-chap2-two-particle-states-2}
\end{equation}
These states have the symmetry property $| a b ; J M \rangle = - (-1)^{J -j_{a}-j_{b}} | b a ; J M \rangle$ which implies that if the states $| a \rangle$ and $| b \rangle$ are identical, only two-body states with even $J$ are allowed. The states (\ref{eqn-chap2-two-particle-states-2}) are antisymmetrized but not strictly normalized. An extra factor of $1 / \sqrt{2}$ is required for normalization in the special case when the two particles occupy the same single-particle orbital $| n_{a} l_{a} j_{a} \rangle$. Hence, the appropriate two-particle states are
\begin{equation}
| a b ; J M \rangle_{\mathrm{NAS}} = (1 + \delta_{ab})^{-1/2} | a b ; J M \rangle_{\mathrm{AS}}.
\label{eqn-chap2-two-particle-states-3}
\end{equation}
Both the normalized antisymmetrized states and the antisymmetrized states are used to calculate the two-body matrix elements $\langle c d ; J | H_{\mathrm{in}} | a b ; J \rangle$ of the (scalar) intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}). The change of basis relation between two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-2}) and two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-3}) is
\begin{equation}
\langle c d ; J | H | a b ; J \rangle_{\mathrm{NAS}} = (1+\delta_{cd})^{-1/2} (1+\delta_{ab})^{-1/2} \langle c d ; J | H | a b ; J \rangle_{\mathrm{AS}}.
\label{eqn-chap2-nas-two-body-matrix-elements}
\end{equation}
A detailed discussion about the calculation of the two-body matrix elements of the intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) is given in Ref.~\cite{caprio2012:csbasis}. A brief overview is also given in Sec.~\ref{sec-chap2-general-basis}.
 

\section{The harmonic oscillator single-particle states}
\label{sec-chap2-harmonic-oscillator-radial-functions}


In this section we will review the basic properties of the harmonic oscillator single-particle states $| \alpha \rangle$~\cite{suhonen2007:nucleons-nucleus,moshinsky1996:oscillator,weniger1985:fourier-plane-wave} which are traditionally used in the NCCI approach because their properties facilitate the many-body calculations. The harmonic oscillator single-particle states are also our starting basis for the construction of natural orbitals which are introduced in Chapter~\ref{chap-chap3}. 


The first important property of the harmonic oscillator single-particle states (relevant to the NCCI approach) is that they allow for the complete removal of spurious center-of-mass states from the low-lying spectrum of the NCCI Hamiltonian provided that an $\Nmax$ truncation is imposed on the many-body basis. The appearance of spurious center-of-mass states results from using the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) for the representation of the NCCI Hamiltonian as a square matrix. A detailed discussion about the appearance of spurious center-of-mass states in an NCCI calculation and the procedure followed for their removal from the low-lying spectrum is given in Sec.~\ref{sec-chap2-many-body-basis}.

The second important property of the harmonic oscillator single-particle states (relevant to many-body calculations and consequently the NCCI approach) is that they simplify the calculation of two-body matrix elements for operators written in terms of relative coordinates, using the Moshinsky transformation~\citep{moshinsky1996:oscillator}. According to  the transformation, products of harmonic oscillator states expressed in single-particle coordinates $R_{n_{1}l_{1}}(\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ transform into products of harmonic oscillator states expressed in terms of relative and center-of mass coordinates $R_{nl}(\mathbf{r}_{\mathrm{rel}})R_{NL}(\mathbf{R})$, where $2 n_{1} + l_{1} + 2 n_{2} + l_{2}= 2 n + l+ 2 N + L$, $\mathbf{r}_{\mathrm{rel}} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}-\mathbf{r}_{2})$, and $\mathbf{R} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}+\mathbf{r}_{2})$. (The factor of $1/\sqrt{2}$ in front of the center-of-mass vector is used instead of the traditional $1/2$ for normalization reasons). The calculation of two-body matrix elements for operators of the form $V(\mathbf{r}_{1}-\mathbf{r}_{2})$ with respect to two-particle states of the form $R_{n_{1}l_{1}} (\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ is then reduced to the calculation of the single-particle matrix element of the operator $V(\mathbf{r}_{\mathrm{rel}})$ with respect to single-particle states of the form $R_{nl}(\mathbf{r}_{\mathrm{rel}})$ and an overlap between single-particle states of the form $R_{NL}(\mathbf{R})$.

Let us now review the harmonic oscillator radial wave functions. If we write the single-particle wave function as $\Psi_{nlm}(\mathbf{r})=r^{-1} R_{nl}(b;r)Y_{lm}(\theta,\phi)$, where $R_{nl}(b;r)$ are radial wave functions and $Y_{lm}(\theta,\phi)$ are spherical harmonics, then $\Psi_{nlm}(\mathbf{r})$ are solutions to the familiar harmonic oscillator central force problem \cite{suhonen2007:nucleons-nucleus} 
\begin{equation}
h(\omega) = \frac{p^{2}}{2m_{\mathrm{N}}} + \frac{m_{\mathrm{N}} \omega^{2} r^{2}}{2}.
\label{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}
\end{equation} 
where $m_{\mathrm{N}}c^{2} \approx 938.92$ MeV is the average nucleon mass and $\omega$ is the oscillator frequency. The length scale of the radial functions $R_{nl}(b;r)$ is set by the oscillator length $b$ which depends on the parameters of the oscillator Hamiltonian (\ref{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}) as $b=\sqrt{\hbar / (m_{\mathrm{N}} \omega})$. The eigenvalues corresponding to each single-particle radial wave function are given by $ (N + 3/2) \hw$, where $N = 2n + l$ is the oscillator quantum (notice that the eigenvalues are evenly spaced by one unit of $\hw$). The radial functions $R_{nl}(b;r)$ are given by
\begin{equation}
R_{nl}(b;r) = b N_{nl} (r/b)^{l+1} L_{n}^{l+1/2}[(r/b)^{2}] e^{-(r/b)^{2}/2},
\label{eqn-chap2-harmonic-oscillator-radial-functions}
\end{equation} 
where $L_{n}^{l+1/2}[(r/b)^{2}]$ are generalized Laguerre polynomials, $n$ is the radial quantum number (which gives the number of nodes in the radial function), $l$ is the angular momentum, and $N_{nl}$ is a normalization factor given by
\begin{equation}
N_{nl} = \frac{1}{b^{3/2}} \left[ \frac{2n!}{(l+n+1/2)!} \right]^{1/2}.
\label{eqn-chap2-harmonic-oscillator-functions-normalization}
\end{equation}
For each $l$, the harmonic oscillator radial functions form a complete discrete basis for square integrable functions on $ \mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} R_{nl}(b;r) R_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-ho-orthonormal}
\end{equation}
 

\section{Symmetries of the NCCI Hamiltonian and the nuclear \\ many-body basis}
\label{sec-chap2-many-body-basis}


The selection of the nuclear many-body basis used in NCCI calculations is based on the symmetries of the NCCI Hamiltonian~(\ref{eqn-chap2-overview-hamiltonian}). The NCCI Hamiltonian is rotationally invariant therefore it conserves the total angular momentum $J$ and the $z$ projection of total angular momentum $M$. Moreover, the Hamiltonian conserves parity. To diagonalize the Hamiltonian we can choose to use many-body states that have good $J$ (a $J$-scheme basis) or many-body states that have good $M$ (an $M$-scheme basis)~\cite{whitehead1977:shell-methods}. Although the $M$-scheme basis involves a larger number of many-body basis states compared to a $J$-scheme basis, constructing $M$-scheme many-body basis states is straightforward (i.e., we do not have to deal with angular momentum coupling as in the $J$-scheme basis). Therefore, for the NCCI calculations discussed here, an $M$-scheme basis is considered. However, the eigenstates of $H$ still have good $J$ which is recovered after diagonalization by calculating the expectation value of the $J^{2}$ operator with respect to the calculated many-body wave function.


To build many-body basis states we start from single-particle states $| nljm \rangle$ and construct fully antisymmetric states (with good $M$) given by~(\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Calculations can be performed for any possible value of $M$ (which is supported by the single-particle states in the many-body basis). For example, for even nuclei $M=0, 1,\ldots$ and for odd nuclei $M=1/2, 3/2, \ldots$ (we do not consider negative values for $M$ here). However, we usually use many-body states with $M=0$ for even nuclei and $M=1/2$ for odd nuclei. This is because for a given $M$ we can only obtain many-body wave functions with $J \geq | M |$. Thus, choosing the lowest possible $M$ allows us to study the ground and first few excited states of a nucleus.


Commonly, for reasons involving the center-of-mass degree of freedom, as discussed in Sec.~\ref{sec-chap2-com-factorization}, the many-body basis is truncated using the $\Nmax$ truncation scheme~\cite{elliott1955:com-shell}. The scheme dictates that only many-body states with $\Ntot \leq N_{0} + \Nmax$ are permitted in the many-body basis, where $N_{0}$ is the number of quanta in the configuration where all the nucleons occupy the lowest permitted oscillator shells. For example, $N_{0}=2$ for $\isotope[6]{He}$ (in this configuration, the two protons occupy the $N=0$ proton shell, two neutrons occupy the $N=0$ neutron shell, and the last two neutrons occupy the $N=1$ shell) and $N_{0} =3$ for $\isotope[7]{Li}$ (because the extra proton compared to $\isotope[6]{He}$ goes into the $N=1$ proton shell). 




Finally, because the nuclear Hamiltonian conserves parity we want our many-body basis to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. A many-body basis truncated at a given $\Nmax$ contains (many-body) states with $N_{\mathrm{tot}} \leq N_{0} + \Nmax$, where $N_{\mathrm{tot}} = \sum_{i} N_{i} = N_{1} + \ldots + N_{A}$, and $N_{i}$ is the oscillator quantum of a nucleon $i$ in its single-particle state. Hence, many-body basis states which belong to this (many-body) basis have parity which is obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the many-body states of the lowest allowed configuration is $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity eigenstates of the nucleus we must build many-body bases with even $\Nmax$ truncations, i.e., $\Nmax = 0, 2, 4, \ldots$. On the other hand, to obtain the unnatural parity eigenstates of the nucleus we must construct many-body bases with odd $\Nmax$ truncations, i.e., $\Nmax = 1, 3, 5, \ldots$. 

%Finally, because the nuclear Hamiltonian conserves parity we want our many-body basis to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. This means that the parity of a many-body state which belongs to the many-body basis can be obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the lowest possible configuration is given by $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity states of the nucleus $\Nmax$ must be even and proceed in steps of $2$, i.e., $\Nmax = 2, 4, 6, \ldots$. On the other hand, to obtain the unnatural parity states of the nucleus $\Nmax$ must be odd and also proceed in steps of $2$, i.e., $\Nmax = 1, 3, 5, \ldots$. 






\section{Spurious center-of-mass states removal}
\label{sec-chap2-com-factorization}


In this section we describe how spurious center-of-mass states result from the diagonalization of the NCCI Hamiltonian matrix built in terms of the set of the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Subsequently, we describe how these spurious states can be removed provided that the $\Nmax$ truncation scheme is used.

The many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) are defined with respect to a fixed point in space. However, physically there is no such point around which all the nucleons are orbiting. Rather we are interested in the internal motion of the nucleons relative to each other within the nucleus, a motion which defines the intrinsic structure of the nucleus.


In principle we can convert to relative coordinates. However, antisymmetrization in Jacobi coordinates (which define the relative motion) is cumbersome. Therefore, we are compelled to work in the full coordinate space which includes both the center of mass and relative degrees of freedom.


Our goal is to describe the relative motion as accurately as possible without unnecessary complications arising from the center of mass motion. In order to accomplish this it helps making certain choices regarding the basis and the Hamiltonian.


We want our eigenfunctions to factorize into center of mass and relative factors. We also want the center of mass factor to be simple and well understood so that it does not interfere with the calculation of energies and observables. In principle, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) is already separated into center of mass and relative coordinates. If we define the center-of-mass momentum as $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, the one-body kinetic energy operator in (\ref{eqn-chap2-overview-full-hamiltonian}) can be decomposed into a center-of-mass and a relative kinetic energy contributions~\cite{vanhees:1983}
\begin{equation}
T = T_{\mathrm{c.m.}} + T_{\mathrm{rel}} = \frac{\left(\sum\limits_{i=1}^{A}\mathbf{p}_{i}\right)^{2}}{2Am_{\mathrm{N}}}  + \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}}.
\label{eqn-chap2-kinetic-energy-decomposition}
\end{equation}
Therefore, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) also separates into center-of-mass and relative parts
\begin{equation}
H= T_{\mathrm{c.m.}} + (T_{\mathrm{rel}} + V).
\label{eqn-chap2-full-separated-hamiltonian}
\end{equation}
Thus, in the full space our eigenfunctions would factorize into a center-of-mass and a relative wave function.

However, we are confined to work in a truncated space. Factorization can still be exact in an oscillator basis when the $\Nmax$ truncation is used. The truncated space then only contains a limited center-of-mass space spanned by center-of-mass harmonic oscillator states with $N_{\mathrm{c.m.}} = 0$, $2$, $\ldots, \Nmax$. We could attempt to diagonalize the Hamiltonian~(\ref{eqn-chap2-full-separated-hamiltonian}) in the truncated space. However, the $T_{\mathrm{c.m.}}$ operator will mix contributions with different center-of-mass excitations $N_{\mathrm{c.m.}}$ and destroy factorization of the eigenfunctions. The Hamiltonian will force us towards states which attempt to diagonalize the center-of-mass kinetic energy operator $T_{\mathrm{c.m.}}$. Therefore, our NCCI calculations would end up approximating spherical waves in the center of mass coordinates, at the expense of accurately describing the intrinsic motion.

Thus, instead, we choose to work with the intrinsic Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V.
\end{equation} 
The resulting Hamiltonian is block diagonal with respect to the number of quanta $N_{\mathrm{c.m.}}$ for the center-of-mass motion. The resulting eigenfunctions will factorize into a center-of-mass factor of good $N_{\mathrm{c.m.}}$ and an intrinsic factor. The total number of quanta in a many-body state is shared between the center-of-mass motion and the intrinsic motion:
\begin{equation}
\Ntot = \sum_{i} N_{i} = N_{\mathrm{c.m.}} + N_{\mathrm{rel}}.
\label{eqn-chap2-number-of-quanta-com-quanta}
\end{equation}
Therefore, in eigenfunctions with $N_{\mathrm{c.m.}} = 0$, the full $\Nmax$ quanta are available to use in describing the intrinsic motion. The higher $N_{\mathrm{c.m.}}$ eigenfunctions produce spurious copies of the spectrum in which the intrinsic motion is described using fewer quanta $N_{\mathrm{rel}} \leq \Nmax - N_{\mathrm{c.m.}}$. 


It is convenient to push the spurious excited center-of-mass states out of the low lying spectrum. We do this by adding a term diagonal in the number of center-of-mass quanta. That is we add a ``Lawson term''~\cite{gloeckner1974:spurious-com} proportional to the $N_{\mathrm{c.m.}}$ operator. This is often equivalently described as adding a center-of-mass harmonic oscillator Hamiltonian. In terms of the center-of-mass coordinate $\mathbf{R} = (\sum_{i} \mathbf{r}_{i})/A$ and the center-of-mass momentum $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, 
\begin{equation}
H_{\mathrm{c.m.}} = \frac{P^{2}}{2Am_{\mathrm{N}}} + \frac{1}{2} A m_{\mathrm{N}} \omega^{2} R^{2}.
\label{eqn-chap2-harmonic-oscillator-many-body-hamiltonian-com}
\end{equation}
Then, $H_{\mathrm{c.m.}} = (N_{\mathrm{c.m.}} + 3/2)\hbar \omega$. Thus we actually diagonalize the Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V + \alpha N_{\mathrm{c.m.}},
\label{eqn-chap2-ncci-hamiltonian-with-lawson}
\end{equation} 
where $\alpha$ is the Lawson term strength (typically a few MeV). This leads to the same eigenstates as the relative Hamiltonian but with the spurious states lifted out of the low-lying spectrum by an amount $\alpha N_{\mathrm{c.m.}}$.




\section{Many-body calculations}
\label{sec-chap2-many-body-calculations}


In this section we will briefly describe the general procedure followed to obtain results using the NCCI approach.

The basic ingredient needed to build the Hamiltonian matrix is the two-body matrix elements of the NCCI Hamiltonian (\ref{eqn-chap2-ncci-hamiltonian-with-lawson}) with respect to many-body basis states like (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Thus, we need to evaluate matrix elements of the form
\begin{equation}
\langle \Phi_{n} | H | \Phi_{m} \rangle,
\label{eqn-chap2-two-body-matrix-elements}
\end{equation}
where $| \Phi_{n} \rangle = | (n_{1}l_{1}j_{1}m_{1}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle$ is a many-body basis state. [The matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) reduce to a sum over two-body matrix elements of the form $\langle c d ; J | H | a b ; J \rangle$ using Wick's theorem]. After calculating the matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) for all the many-body states in our basis we obtain the Hamiltonian matrix
\begin{equation}
  \begin{pmatrix}
    \langle \Phi_{1} | H | \Phi_{1} \rangle & \langle \Phi_{1} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{1} | H | \Phi_{m} \rangle \\
    \langle \Phi_{2} | H | \Phi_{1} \rangle & \langle \Phi_{2} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{2} | H | \Phi_{m} \rangle \\
    \vdots & \vdots & \ddots & \vdots \\
   \langle \Phi_{d} | H | \Phi_{1} \rangle & \langle \Phi_{d} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{d} | H | \Phi_{d} \rangle
  \end{pmatrix}
\label{eqn-chap2-ncci-hamiltonian-matrix}
\end{equation}
The dimension $d$ of the matrix (\ref{eqn-chap2-ncci-hamiltonian-matrix}) is equal to the number of many-body basis states for a given nucleus and $\Nmax$ truncation (see Fig.~\ref{fig-chap1-NNCI-dimension}). Diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}) yields the nuclear many-body wave function
\begin{equation}
| \Psi \rangle = \sum\limits_{n=1}^{d} c_{n} | \Phi_{n} \rangle.
\label{eqn-chap2-ncci-wave-functions}
\end{equation}
%where $c_{n}$ are coefficients obtained from the diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}).


The diagonalization of the Hamiltonian matrix is commonly performed using the Lanczos algorithm~\cite{komzsik2003:lanczos-method,lanczos1950:algorithm}. The algorithm transforms the generally large sparse matrix (\ref{eqn-chap2-ncci-wave-functions}) into a tridiagonal matrix (of lower dimension than the original matrix). The tridiagonal matrix is then diagonalized (using an appropriate algorithm) and the eigenvalues and eigenvectors (of the tridiagonal matrix) are obtained. The eigenvectors of the tridiagonal matrix (Lanczos vectors) must then be converted from the Lanczos vector space to the original many-body basis. The process established by Lanczos proceeds as follows: If $H$ is a Hamiltonian matrix of order $n$ (i.e., the matrix dimension is $n \times n$), then we start with a random initial vector $b_{0}$ which is used to construct $m$ vectors (orthogonal to each other) according to the algorithm
\begin{align}
b_{0} & = \mathrm{random}, \nonumber & \\
b_{1} & = (H - \alpha_{0}) b_{0}, \nonumber \\
b_{2} & = (H - \alpha_{1}) b_{1} - \beta_{0} b_{0}, \nonumber \\
b_{3} & = (H - \alpha_{2}) b_{2} -\beta_{1} b_{1}, \nonumber \\
 \vdots  \nonumber & \\
b_{m} & = (H - \alpha_{m-1}) b_{m-1} - \beta_{m-2} b_{m-2} = 0,
\label{eqn-chap2-lanczos-algorithm}
\end{align}
where $m \leq n$. The equality to zero in the last step means the end of the process. The coefficients $\alpha_{m-1}$ and $\beta_{m-2}$ are determined by requiring that the norm of the vector $\parallel b_{m} \parallel$ is minimized. The coefficients are then used to build the tridiagonal matrix 
\begin{equation}
T =  \begin{pmatrix}
\alpha_{0} & \beta_{0} &   &   & 0\\ 
\beta_{0}  & \alpha_{1} & \beta_{1} & \\
                 & \ddots & \ddots & \ddots & \\
                 &  & \beta_{k-2} & \alpha_{k-1} &\beta_{k-1} \\
           0      & & & \beta_{k-1} & \alpha_{k}
  \end{pmatrix}
\label{eqn-chap2-tridiagonal-matrix}
\end{equation}
The eigenvalues of $T$ converge to the eigenvalues of $H$ provided that a sufficient number of iterations $k$, where $k < n$, is performed. 


The generally large sizes of the NCCI Hamiltonian matrices require the use of parallel computing which handles both the storage and the diagonalization of the Hamiltonian matrix. For the calculations presented in this thesis, we use the parallel code Many Fermion Dynamics-Nuclear (MFDn) \cite{maris2010:ncsm-mfdn-iccs10,vary2009:ncsm-mfdn-scidac09} developed by the Iowa State University group handles the construction of the many-body basis, the construction of the Hamiltonian matrix, the storage of the matrix over multiple cores, and the Lanczos diagonalization of the matrix. The input to the code includes the two-body matrix elements of the Hamiltonian, the $\Nmax$ truncation of the many-body basis, the number of protons ($Z$) and neutrons ($N$) of the nucleus we want to study, the number of Lanczos iterations we want to perform, and various other control parameters. The program outputs the eigenvalues (which are the nuclear level energies), the one-body density matrices (described in Sec.~\ref{sec-chap2-one-body-density-matrix}), and other observables.


\section{The one-body density matrix}
\label{sec-chap2-one-body-density-matrix}


The one-body density matrix can be calculated using the many-body wave functions obtained in a many-body calculation. It is more frequently used for the calculation of the matrix elements of one-body operators~\cite{suhonen2007:nucleons-nucleus}. Moreover, the static one-body density matrix contains information about correlations in the many-body wave function as described below. In second quantization, the transition one-body density matrix is given by
\begin{equation}
\rho_{\alpha\beta}^{\mathrm{f\,i}} = \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger} c_{\beta} | \Psi_{\mathrm{i}} \rangle,
\label{eqn-chap2-one-body-density-operator}
\end{equation}
where $| \Psi_{\mathrm{i}} \rangle$ and $| \Psi_{\mathrm{f}} \rangle$ are the many-body wave functions of an initial and a final nuclear state respectively. Using (\ref{eqn-chap2-one-body-density-operator}), the matrix elements of a one-body operator $\mathcal{O}$ are obtained as
\begin{equation}
\langle \Psi_{\mathrm{f}} | \mathcal{O} | \Psi_{\mathrm{i}} \rangle =  \sum_{\alpha\beta} \langle \alpha | \mathcal{O} | \beta \rangle \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger}c_{\beta} | \Psi_{\mathrm{i}} \rangle.
\label{eqn-chap2-one-body-operator-matrix-elements}
\end{equation}


The static one-body density matrix (i.e., the one-body density matrix obtained for the same initial and final many-body wave functions) contains information about correlations in the many-body wave function. By definition, an uncorrelated many-body wave function can be written as a single Slater determinant, i.e., $| \Psi \rangle = | a_{1} \ldots a_{A} \rangle$. For an uncorrelated many-body wave function, it is easy to see that the diagonal matrix elements $\rho_{\alpha\alpha} = \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle $ are equal to $1$ (which reflects the fact that each single-particle state is occupied by exactly one nucleon), while all the off diagonal matrix elements $\rho_{\alpha\beta}$ are equal to $0$. The sum of the diagonal matrix elements is equal to the total number of nucleons $A$ in the many-body wave function. In the case of a correlated many-body wave function, such as the ones calculated in an NCCI calculation, the one-body density matrix is not (in general) diagonal. The off diagonal matrix elements $\rho_{\alpha\beta}$ of the density matrix provide a measure of how correlated the many-body wave function is, while the diagonal matrix elements $\rho_{\alpha\alpha}$ provide the occupancies of each single-particle state $| a_{i} \rangle$ in the many-body wave function. The sum over the diagonal matrix elements is still equal to the total number of nucleons in the many-body wave function
\begin{equation}
\sum_{\alpha} \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle = A.
\label{eqn-chap2-density-matrix-number}
\end{equation}
It is important to stress here that a diagonal one-body density matrix does not necessarily indicate that a many-body wave function is uncorrelated unless the diagonal matrix elements $\rho_{\alpha \alpha}$ are exactly equal to $1$. The one-body density matrix is the starting point for the construction of natural orbitals in Chapter~\ref{chap-chap3}.


\section{Example calculations and infrared extrapolations}
\label{sec-chap2-example-calculations}


In this section we perform NCCI calculations to obtain the ground state energy and proton radius of the isotopes $\isotope[3,4]{He}$. Our goal is to revisit the convergence properties of NCCI calculations using the harmonic oscillator basis and to extrapolate the calculated results to the full $\Nmax \rightarrow \infty$ space using the infrared extrapolation method which we present and discuss here.


In Fig.~\ref{fig-chap2-helium3-helium4}, we plot the calculated ground state energy (left) and proton radius (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom). Calculations were performed for even truncations of the many-body basis up to $\Nmax = 16$ (in steps of $2$) which scan the $\hw$ range $10$-$40$ MeV. The solid lines correspond to the calculated results, the dashed horizontal lines correspond to the experimental results, and the dotted lines connect extrapolated results obtained using the infrared extrapolation method (discussed below). The experimental binding energies are taken from~\cite{npa-purcell-a-3-data:2010,npa-tilley-a-4-data:1992}, while the proton radii are deduced using the experimentally measured nuclear charge radii reported in~\cite{angeli-marinova-nuclear-charge-radii:2013} and equation ($6$) in Ref.~\cite{bacca2012:6he-hyperspherical}. As we observe, the calculated ground state energy and proton radius of $\isotope[4]{He}$ converge. On the other hand, the calculated ground state energy of $\isotope[3]{He}$ approaches convergence (to the $\sim 0.01$ MeV level), while the proton radius does not converge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{\plotspath /ho_no_comparison/Z2-N1-Z2-N2-rp-e-HO-thesis-chapter1-170227.pdf}
\caption[Calculated ground state energy and proton radius in the ground state of {\protect $\isotope[3]{He}$} and {\protect $\isotope[4]{He}$}, obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The calculated results are extrapolated to the full space using the infrared extrapolation method.]{Calculated ground state energy (left) and proton radius in the ground state (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom), obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The dashed horizontal lines show the experimental results. The crosses connected by dotted lines are obtained by extrapolating calculated results using the infrared extrapolation method as described in the text.}
\label{fig-chap2-helium3-helium4}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 


Comparisons of NCCI calculations with experimental results are only meaningful once full convergence is achieved. However, when the calculated results do not converge we can attempt to extrapolate results obtained in truncated spaces to the full $\Nmax \rightarrow \infty$ space. One such example was presented in Chapter~\ref{chap-chap1}, where we used an empirical extrapolation method to extrapolate the calculated ground state energy of $\isotope[6]{He}$ to the full space. Here, we use the infrared extrapolation method to extrapolate the calculated ground state energy and proton radius of $\isotope[3,4]{He}$ to the full space. Extrapolating the converged $\isotope[4]{He}$ results serves as a test of the infrared method as we expect the extrapolated results to agree with the converged results.


The infrared extrapolation method~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation, more2013:ir-extrapolation,furnstahl2014:ir-expansion, furnstahl2015:ir-extrapolations,odell-papenbrock-ir-extrapolation-quadruple:2016} starts with the assumption that the truncated many-body basis  induces both a short-range ultraviolet (UV) and a long-range infrared (IR) cutoff on the ability of the many-body basis to describe the many-body wave function. Quantitatively, if the highest occupied single-particle orbital in the many-body basis has $N$ oscillator quanta, then to a first approximation the momentum space (UV) cutoff is~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation}
\begin{equation}
\Lambda_{\mathrm{UV}} = \sqrt{2(N+3/2)} \,\, \hbar/b,
\label{eqn-chap2-uv-cutoff}
\end{equation}
and the coordinate space (IR) cutoff is
\begin{equation}
L = \sqrt{2(N+3/2)} \,\, b,
\label{eqn-chap2-ir-cutoff}
\end{equation}
where $b$ is the oscillator length.  Assuming that ultraviolet convergence of the calculated results is reached (this typically happens when the ultraviolet cutoff of the internucleon interaction $\lambda$ is smaller than the ultraviolet cutoff $\Lambda_{\mathrm{UV}}$ of the basis), the bound state energies will converge exponentially with respect to $L$
\begin{equation}
E(N_{\mathrm{max}},\hbar\omega) = E_{\infty} +  a_{0} e^{-2 k_{\infty} L(N_{\mathrm{max}},\hbar\omega)},
\label{eqn-chap2-energy-extrapolation-theoretical}
\end{equation}
and the radii will converge as
\begin{equation}
r^{2}(L) = r_{\infty}^{2} [1 - (c_{0}+c_{1}\beta^{-2})\beta^{3}e^{-\beta}],
\label{eqn-chap2-rms-extrapolation}
\end{equation}
where $E_{\infty}$, $a_{0}$, $k_{\infty}$, $c_{0}$, $ c_{1}$, and $r_{\infty}^{2}$ are obtained by fitting (UV converged) calculated results and $\beta = 2k_{\infty} L$ [$k_{\infty}$ is taken from the energy fit in (\ref{eqn-chap2-energy-extrapolation-theoretical})]. The infrared cutoff was later studied in more detail and a more precise expression for $L$ was obtained by finding the lowest eigenvalue of the operator $p^{2}$ in a finite oscillator basis~\cite{more2013:ir-extrapolation} 
\begin{equation}
L(N,\hbar\omega) = \sqrt{2(N+\Delta N + 3/2)} \,\, b(\hbar\omega),
\label{eqn-chap2-ir-length}
\end{equation}
where $\Delta N = 2$ is an offset determined from the diagonalization of $p^{2}$.



The exponential convergence of the bound-state energies with respect to $L$ can be understood as follows~\cite{furnstahl2012:ho-extrapolation}. The finite extent $L$ of the oscillator basis in position space effectively imposes a Dirichlet boundary condition on the bound state wave function at $r = L$. The exponential convergence with respect to $L$ is thus directly related to the exponential fall-off of the bound-state wave functions in position space. 


Let us now use the infrared extrapolation method with our calculated results. Here, we perform a three point extrapolation using the calculated results at $\Nmax=12$, $14$, and $16$ sharing the same $\hw$ parameter. We use results obtained using $\hw$ parameters $\hw \gtrsim 14$ MeV which have large $\Lambda_{UV}$ somewhat comparable to the ultraviolet cutoff $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16}$ of the JISP$16$ interaction~\cite{shirokov2007:nn-jisp16}. Specifically, the JISP$16$ interaction is obtained by fitting scattering data in a harmonic oscillator space with $N=8$ and $\hw = 40$ MeV, which means that according to (\ref{eqn-chap2-uv-cutoff}) $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16} \approx 800$ $\mathrm{MeV}/c$. For the NCCI calculation with $\Nmax = 12$ and $\hw \approx 14$ MeV equation (\ref{eqn-chap2-uv-cutoff}) yields $\Lambda_{\mathrm{UV}} \approx 600$ $\mathrm{MeV}/c$ which is perhaps too low compared to the UV cutoff of JISP$16$.


In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (c)] and proton radius [panel (d)] of $\isotope[4]{He}$. As expected, the extrapolated results converge for both observables. A closer inspection reveals that a slight $\hw$ dependence persists which is however very small (at the $0.01$ MeV level and $0.01$ fm level for the extrapolated energy and proton radius respectively). For low $\hw$ parameters, the extrapolated energy does not converge something that we expect since the calculated results used for the extrapolation are not fully UV converged. On the other hand, for high $\hw$ the extrapolated results converge since the calculated results used for the extrapolation are UV converged. The extrapolated ground state energy at $\hw \approx 20$ MeV ($-28.3$ MeV) agrees with the calculated result at the variational minimum of the $\Nmax = 16$ curve ($-28.3$ MeV) and the experimental result ($-28.3$ MeV). On the other hand, the extrapolated proton radius at $\hw \approx 20$ MeV ($1.44$ fm) agrees with the calculated result at $\Nmax = 16$ ($1.44$ fm); however, it is about $\sim 0.02$ fm short of the experimental result [$r_{p} = 1.462(6)$ fm]. Thus, the NCCI calculation using the JISP$16$ interaction correctly predicts the binding energy of $\isotope[4]{He}$, while the prediction for the proton radius is about $\sim 1.5$ $\%$ short of the experimental result.






In Fig.~\ref{fig-chap2-helium3-helium4}, we also show the extrapolated results for the ground state energy [panel (a)] and proton radius [panel (b)] of $\isotope[3]{He}$. We observe that the calculated ground state energy converges (to the $0.01$ MeV level). The extrapolated ground state energy at $\hw \approx 20$ MeV ($-7.67$ MeV) is about $\sim 0.05$ MeV short of the experimental result ($-7.72$ MeV). The extrapolated proton radius staggers around the experimental result [$r_{p} = 1.774(6)$ fm] at the $0.1$ fm level. However, since full convergence is not achieved we cannot assess whether the calculation correctly predicts the proton radius.



\section{Using a general single-particle basis in NCCI calculations}
\label{sec-chap2-general-basis}


In this section we review the procedure followed to derive the two-body matrix elements of the NCCI Hamiltonian in a general single-particle basis. The discussion follows closely the derivations discussed in Ref.~\cite{caprio2012:csbasis} where the two-body matrix elements of the NCCI Hamiltonian with respect to the Laguerre basis were derived. 



To build the Hamiltonian matrix using a general single-particle basis we need to calculate the two-body matrix elements of the interaction and relative kinetic energy operators in the general basis. In the case where the two-body matrix elements of the interaction with respect to some single-particle basis are known, we can use a two-body transformation to obtain the two-body matrix elements with respect to the general basis. For example, the JISP$16$ interaction is expressed in terms of the harmonic oscillator basis. Therefore, we can use a two-body transformation which will yield the two-body matrix elements in the general basis. Specifically, if $a = (n_{a}l_{a}j_{a})$ is a harmonic oscillator single-particle orbital and $a' = (n_{a'} l_{a'} j_{a'})$ is a general single-particle orbital then for antisymmetrized two-body states such as (\ref{eqn-chap2-two-particle-states-2}) the transformation is given by~\cite{hagen2006:gdm-realistic}
\begin{equation}
\langle c' d'; J | V | a' b'; J \rangle_{\mathrm{AS}} = \sum_{abcd} \langle a | a' \rangle \langle b | b' \rangle \langle c | c' \rangle \langle d | d' \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{AS}},
\label{eqn-chap2-two-body-interaction-transformation}
\end{equation}
where $\langle a | a' \rangle$ is an overlap bracket. For normalized antisymmetrized states such as (\ref{eqn-chap2-two-particle-states-3}) the transformation is given by
\begin{multline}
\langle c' d'; J | V | a' b'; J \rangle_{\mathrm{NAS}} = (1+\delta_{a'b'})^{-1/2} (1+\delta_{c'd'})^{-1/2} \\  \sum_{abcd} (1+\delta_{ab})^{1/2} (1+\delta_{cd})^{1/2} \langle a | a' \rangle \langle b | b' \rangle \langle c | c' \rangle \langle d | d' \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{NAS}}.
\label{eqn-chap2-two-body-interaction-transformation-nas}
\end{multline}
The overlap bracket is given by 
\begin{equation}
\langle a | a' \rangle = \langle R_{n_{a}l_{a}} | R_{n_{a'} l_{a'}} \rangle \delta_{(l_{a}j_{a})(l_{a'}j_{a'})}, 
\label{eqn-chap2-overlap-bracket}
\end{equation}
where 
\begin{equation}
\langle R_{n_{a}l_{a}} | R_{n_{a'}l_{a}} \rangle = \int_{0}^{\infty} dr R_{n_{a}l_{a}}(b_{\mathrm{HO}};r) R_{n_{a'}l_{a}}(b_{a'};r), 
\label{eqn-chap2-overlap-integral}
\end{equation}
and $b_{\mathrm{HO}}$ and $b_{a'}$ are the characteristic lengths of the harmonic oscillator basis and the general basis respectively. The transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) [or (\ref{eqn-chap2-two-body-interaction-transformation-nas})] involves an infinite quadruple sum over orbitals. The sum must be truncated, e.g., according to a one-body shell cutoff $\Ncut$ which must be selected in a way which ensures that NCCI calculations in the general basis are $\Ncut$ independent.


In principle, the two-body transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) can be used to obtain the two-body matrix elements of the relative kinetic energy operator in the general basis (provided that the matrix elements in the harmonic oscillator or some other single-particle basis are known). However, in Ref.~\cite{caprio2012:csbasis} the transformation was found to yield calculated results which are highly sensitive to the $N_{\mathrm{cut}}$ truncation. Therefore, the two-body matrix elements of the relative kinetic energy operator were calculated directly in the general single-particle basis~\cite{caprio2012:csbasis}. Recall that the relative kinetic energy operator separates into one and two-body parts. Specifically, rearranging (\ref{eqn-chap2-kinetic-energy-decomposition}) we get
\begin{equation}
T_{\mathrm{rel}}  = \frac{1}{4 A m_{\mathrm{N}}} \sum_{i \neq j}^{A} (\mathbf{p}_{i}-\mathbf{p}_{j})^{2} = \frac{1}{2 A m_{\mathrm{N}}} \left[ (A-1) \sum_{i=1}^{A} p_{i}^{2} - \sum_{i \neq j}^{A} \mathbf{p}_{i} \cdot \mathbf{p}_{j} \right].
\label{eqn-chap2-kinetic-energy-decomposition-matrix-elements}
\end{equation}
The first term is a one-body operator the matrix elements of which can be calculated using the momentum space representation of the general single-particle basis. The second term is a two-body operator the matrix elements of which factorize according to Racah's reduction formula~\cite{suhonen2007:nucleons-nucleus}
\begin{equation}
\langle cd;J | \mathbf{p}_{1} \cdot \mathbf{p}_{2} | ab; J \rangle = (-1)^{j_{d}+j_{a}+J} \Gj{j_{c}}{j_{d}}{J}{j_{b}}{j_{a}}{1} \langle c || \mathbf{p}_{1} || a \rangle \langle d || \mathbf{p}_{2} || b \rangle,
\label{eqn-chap2-kinetic-energy-two-body-matrix-elements}
\end{equation}
where $\langle b || \mathbf{p} || a \rangle \propto [\int_{0}^{\infty} dk \tilde{S}_{n_{a}l_{a}}(b;k) k \tilde{S}_{n_{b}l_{b}}(b;k)] \langle l_{b} j_{b} || Y_{1} || l_{a} j_{a} \rangle$.  















==> chapters/chapter2/chapter2_draft_170325.tex <==
\chapter{INTRODUCTION TO THE NO-CORE CONFIGURATION INTERACTION APPROACH}
\label{chap-chap2}


\section{Overview}
\label{sec-chap2-overview}


In this chapter a broad overview of quantum many-body theory is presented focusing on the tools necessary to work with the no-core configuration interaction (NCCI) approach. The NCCI approach utilizes second quantization to cast the nuclear Hamiltonian into a square matrix in terms of a many-body basis. Here we describe all the steps needed to build and diagonalize the Hamiltonian matrix in some detail. Moreover, example calculations are presented and extrapolated using the infrared extrapolation method.


The general nuclear Hamiltonian for a system of $A$ nucleons interacting via two and/or three-body interactions $V(\mathbf{r}_{i},\mathbf{r}_{j})$ and $V(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k})$ respectively is given by
\begin{equation}
H = \frac{1}{2m_{\mathrm{N}}} \sum\limits_{i = 1}^{A} p_{i}^{2} + \sum_{i < j}^{A} V(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i < j < k}^{A} V_{\mathrm{NNN}}(\mathbf{r}_{i},\mathbf{r}_{j},\mathbf{r}_{k}).
\label{eqn-chap2-overview-full-hamiltonian}
\end{equation}
Although three nucleon interactions are needed to accurately reproduce experimental data~\citep{pieperqmc:2008}, two-body interactions  provide a simpler context in which to focus on the main goal of this thesis, which is to introduce an alternative single-particle basis (other than the traditional harmonic oscillator basis) for NCCI calculations. Thus for the purpose of this thesis, we omit three-body terms from the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}).


Moreover, for reasons that have to do with the center-of-mass degree of freedom (described in Sec.~\ref{sec-chap2-com-factorization}) in the NCCI approach we do not work with the Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}). Instead, we work with the translationally invariant intrinsic Hamiltonian \citep{vanhees:1983,lipkin:1958}
\begin{equation}
H_{\mathrm{in}} = T_{\mathrm{rel}} + V = \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}} 
+ \sum_{i < j}^{A} V_{\mathrm{NN}}(\mathbf{r}_{i},\mathbf{r}_{j}) + \sum_{i < j}^{Z} V_{\mathrm{C}}(\mathbf{r}_{i},\mathbf{r}_{j}) ,
\label{eqn-chap2-overview-hamiltonian}
\end{equation}
where $m_{\mathrm{N}} c^{2} = 938.92$ MeV is the average nucleon mass, $V_{\mathrm{NN}}$ is the internucleon interaction, and $V_{\mathrm{C}}$ is the Coulomb interaction. 


We start with a brief summary of second quantization (Sec.~\ref{sec-chap2-second-quantization}) which is then used to derive the two-body matrix elements of the NCCI Hamiltonian (Sec.~\ref{sec-chap2-tbme}). Consequently, we discuss the harmonic oscillator single-particle radial functions (Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}) and the nuclear many-body basis (Sec.~\ref{sec-chap2-many-body-basis}). The complete factorization of the center-of-mass and intrinsic portions of the many-body wave function (Sec.~\ref{sec-chap2-com-factorization}) and a description of the procedure followed to perform many-body calculations using the NCCI approach (Sec.~\ref{sec-chap2-many-body-calculations}) follow. The one-body density matrix and its properties are reviewed (Sec.~\ref{sec-chap2-one-body-density-matrix}). Example calculations for the nuclei $\isotope[3]{He}$ and $\isotope[4]{He}$ are presented, and the calculated results are extrapolated using the infrared extrapolation method (Sec.~\ref{sec-chap2-example-calculations}). We conclude this Chapter with an overview of the steps needed to perform an NCCI calculation using a general single-particle basis (Sec.~\ref{sec-chap2-general-basis}).


\section{Second quantization}
\label{sec-chap2-second-quantization}


Second quantization is used to describe systems of many identical particles. In what follows the notational conventions of Negele are used~\cite{negele1988:many-particle}.


The Hilbert space of $A$ distinguishable particles $ \mathcal{H}^{A}$ is spanned by the tensor product of $A$ distinguishable particles occupying single-particle states which belong to the single-particle Hilbert space $\mathcal{H}$ 
\begin{equation}
\mathcal{H}^{A} = \mathcal{H} \otimes \mathcal{H} \otimes \ldots \otimes \mathcal{H}.
\label{eqn-chap2-hilbert-space-product}
\end{equation}
If $\left\{ | a \rangle \right\}$ is an orthonormal basis for $\mathcal{H}$, an orthonormal basis for $\mathcal{H}^{A}$ can be constructed as the set of tensor product states
\begin{equation}
| a_{1} \ldots a_{A} ) \equiv |a_{1} \rangle \otimes |a_{2} \rangle \otimes \ldots \otimes |a_{A} \rangle,
\label{eqn-chap2-many-body-basis-product}
\end{equation}
where the curved parenthesis on the left hand side of (\ref{eqn-chap2-many-body-basis-product}) denotes that the many-body state is a simple product of single-particle states (i.e., no assumptions are made about the symmetry of the many-body state). 


The space of $A$ indistinguishable fermions $\mathcal{F}^{A}$ is spanned by fully antisymmetric many-body states constructed using the many-body states of $\mathcal{H}^{A}$  
\begin{equation}
| a_{1} \ldots a_{A} \rangle = \frac{1}{\sqrt{A!}} \sum_{P} (-1)^{P} | a_{P_{1}} \rangle \otimes | a_{P_{2}} \rangle \otimes \ldots \otimes | a_{P_{A}} \rangle.
\label{eqn-chap2-many-body-basis-antisymmetric}
\end{equation} 
The sum over $P$ is a sum over all possible permutations $(P_{1},\,P_{2},\ldots,P_{A})$ of the set $(a_{1},\,a_{2},\,\ldots, a_{A})$. Moreover, $(-1)^{P}$ is determined by counting the number of transpositions of two elements which brings a permutation to its original form $(a_{1},\,a_{2},\,\ldots, a_{A})$. 


The Fock space $F$ for fermions is the (Hilbert) direct sum of the fermion spaces $\mathcal{F}^{0}$, $\mathcal{F}^{1}$, $\mathcal{F}^{2}$, $\ldots$, $\mathcal{F}^{A}$, $\ldots$ for zero, one, two, etc particles
\begin{equation}
F = \mathcal{F}^{0} \oplus \mathcal{F}^{1} \oplus \mathcal{F}^{2} \oplus \ldots \oplus \mathcal{F}^{A} \oplus \ldots.
\label{eqn-chap2-fock-space}
\end{equation}
Here $\mathcal{F}^{0}$ is the space of no particles, $\mathcal{F}^{1}$ is identical to $\mathcal{H}$, and $\mathcal{F}^{A}$ with $A \geq 2$ is the space spanned by many-body states given by (\ref{eqn-chap2-many-body-basis-antisymmetric}).


Creation and annihilation operators generate the entire Fock space $F$ by adding (removing) single-particle states to (from) many-body states. The fermionic creation operator $c_{a}^{\dagger}$ adds a particle in a single-particle state $| a \rangle$ to the many-body state $| a_{1} \ldots a_{A} \rangle$ as follows
\begin{equation}
c_{a}^{\dagger} | a_{1} a_{2} \ldots a_{A} \rangle = | a a_{1} a_{2} \ldots a_{A} \rangle,
\label{eqn-chap2-creation-operator}
\end{equation}
where the definition implies that the particle is added to the left of the initial many-body state. Now, because of the antisymmetry requirement for fermions we cannot act with the $c_{a}^{\dagger}$ operator on the state $| a a_{1} a_{2} \ldots a_{A} \rangle$ (and thus add the single-particle state $| a \rangle$ twice). This state is equal to zero by definition
\begin{equation}
c_{a}^{\dagger} |a a_{1} a_{2} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-creation-operator-2}
\end{equation}
Similarly an annihilation operator $c_{a}$ removes a particle occupying the single-particle state $|a\rangle$ from a many-body state
\begin{equation}
c_{a} |a a_{1} \ldots a_{A} \rangle = | a_{1} \ldots a_{A} \rangle.
\label{eqn-chap2-annihilation-operator}
\end{equation}
For completeness, note that in general $c_{a} | a_{1} a_{2} \ldots a \ldots a_{A} \rangle = (-1)^{P} | a_{1} a_{2} \ldots a_{A} \rangle$ where $P$ is the number of transpositions of two elements needed to bring the particle in the single-particle state $| a \rangle$ to the front of the many-body state. For example $c_{a_{2}} | a_{1} a_{2} a_{3} \rangle = - |a_{1} a_{3} \rangle$. If $c_{a}$ acts on a state $| a_{1} \ldots a_{A} \rangle$, i.e., a state which has no particle in the single-particle state $| a \rangle$, then the action of $c_{a}$ on the many-body state $| a_{1} \ldots a_{A} \rangle$ yields zero
\begin{equation}
c_{a} |a_{1} \ldots a_{A} \rangle = 0.
\label{eqn-chap2-annihilation-operator-2}
\end{equation}
Following from~(\ref{eqn-chap2-creation-operator})-(\ref{eqn-chap2-annihilation-operator-2}), we conclude that the creation and annihilation operators obey the fermionic anticommutation relation
\begin{equation}
\lbrace c_{a} , c_{b}^{\dagger} \rbrace = \delta_{ab}.
\label{eqn-chap2-anti-commutation}
\end{equation}


One-body operators are operators which can be written as a sum of single-particle operators acting on one particle at a time. To be able to calculate the matrix elements of one-body operators with respect to many body states like (\ref{eqn-chap2-many-body-basis-antisymmetric}), it is useful to express them in terms of creation and annihilation operators. To arrive at this expression, let us first use the many-body states of $\mathcal{H}^{A}$ to calculate the matrix elements of a one-body operator $T = \sum_{i=1}^{A} t_{i}$. For the diagonal matrix elements (i.e., between the same many-body states) we have
\begin{multline}
( a_{1}a_{2} \ldots a_{A} | T | a_{1} a_{2} \ldots a_{A} ) = \\  
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2} \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \\
\langle a_{1} | t_{1} | a_{1} \rangle + \ldots + \langle a_{A} | t_{A} | a_{A} \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-identical-states}
\end{multline}
where we used the fact that the single-particle states are orthonormal hence $\langle a_{i} | a_{j} \rangle = \delta_{a_{i}a_{j}}$. Let us now evaluate the non-diagonal matrix elements of $T$ starting with the matrix elements between the many-body state $ | a_{1} a_{2} \ldots a_{A} )$ and the many-body state $ | a_{1} a_{2}' \ldots a_{A} )$, where $| a_{2} \rangle \neq | a_{2}' \rangle$. We have
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1} a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1} \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \langle a_{1} | a_{1} \rangle \langle a_{2} | t_{2} | a_{2}' \rangle \langle a_{3} | a_{3} \rangle \ldots \langle a_{A} | a_{A} \rangle + \\
+ \ldots + \langle a_{1} | a_{1} \rangle \ldots \langle a_{A-1} | a_{A-1} \rangle  \langle a_{A} | t_{A} | a_{A} \rangle = \langle a_{2} | t_{2} | a_{2}' \rangle,
\label{eqn-chap2-one-body-operator-matrix-elements-one-sp-state-different}
\end{multline}
since $\langle a_{2} | a_{2}' \rangle = 0 $. Finally, the matrix elements of $T$ between the many-body states $| a_{1} a_{2} \ldots a_{A} )$ and $| a_{1}' a_{2}' \ldots a_{A} )$, where $| a_{1} \rangle \neq | a_{1}' \rangle$ and $| a_{2} \rangle \neq | a_{2}' \rangle$, are
\begin{multline}
( a_{1} a_{2} \ldots a_{A} | T | a_{1}' a_{2}' \ldots a_{A} ) = \\
\langle a_{1} | t_{1} | a_{1}' \rangle \langle a_{2} | a_{2}' \rangle \ldots \langle a_{A} | a_{A} \rangle + \ldots + \langle a_{1} | a_{1}' \rangle \ldots \langle a_{A} | t_{A} | a_{A} \rangle = 0.
\label{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}
\end{multline}
Thus, the matrix elements of the one-body operator $T$ with respect to many-body states of $\mathcal{H}^{A}$ are fully defined by the sum over single-particle matrix elements of $\mathcal{H}$. If we now define the single-particle vacuum state $| - \rangle$ (i.e., a non-occupied single-particle state), then $c_{a}^{\dagger} | - \rangle = | a \rangle$. Using this definition and (\ref{eqn-chap2-one-body-operator-matrix-elements-identical-states})-(\ref{eqn-chap2-one-body-operator-matrix-elements-two-sp-state-different}) we can write a one-body operator as
\begin{equation}
T = \sum_{ab} t_{ab} c_{a}^{\dagger} c_{b},
\label{eqn-chap2-one-body-operator-second-quantization}
\end{equation}
where $t_{ab} = \langle a | t | b \rangle$.

Similarly, the matrix elements of a two-body operator $V = \frac{1}{2} \sum_{i \neq j} u_{ij}$ with respect to the many-body states of $ \mathcal{H}^{A}$ are fully defined by the matrix elements $u_{abcd} = (ab | u | cd )$ calculated using the states of $\mathcal{H}^{2}$. Thus we can write $V$ as
\begin{equation}
V = \frac{1}{2} \sum_{abcd} u_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c}.
\label{eqn-chap2-interaction-second-quantized}
\end{equation}
However, it is more convenient to write the two-body operator as
\begin{equation}
V = \frac{1}{4} \sum_{abcd} \bar{u}_{abcd} c_{a}^{\dagger} c_{b}^{\dagger} c_{d} c_{c},
\label{eqn-chap2-interaction-second-quantized-antisymmetrized}
\end{equation}
where $\bar{u}_{abcd} = u_{abcd} - u_{abdc} = \langle ab | u | cd \rangle$ are normalized and antisymmetrized two-body matrix elements.


\section{Two-body matrix elements for the NCCI Hamiltonian}
\label{sec-chap2-tbme}

In the context of the NCCI approach, the most commonly used single-particle states are the harmonic oscillator single-particle basis states (see Sec.~\ref{sec-chap2-harmonic-oscillator-radial-functions}). A harmonic oscillator single-particle state is labeled by the quantum numbers $| \alpha \rangle \equiv |n_{a}l_{a}j_{a}m_{a} \rangle$, where $n_{a}$ is the harmonic oscillator radial quantum number, $l_{a}$ is the angular momentum, $j_{a}$ is the total angular momentum, and $m_{a}$ is the $z$ projection of the total angular momentum. Using the harmonic oscillator single-particle states we can construct fully antisymmetric many-body basis states for the NCCI approach
\begin{equation}
| (n_{a}l_{a}j_{a}m_{a}) (n_{b}l_{b}j_{b}m_{b}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle.
\label{eqn-chap2-many-body-state-harmonic-oscillator}
\end{equation} 
Many-body states such as (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) have a total $z$ projection of total angular momentum $M=\sum_{i=1}^{A} m_{i}$ and a total number of oscillator quanta $N_{\mathrm{tot}}=\sum_{i=1}^{A} (2n_{i} + l_{i}) = \sum_{i=1}^{A} N_{i}$. The harmonic oscillator single-particle states $| \alpha \rangle$ are given as the tensor product 
\begin{equation}
| \alpha \rangle = \left[| R_{n_{a} l_{a}} Y_{l_{a}} \rangle \times |\frac{1}{2} \rangle \right]_{j_{a}m_{a}},
\label{eqn-oscillator-orbitals-second-quantization}
\end{equation}
where $R_{n_{a}l_{a}}$ is a harmonic oscillator radial function, $Y_{l_{a}}$ is a spherical harmonic, and $|\frac{1}{2} \rangle$ is a spinor. The subscripts $j_{a}$ and $m_{a}$ indicate that $| R_{n_{a} l_{a}} Y_{l_{a}} \rangle$ (a spherical tensor of rank $l_{a}$) and the spinor $| \frac{1}{2} \rangle$ are coupled to total angular momentum $j_{a}$ and $z$ projection of total angular momentum $m_{a}$~\cite{rose1957:am}. 


The Hilbert space of the NCCI Hamiltonian is spanned by the many-body states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) which provide a basis for the representation of the Hamiltonian as a square matrix. To cast the Hamiltonian into a square matrix we must first calculate the two-body matrix elements of the relative kinetic energy and two-body $NN$ interaction operators. The two-body matrix elements are calculated with respect to two-particle states, coupled to total angular momentum $J$. For distinguishable particles (e.g., one proton and one neutron states), angular momentum coupled two-particle states are defined as 
\begin{equation}
| a b ; J ) = \sum_{m_{a}m_{b}} \langle j_{a} m_{a} j_{b} m_{b} | J M \rangle |a m_{a} \rangle | b m_{b} \rangle,
\label{eqn-chap2-two-particle-states-1}
\end{equation}
where $| a m_{a} \rangle = | n_{a} l_{a} j_{a} m_{a} \rangle$, $\langle j_{a} m_{a} j_{b} m_{b} | J M \rangle $ is a Clebsch-Gordan coefficient, and the parenthesis implies that the two-particle state is not antisymmetrized. For two identical fermions we can obtain fully antisymmetrized states using the states $| a b ; J )$. We have
\begin{equation}
| a b ; J M \rangle_{\mathrm{AS}} = \frac{1}{\sqrt{2}} \left[ | a b ; J M ) - (-1)^{J - j_{a} - j_{b}} | b a ; J M \rangle \right].
\label{eqn-chap2-two-particle-states-2}
\end{equation}
These states have the symmetry property $| a b ; J M \rangle = - (-1)^{J -j_{a}-j_{b}} | b a ; J M \rangle$ which implies that if the states $| a \rangle$ and $| b \rangle$ are identical, only two-body states with even $J$ are allowed. The states (\ref{eqn-chap2-two-particle-states-2}) are antisymmetrized but not strictly normalized. An extra factor of $1 / \sqrt{2}$ is required for normalization in the special case when the two particles occupy the same single-particle orbital $| n_{a} l_{a} j_{a} \rangle$. Hence, the appropriate two-particle states are
\begin{equation}
| a b ; J M \rangle_{\mathrm{NAS}} = (1 + \delta_{ab})^{-1/2} | a b ; J M \rangle_{\mathrm{AS}}.
\label{eqn-chap2-two-particle-states-3}
\end{equation}
Both the normalized antisymmetrized states and the antisymmetrized states are used to calculate the two-body matrix elements $\langle c d ; J | H_{\mathrm{in}} | a b ; J \rangle$ of the (scalar) intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}). The change of basis relation between two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-2}) and two-body matrix elements calculated with respect to the states (\ref{eqn-chap2-two-particle-states-3}) is
\begin{equation}
\langle c d ; J | H | a b ; J \rangle_{\mathrm{NAS}} = (1+\delta_{cd})^{-1/2} (1+\delta_{ab})^{-1/2} \langle c d ; J | H | a b ; J \rangle_{\mathrm{AS}}.
\label{eqn-chap2-nas-two-body-matrix-elements}
\end{equation}
A detailed discussion about the calculation of the two-body matrix elements of the intrinsic Hamiltonian (\ref{eqn-chap2-overview-hamiltonian}) is given in Ref.~\cite{caprio2012:csbasis}. A brief overview is also given in Sec.~\ref{sec-chap2-general-basis}.
 

\section{The harmonic oscillator single-particle states}
\label{sec-chap2-harmonic-oscillator-radial-functions}


In this section we will review the basic properties of the harmonic oscillator single-particle states $| \alpha \rangle$~\cite{suhonen2007:nucleons-nucleus,moshinsky1996:oscillator,weniger1985:fourier-plane-wave} which are traditionally used in the NCCI approach because their properties facilitate the many-body calculations. The harmonic oscillator single-particle states are also our starting basis for the construction of natural orbitals which are introduced in Chapter~\ref{chap-chap3}. 


The first important property of the harmonic oscillator single-particle states (relevant to the NCCI approach) is that they allow for the complete removal of spurious center-of-mass states from the low-lying spectrum of the NCCI Hamiltonian provided that an $\Nmax$ truncation is imposed on the many-body basis. The appearance of spurious center-of-mass states results from using the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) for the representation of the NCCI Hamiltonian as a square matrix. A detailed discussion about the appearance of spurious center-of-mass states in an NCCI calculation and the procedure followed for their removal from the low-lying spectrum is given in Sec.~\ref{sec-chap2-many-body-basis}.

The second important property of the harmonic oscillator single-particle states (relevant to many-body calculations and consequently the NCCI approach) is that they simplify the calculation of two-body matrix elements for operators written in terms of relative coordinates, using the Moshinsky transformation~\citep{moshinsky1996:oscillator}. According to  the transformation, products of harmonic oscillator states expressed in single-particle coordinates $R_{n_{1}l_{1}}(\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ transform into products of harmonic oscillator states expressed in terms of relative and center-of mass coordinates $R_{nl}(\mathbf{r}_{\mathrm{rel}})R_{NL}(\mathbf{R})$, where $2 n_{1} + l_{1} + 2 n_{2} + l_{2}= 2 n + l+ 2 N + L$, $\mathbf{r}_{\mathrm{rel}} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}-\mathbf{r}_{2})$, and $\mathbf{R} = \frac{1}{\sqrt{2}} (\mathbf{r}_{1}+\mathbf{r}_{2})$. (The factor of $1/\sqrt{2}$ in front of the center-of-mass vector is used instead of the traditional $1/2$ for normalization reasons). The calculation of two-body matrix elements for operators of the form $V(\mathbf{r}_{1}-\mathbf{r}_{2})$ with respect to two-particle states of the form $R_{n_{1}l_{1}} (\mathbf{r}_{1}) R_{n_{2}l_{2}}(\mathbf{r}_{2})$ is then reduced to the calculation of the single-particle matrix element of the operator $V(\mathbf{r}_{\mathrm{rel}})$ with respect to single-particle states of the form $R_{nl}(\mathbf{r}_{\mathrm{rel}})$ and an overlap between single-particle states of the form $R_{NL}(\mathbf{R})$.

Let us now review the harmonic oscillator radial wave functions. If we write the single-particle wave function as $\Psi_{nlm}(\mathbf{r})=r^{-1} R_{nl}(b;r)Y_{lm}(\theta,\phi)$, where $R_{nl}(b;r)$ are radial wave functions and $Y_{lm}(\theta,\phi)$ are spherical harmonics, then $\Psi_{nlm}(\mathbf{r})$ are solutions to the familiar harmonic oscillator central force problem \cite{suhonen2007:nucleons-nucleus} 
\begin{equation}
h(\omega) = \frac{p^{2}}{2m_{\mathrm{N}}} + \frac{m_{\mathrm{N}} \omega^{2} r^{2}}{2}.
\label{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}
\end{equation} 
where $m_{\mathrm{N}}c^{2} \approx 938.92$ MeV is the average nucleon mass and $\omega$ is the oscillator frequency. The length scale of the radial functions $R_{nl}(b;r)$ is set by the oscillator length $b$ which depends on the parameters of the oscillator Hamiltonian (\ref{eqn-chap2-harmonic-oscillator-one-body-hamiltonian}) as $b=\sqrt{\hbar / (m_{\mathrm{N}} \omega})$. The eigenvalues corresponding to each single-particle radial wave function are given by $ (N + 3/2) \hw$, where $N = 2n + l$ is the oscillator quantum (notice that the eigenvalues are evenly spaced by one unit of $\hw$). The radial functions $R_{nl}(b;r)$ are given by
\begin{equation}
R_{nl}(b;r) = b N_{nl} (r/b)^{l+1} L_{n}^{l+1/2}[(r/b)^{2}] e^{-(r/b)^{2}/2},
\label{eqn-chap2-harmonic-oscillator-radial-functions}
\end{equation} 
where $L_{n}^{l+1/2}[(r/b)^{2}]$ are generalized Laguerre polynomials, $n$ is the radial quantum number (which gives the number of nodes in the radial function), $l$ is the angular momentum, and $N_{nl}$ is a normalization factor given by
\begin{equation}
N_{nl} = \frac{1}{b^{3/2}} \left[ \frac{2n!}{(l+n+1/2)!} \right]^{1/2}.
\label{eqn-chap2-harmonic-oscillator-functions-normalization}
\end{equation}
For each $l$, the harmonic oscillator radial functions form a complete discrete basis for square integrable functions on $ \mathbb{R}^{+}$
\begin{equation}
\int_{0}^{\infty} R_{nl}(b;r) R_{n'l}(b;r) = \delta_{nn'}.
\label{eqn-chap2-ho-orthonormal}
\end{equation}
 

\section{Symmetries of the NCCI Hamiltonian and the nuclear \\ many-body basis}
\label{sec-chap2-many-body-basis}


The selection of the nuclear many-body basis used in NCCI calculations is based on the symmetries of the NCCI Hamiltonian~(\ref{eqn-chap2-overview-hamiltonian}). The NCCI Hamiltonian is rotationally invariant therefore it conserves the total angular momentum $J$ and the $z$ projection of total angular momentum $M$. Moreover, the Hamiltonian conserves parity. To diagonalize the Hamiltonian we can choose to use many-body states that have good $J$ (a $J$-scheme basis) or many-body states that have good $M$ (an $M$-scheme basis)~\cite{whitehead1977:shell-methods}. Although the $M$-scheme basis involves a larger number of many-body basis states compared to a $J$-scheme basis, constructing $M$-scheme many-body basis states is straightforward (i.e., we do not have to deal with angular momentum coupling as in the $J$-scheme basis). Therefore, for the NCCI calculations discussed here, an $M$-scheme basis is considered. However, the eigenstates of $H$ still have good $J$ which is recovered after diagonalization by calculating the expectation value of the $J^{2}$ operator with respect to the calculated many-body wave function.


To build many-body basis states we start from single-particle states $| nljm \rangle$ and construct fully antisymmetric states (with good $M$) given by~(\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Calculations can be performed for any possible value of $M$ (which is supported by the single-particle states in the many-body basis). For example, for even nuclei $M=0, 1,\ldots$ and for odd nuclei $M=1/2, 3/2, \ldots$ (we do not consider negative values for $M$ here). However, we usually use many-body states with $M=0$ for even nuclei and $M=1/2$ for odd nuclei. This is because for a given $M$ we can only obtain many-body wave functions with $J \geq | M |$. Thus, choosing the lowest possible $M$ allows us to study the ground and first few excited states of a nucleus.


Commonly, for reasons involving the center-of-mass degree of freedom, as discussed in Sec.~\ref{sec-chap2-com-factorization}, the many-body basis is truncated using the $\Nmax$ truncation scheme~\cite{elliott1955:com-shell}. The scheme dictates that only many-body states with $\Ntot \leq N_{0} + \Nmax$ are permitted in the many-body basis, where $N_{0}$ is the number of quanta in the configuration where all the nucleons occupy the lowest permitted oscillator shells. For example, $N_{0}=2$ for $\isotope[6]{He}$ (in this configuration, the two protons occupy the $N=0$ proton shell, two neutrons occupy the $N=0$ neutron shell, and the last two neutrons occupy the $N=1$ shell) and $N_{0} =3$ for $\isotope[7]{Li}$ (because the extra proton compared to $\isotope[6]{He}$ goes into the $N=1$ proton shell). 




Finally, because the nuclear Hamiltonian conserves parity we want our many-body basis to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. A many-body basis truncated at a given $\Nmax$ contains (many-body) states with $N_{\mathrm{tot}} \leq N_{0} + \Nmax$, where $N_{\mathrm{tot}} = \sum_{i} N_{i} = N_{1} + \ldots + N_{A}$, and $N_{i}$ is the oscillator quantum of a nucleon $i$ in its single-particle state. Hence, many-body basis states which belong to this (many-body) basis have parity which is obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the many-body states of the lowest allowed configuration is $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity eigenstates of the nucleus we must build many-body bases with even $\Nmax$ truncations, i.e., $\Nmax = 0, 2, 4, \ldots$. On the other hand, to obtain the unnatural parity eigenstates of the nucleus we must construct many-body bases with odd $\Nmax$ truncations, i.e., $\Nmax = 1, 3, 5, \ldots$. 

%Finally, because the nuclear Hamiltonian conserves parity we want our many-body basis to have good parity. Recall that the parity of a harmonic oscillator single-particle state is given by $(-1)^{l}$, or, equivalently, $(-1)^{N}$ since $N=2n+l$. This means that the parity of a many-body state which belongs to the many-body basis can be obtained as the product $(-1)^{N_{1}}\ldots (-1)^{N_{A}} = (-1)^{\Ntot}$. The parity of the lowest possible configuration is given by $(-1)^{N_{0}}$, which we call the natural parity of the nucleus. Thus, to obtain the natural parity states of the nucleus $\Nmax$ must be even and proceed in steps of $2$, i.e., $\Nmax = 2, 4, 6, \ldots$. On the other hand, to obtain the unnatural parity states of the nucleus $\Nmax$ must be odd and also proceed in steps of $2$, i.e., $\Nmax = 1, 3, 5, \ldots$. 






\section{Spurious center-of-mass states removal}
\label{sec-chap2-com-factorization}


In this section we describe how spurious center-of-mass states result from the diagonalization of the NCCI Hamiltonian matrix built in terms of the set of the many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Subsequently, we describe how these spurious states can be removed provided that the $\Nmax$ truncation scheme is used.

The many-body basis states (\ref{eqn-chap2-many-body-state-harmonic-oscillator}) are defined with respect to a fixed point in space. However, physically there is no such point around which all the nucleons are orbiting. Rather we are interested in the internal motion of the nucleons relative to each other within the nucleus, a motion which defines the intrinsic structure of the nucleus.


In principle we can convert to relative coordinates. However, antisymmetrization in Jacobi coordinates (which define the relative motion) is cumbersome. Therefore, we are compelled to work in the full coordinate space which includes both the center of mass and relative degrees of freedom.


Our goal is to describe the relative motion as accurately as possible without unnecessary complications arising from the center of mass motion. In order to accomplish this it helps making certain choices regarding the basis and the Hamiltonian.


We want our eigenfunctions to factorize into center of mass and relative factors. We also want the center of mass factor to be simple and well understood so that it does not interfere with the calculation of energies and observables. In principle, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) is already separated into center of mass and relative coordinates. If we define the center-of-mass momentum as $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, the one-body kinetic energy operator in (\ref{eqn-chap2-overview-full-hamiltonian}) can be decomposed into a center-of-mass and a relative kinetic energy contributions~\cite{vanhees:1983}
\begin{equation}
T = T_{\mathrm{c.m.}} + T_{\mathrm{rel}} = \frac{\left(\sum\limits_{i=1}^{A}\mathbf{p}_{i}\right)^{2}}{2Am_{\mathrm{N}}}  + \sum_{i \neq j}^{A} \frac{(\mathbf{p}_{i}-\mathbf{p}_{j})^{2}}{4 A m_{\mathrm{N}}}.
\label{eqn-chap2-kinetic-energy-decomposition}
\end{equation}
Therefore, the full Hamiltonian (\ref{eqn-chap2-overview-full-hamiltonian}) also separates into center-of-mass and relative parts
\begin{equation}
H= T_{\mathrm{c.m.}} + (T_{\mathrm{rel}} + V).
\label{eqn-chap2-full-separated-hamiltonian}
\end{equation}
Thus, in the full space our eigenfunctions would factorize into a center-of-mass and a relative wave function.

However, we are confined to work in a truncated space. Factorization can still be exact in an oscillator basis when the $\Nmax$ truncation is used. The truncated space then only contains a limited center-of-mass space spanned by center-of-mass harmonic oscillator states with $N_{\mathrm{c.m.}} = 0$, $2$, $\ldots, \Nmax$. We could attempt to diagonalize the Hamiltonian~(\ref{eqn-chap2-full-separated-hamiltonian}) in the truncated space. However, the $T_{\mathrm{c.m.}}$ operator will mix contributions with different center-of-mass excitations $N_{\mathrm{c.m.}}$ and destroy factorization of the eigenfunctions. The Hamiltonian will force us towards states which attempt to diagonalize the center-of-mass kinetic energy operator $T_{\mathrm{c.m.}}$. Therefore, our NCCI calculations would end up approximating spherical waves in the center of mass coordinates, at the expense of accurately describing the intrinsic motion.

Thus, instead, we choose to work with the intrinsic Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V.
\end{equation} 
The resulting Hamiltonian is block diagonal with respect to the number of quanta $N_{\mathrm{c.m.}}$ for the center-of-mass motion. The resulting eigenfunctions will factorize into a center-of-mass factor of good $N_{\mathrm{c.m.}}$ and an intrinsic factor. The total number of quanta in a many-body state is shared between the center-of-mass motion and the intrinsic motion:
\begin{equation}
\Ntot = \sum_{i} N_{i} = N_{\mathrm{c.m.}} + N_{\mathrm{rel}}.
\label{eqn-chap2-number-of-quanta-com-quanta}
\end{equation}
Therefore, in eigenfunctions with $N_{\mathrm{c.m.}} = 0$, the full $\Nmax$ quanta are available to use in describing the intrinsic motion. The higher $N_{\mathrm{c.m.}}$ eigenfunctions produce spurious copies of the spectrum in which the intrinsic motion is described using fewer quanta $N_{\mathrm{rel}} \leq \Nmax - N_{\mathrm{c.m.}}$. 


It is convenient to push the spurious excited center-of-mass states out of the low lying spectrum. We do this by adding a term diagonal in the number of center-of-mass quanta. That is we add a ``Lawson term''~\cite{gloeckner1974:spurious-com} proportional to the $N_{\mathrm{c.m.}}$ operator. This is often equivalently described as adding a center-of-mass harmonic oscillator Hamiltonian. In terms of the center-of-mass coordinate $\mathbf{R} = (\sum_{i} \mathbf{r}_{i})/A$ and the center-of-mass momentum $\mathbf{P} = \sum_{i} \mathbf{p}_{i}$, 
\begin{equation}
H_{\mathrm{c.m.}} = \frac{P^{2}}{2Am_{\mathrm{N}}} + \frac{1}{2} A m_{\mathrm{N}} \omega^{2} R^{2}.
\label{eqn-chap2-harmonic-oscillator-many-body-hamiltonian-com}
\end{equation}
Then, $H_{\mathrm{c.m.}} = (N_{\mathrm{c.m.}} + 3/2)\hbar \omega$. Thus we actually diagonalize the Hamiltonian
\begin{equation}
H = T_{\mathrm{rel}} + V + \alpha N_{\mathrm{c.m.}},
\label{eqn-chap2-ncci-hamiltonian-with-lawson}
\end{equation} 
where $\alpha$ is the Lawson term strength (typically a few MeV). This leads to the same eigenstates as the relative Hamiltonian but with the spurious states lifted out of the low-lying spectrum by an amount $\alpha N_{\mathrm{c.m.}}$.




\section{Many-body calculations}
\label{sec-chap2-many-body-calculations}


In this section we will briefly describe the general procedure followed to obtain results using the NCCI approach.

The basic ingredient needed to build the Hamiltonian matrix is the two-body matrix elements of the NCCI Hamiltonian (\ref{eqn-chap2-ncci-hamiltonian-with-lawson}) with respect to many-body basis states like (\ref{eqn-chap2-many-body-state-harmonic-oscillator}). Thus, we need to evaluate matrix elements of the form
\begin{equation}
\langle \Phi_{n} | H | \Phi_{m} \rangle,
\label{eqn-chap2-two-body-matrix-elements}
\end{equation}
where $| \Phi_{n} \rangle = | (n_{1}l_{1}j_{1}m_{1}) \ldots (n_{A}l_{A}j_{A}m_{A}) \rangle$ is a many-body basis state. [The matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) reduce to a sum over two-body matrix elements of the form $\langle c d ; J | H | a b ; J \rangle$ using Wick's theorem]. After calculating the matrix elements (\ref{eqn-chap2-two-body-matrix-elements}) for all the many-body states in our basis we obtain the Hamiltonian matrix
\begin{equation}
  \begin{pmatrix}
    \langle \Phi_{1} | H | \Phi_{1} \rangle & \langle \Phi_{1} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{1} | H | \Phi_{m} \rangle \\
    \langle \Phi_{2} | H | \Phi_{1} \rangle & \langle \Phi_{2} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{2} | H | \Phi_{m} \rangle \\
    \vdots & \vdots & \ddots & \vdots \\
   \langle \Phi_{d} | H | \Phi_{1} \rangle & \langle \Phi_{d} | H | \Phi_{2} \rangle & \ldots & \langle \Phi_{d} | H | \Phi_{d} \rangle
  \end{pmatrix}
\label{eqn-chap2-ncci-hamiltonian-matrix}
\end{equation}
The dimension $d$ of the matrix (\ref{eqn-chap2-ncci-hamiltonian-matrix}) is equal to the number of many-body basis states for a given nucleus and $\Nmax$ truncation (see Fig.~\ref{fig-chap1-NNCI-dimension}). Diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}) yields the nuclear many-body wave function
\begin{equation}
| \Psi \rangle = \sum\limits_{n=1}^{d} c_{n} | \Phi_{n} \rangle.
\label{eqn-chap2-ncci-wave-functions}
\end{equation}
%where $c_{n}$ are coefficients obtained from the diagonalization of (\ref{eqn-chap2-ncci-hamiltonian-matrix}).


The diagonalization of the Hamiltonian matrix is commonly performed using the Lanczos algorithm~\cite{komzsik2003:lanczos-method,lanczos1950:algorithm}. The algorithm transforms the generally large sparse matrix (\ref{eqn-chap2-ncci-wave-functions}) into a tridiagonal matrix (of lower dimension than the original matrix). The tridiagonal matrix is then diagonalized (using an appropriate algorithm) and the eigenvalues and eigenvectors (of the tridiagonal matrix) are obtained. The eigenvectors of the tridiagonal matrix (Lanczos vectors) must then be converted from the Lanczos vector space to the original many-body basis. The process established by Lanczos proceeds as follows: If $H$ is a Hamiltonian matrix of order $n$ (i.e., the matrix dimension is $n \times n$), then we start with a random initial vector $b_{0}$ which is used to construct $m$ vectors (orthogonal to each other) according to the algorithm
\begin{align}
b_{0} & = \mathrm{random}, \nonumber & \\
b_{1} & = (H - \alpha_{0}) b_{0}, \nonumber \\
b_{2} & = (H - \alpha_{1}) b_{1} - \beta_{0} b_{0}, \nonumber \\
b_{3} & = (H - \alpha_{2}) b_{2} -\beta_{1} b_{1}, \nonumber \\
 \vdots  \nonumber & \\
b_{m} & = (H - \alpha_{m-1}) b_{m-1} - \beta_{m-2} b_{m-2} = 0,
\label{eqn-chap2-lanczos-algorithm}
\end{align}
where $m \leq n$. The equality to zero in the last step means the end of the process. The coefficients $\alpha_{m-1}$ and $\beta_{m-2}$ are determined by requiring that the norm of the vector $\parallel b_{m} \parallel$ is minimized. The coefficients are then used to build the tridiagonal matrix 
\begin{equation}
T =  \begin{pmatrix}
\alpha_{0} & \beta_{0} &   &   & 0\\ 
\beta_{0}  & \alpha_{1} & \beta_{1} & \\
                 & \ddots & \ddots & \ddots & \\
                 &  & \beta_{k-2} & \alpha_{k-1} &\beta_{k-1} \\
           0      & & & \beta_{k-1} & \alpha_{k}
  \end{pmatrix}
\label{eqn-chap2-tridiagonal-matrix}
\end{equation}
The eigenvalues of $T$ converge to the eigenvalues of $H$ provided that a sufficient number of iterations $k$, where $k < n$, is performed. 


The generally large sizes of the NCCI Hamiltonian matrices require the use of parallel computing which handles both the storage and the diagonalization of the Hamiltonian matrix. For the calculations presented in this thesis, we use the parallel code Many Fermion Dynamics-Nuclear (MFDn) \cite{maris2010:ncsm-mfdn-iccs10,vary2009:ncsm-mfdn-scidac09} developed by the Iowa State University group handles the construction of the many-body basis, the construction of the Hamiltonian matrix, the storage of the matrix over multiple cores, and the Lanczos diagonalization of the matrix. The input to the code includes the two-body matrix elements of the Hamiltonian, the $\Nmax$ truncation of the many-body basis, the number of protons ($Z$) and neutrons ($N$) of the nucleus we want to study, the number of Lanczos iterations we want to perform, and various other control parameters. The program outputs the eigenvalues (which are the nuclear level energies), the one-body density matrices (described in Sec.~\ref{sec-chap2-one-body-density-matrix}), and other observables.


\section{The one-body density matrix}
\label{sec-chap2-one-body-density-matrix}


The one-body density matrix can be calculated using the many-body wave functions obtained in a many-body calculation. It is more frequently used for the calculation of the matrix elements of one-body operators~\cite{suhonen2007:nucleons-nucleus}. Moreover, the static one-body density matrix contains information about correlations in the many-body wave function as described below. In second quantization, the transition one-body density matrix is given by
\begin{equation}
\rho_{\alpha\beta}^{\mathrm{f\,i}} = \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger} c_{\beta} | \Psi_{\mathrm{i}} \rangle,
\label{eqn-chap2-one-body-density-operator}
\end{equation}
where $| \Psi_{\mathrm{i}} \rangle$ and $| \Psi_{\mathrm{f}} \rangle$ are the many-body wave functions of an initial and a final nuclear state respectively. Using (\ref{eqn-chap2-one-body-density-operator}), the matrix elements of a one-body operator $\mathcal{O}$ are obtained as
\begin{equation}
\langle \Psi_{\mathrm{f}} | \mathcal{O} | \Psi_{\mathrm{i}} \rangle =  \sum_{\alpha\beta} \langle \alpha | \mathcal{O} | \beta \rangle \langle \Psi_{\mathrm{f}} | c_{\alpha}^{\dagger}c_{\beta} | \Psi_{\mathrm{i}} \rangle.
\label{eqn-chap2-one-body-operator-matrix-elements}
\end{equation}


The static one-body density matrix (i.e., the one-body density matrix obtained for the same initial and final many-body wave functions) contains information about correlations in the many-body wave function. By definition, an uncorrelated many-body wave function can be written as a single Slater determinant, i.e., $| \Psi \rangle = | a_{1} \ldots a_{A} \rangle$. For an uncorrelated many-body wave function, it is easy to see that the diagonal matrix elements $\rho_{\alpha\alpha} = \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle $ are equal to $1$ (which reflects the fact that each single-particle state is occupied by exactly one nucleon), while all the off diagonal matrix elements $\rho_{\alpha\beta}$ are equal to $0$. The sum of the diagonal matrix elements is equal to the total number of nucleons $A$ in the many-body wave function. In the case of a correlated many-body wave function, such as the ones calculated in an NCCI calculation, the one-body density matrix is not (in general) diagonal. The off diagonal matrix elements $\rho_{\alpha\beta}$ of the density matrix provide a measure of how correlated the many-body wave function is, while the diagonal matrix elements $\rho_{\alpha\alpha}$ provide the occupancies of each single-particle state $| a_{i} \rangle$ in the many-body wave function. The sum over the diagonal matrix elements is still equal to the total number of nucleons in the many-body wave function
\begin{equation}
\sum_{\alpha} \langle \Psi | c_{\alpha}^{\dagger} c_{\alpha} | \Psi \rangle = A.
\label{eqn-chap2-density-matrix-number}
\end{equation}
It is important to stress here that a diagonal one-body density matrix does not necessarily indicate that a many-body wave function is uncorrelated unless the diagonal matrix elements $\rho_{\alpha \alpha}$ are exactly equal to $1$. The one-body density matrix is the starting point for the construction of natural orbitals in Chapter~\ref{chap-chap3}.


\section{Example calculations and infrared extrapolations}
\label{sec-chap2-example-calculations}


In this section we perform NCCI calculations to obtain the ground state energy and proton radius of the isotopes $\isotope[3,4]{He}$. Our goal is to revisit the convergence properties of NCCI calculations using the harmonic oscillator basis and to extrapolate the calculated results to the full $\Nmax \rightarrow \infty$ space using the infrared extrapolation method which we present and discuss here.


In Fig.~\ref{fig-chap2-helium3-helium4}, we plot the calculated ground state energy (left) and proton radius (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom). Calculations were performed for even truncations of the many-body basis up to $\Nmax = 16$ (in steps of $2$) which scan the $\hw$ range $10$-$40$ MeV. The solid lines correspond to the calculated results, the dashed horizontal lines correspond to the experimental results, and the dotted lines connect extrapolated results obtained using the infrared extrapolation method (discussed below). The experimental binding energies are taken from~\cite{npa-purcell-a-3-data:2010,npa-tilley-a-4-data:1992}, while the proton radii are deduced using the experimentally measured nuclear charge radii reported in~\cite{angeli-marinova-nuclear-charge-radii:2013} and equation ($6$) in Ref.~\cite{bacca2012:6he-hyperspherical}. As we observe, the calculated ground state energy and proton radius of $\isotope[4]{He}$ converge. On the other hand, the calculated ground state energy of $\isotope[3]{He}$ approaches convergence (to the $\sim 0.01$ MeV level), while the proton radius does not converge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{\plotspath /ho_no_comparison/Z2-N1-Z2-N2-rp-e-HO-thesis-chapter1-170227.pdf}
\caption[Calculated ground state energy and proton radius in the ground state of {\protect $\isotope[3]{He}$} and {\protect $\isotope[4]{He}$}, obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The calculated results are extrapolated to the full space using the infrared extrapolation method.]{Calculated ground state energy (left) and proton radius in the ground state (right) of $\isotope[3]{He}$ (top) and $\isotope[4]{He}$ (bottom), obtained using the harmonic oscillator basis, the JISP$16$ $NN$ interaction, the Coulomb interaction between protons, truncations of the many-body basis up to $\Nmax = 16$, and $\hw$ parameters in the range $10$-$40$ MeV. The dashed horizontal lines show the experimental results. The crosses connected by dotted lines are obtained by extrapolating calculated results using the infrared extrapolation method as described in the text.}
\label{fig-chap2-helium3-helium4}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 


Comparisons of NCCI calculations with experimental results are only meaningful once full convergence is achieved. However, when the calculated results do not converge we can attempt to extrapolate results obtained in truncated spaces to the full $\Nmax \rightarrow \infty$ space. One such example was presented in Chapter~\ref{chap-chap1}, where we used an empirical extrapolation method to extrapolate the calculated ground state energy of $\isotope[6]{He}$ to the full space. Here, we use the infrared extrapolation method to extrapolate the calculated ground state energy and proton radius of $\isotope[3,4]{He}$ to the full space. Extrapolating the converged $\isotope[4]{He}$ results serves as a test of the infrared method as we expect the extrapolated results to agree with the converged results.


The infrared extrapolation method~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation, more2013:ir-extrapolation,furnstahl2014:ir-expansion, furnstahl2015:ir-extrapolations,odell-papenbrock-ir-extrapolation-quadruple:2016} starts with the assumption that the truncated many-body basis  induces both a short-range ultraviolet (UV) and a long-range infrared (IR) cutoff on the ability of the many-body basis to describe the many-body wave function. Quantitatively, if the highest occupied single-particle orbital in the many-body basis has $N$ oscillator quanta, then to a first approximation the momentum space (UV) cutoff is~\cite{coon2012:nscm-ho-regulator,furnstahl2012:ho-extrapolation}
\begin{equation}
\Lambda_{\mathrm{UV}} = \sqrt{2(N+3/2)} \,\, \hbar/b,
\label{eqn-chap2-uv-cutoff}
\end{equation}
and the coordinate space (IR) cutoff is
\begin{equation}
L = \sqrt{2(N+3/2)} \,\, b,
\label{eqn-chap2-ir-cutoff}
\end{equation}
where $b$ is the oscillator length.  Assuming that ultraviolet convergence of the calculated results is reached (this typically happens when the ultraviolet cutoff of the internucleon interaction $\lambda$ is smaller than the ultraviolet cutoff $\Lambda_{\mathrm{UV}}$ of the basis), the bound state energies will converge exponentially with respect to $L$
\begin{equation}
E(N_{\mathrm{max}},\hbar\omega) = E_{\infty} +  a_{0} e^{-2 k_{\infty} L(N_{\mathrm{max}},\hbar\omega)},
\label{eqn-chap2-energy-extrapolation-theoretical}
\end{equation}
and the radii will converge as
\begin{equation}
r^{2}(L) = r_{\infty}^{2} [1 - (c_{0}+c_{1}\beta^{-2})\beta^{3}e^{-\beta}],
\label{eqn-chap2-rms-extrapolation}
\end{equation}
where $E_{\infty}$, $a_{0}$, $k_{\infty}$, $c_{0}$, $ c_{1}$, and $r_{\infty}^{2}$ are obtained by fitting (UV converged) calculated results and $\beta = 2k_{\infty} L$ [$k_{\infty}$ is taken from the energy fit in (\ref{eqn-chap2-energy-extrapolation-theoretical})]. The infrared cutoff was later studied in more detail and a more precise expression for $L$ was obtained by finding the lowest eigenvalue of the operator $p^{2}$ in a finite oscillator basis~\cite{more2013:ir-extrapolation} 
\begin{equation}
L(N,\hbar\omega) = \sqrt{2(N+\Delta N + 3/2)} \,\, b(\hbar\omega),
\label{eqn-chap2-ir-length}
\end{equation}
where $\Delta N = 2$ is an offset determined from the diagonalization of $p^{2}$.



The exponential convergence of the bound-state energies with respect to $L$ can be understood as follows~\cite{furnstahl2012:ho-extrapolation}. The finite extent $L$ of the oscillator basis in position space effectively imposes a Dirichlet boundary condition on the bound state wave function at $r = L$. The exponential convergence with respect to $L$ is thus directly related to the exponential fall-off of the bound-state wave functions in position space. 


Let us now use the infrared extrapolation method with our calculated results. Here, we perform a three point extrapolation using the calculated results at $\Nmax=12$, $14$, and $16$ sharing the same $\hw$ parameter. We use results obtained using $\hw$ parameters $\hw \gtrsim 14$ MeV which have large $\Lambda_{UV}$ somewhat comparable to the ultraviolet cutoff $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16}$ of the JISP$16$ interaction~\cite{shirokov2007:nn-jisp16}. Specifically, the JISP$16$ interaction is obtained by fitting scattering data in a harmonic oscillator space with $N=8$ and $\hw = 40$ MeV, which means that according to (\ref{eqn-chap2-uv-cutoff}) $\Lambda_{\mathrm{UV}}^{\mathrm{JISP}16} \approx 800$ $\mathrm{MeV}/c$. For the NCCI calculation with $\Nmax = 12$ and $\hw \approx 14$ MeV equation (\ref{eqn-chap2-uv-cutoff}) yields $\Lambda_{\mathrm{UV}} \approx 600$ $\mathrm{MeV}/c$ which is perhaps too low compared to the UV cutoff of JISP$16$.


In Fig.~\ref{fig-chap2-helium3-helium4}, we show the extrapolated results for the ground state energy [panel (c)] and proton radius [panel (d)] of $\isotope[4]{He}$. As expected, the extrapolated results converge for both observables. A closer inspection reveals that a slight $\hw$ dependence persists which is however very small (at the $0.01$ MeV level and $0.01$ fm level for the extrapolated energy and proton radius respectively). For low $\hw$ parameters, the extrapolated energy does not converge something that we expect since the calculated results used for the extrapolation are not fully UV converged. On the other hand, for high $\hw$ the extrapolated results converge since the calculated results used for the extrapolation are UV converged. The extrapolated ground state energy at $\hw \approx 20$ MeV ($-28.3$ MeV) agrees with the calculated result at the variational minimum of the $\Nmax = 16$ curve ($-28.3$ MeV) and the experimental result ($-28.3$ MeV). On the other hand, the extrapolated proton radius at $\hw \approx 20$ MeV ($1.44$ fm) agrees with the calculated result at $\Nmax = 16$ ($1.44$ fm); however, it is about $\sim 0.02$ fm short of the experimental result [$r_{p} = 1.462(6)$ fm]. Thus, the NCCI calculation using the JISP$16$ interaction correctly predicts the binding energy of $\isotope[4]{He}$, while the prediction for the proton radius is about $\sim 1.5$ $\%$ short of the experimental result.






In Fig.~\ref{fig-chap2-helium3-helium4}, we also show the extrapolated results for the ground state energy [panel (a)] and proton radius [panel (b)] of $\isotope[3]{He}$. We observe that the calculated ground state energy converges (to the $0.01$ MeV level). The extrapolated ground state energy at $\hw \approx 20$ MeV ($-7.67$ MeV) is about $\sim 0.05$ MeV short of the experimental result ($-7.72$ MeV). The extrapolated proton radius staggers around the experimental result [$r_{p} = 1.774(6)$ fm] at the $0.1$ fm level. However, since full convergence is not achieved we cannot assess whether the calculation correctly predicts the proton radius.



\section{Using a general single-particle basis in NCCI calculations}
\label{sec-chap2-general-basis}


In this section we review the procedure followed to derive the two-body matrix elements of the NCCI Hamiltonian in a general single-particle basis. The discussion follows closely the derivations discussed in Ref.~\cite{caprio2012:csbasis} where the two-body matrix elements of the NCCI Hamiltonian with respect to the Laguerre basis were derived. 



To build the Hamiltonian matrix using a general single-particle basis we need to calculate the two-body matrix elements of the interaction and relative kinetic energy operators in the general basis. In the case where the two-body matrix elements of the interaction with respect to some single-particle basis are known, we can use a two-body transformation to obtain the two-body matrix elements with respect to the general basis. For example, the JISP$16$ interaction is expressed in terms of the harmonic oscillator basis. Therefore, we can use a two-body transformation which will yield the two-body matrix elements in the general basis. Specifically, if $a = (n_{a}l_{a}j_{a})$ is a harmonic oscillator single-particle orbital and $a' = (n_{a'} l_{a'} j_{a'})$ is a general single-particle orbital then for antisymmetrized two-body states such as (\ref{eqn-chap2-two-particle-states-2}) the transformation is given by~\cite{hagen2006:gdm-realistic}
\begin{equation}
\langle c' d'; J | V | a' b'; J \rangle_{\mathrm{AS}} = \sum_{abcd} \langle a | a' \rangle \langle b | b' \rangle \langle c | c' \rangle \langle d | d' \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{AS}},
\label{eqn-chap2-two-body-interaction-transformation}
\end{equation}
where $\langle a | a' \rangle$ is an overlap bracket. For normalized antisymmetrized states such as (\ref{eqn-chap2-two-particle-states-3}) the transformation is given by
\begin{multline}
\langle c' d'; J | V | a' b'; J \rangle_{\mathrm{NAS}} = (1+\delta_{a'b'})^{-1/2} (1+\delta_{c'd'})^{-1/2} \\  \sum_{abcd} (1+\delta_{ab})^{1/2} (1+\delta_{cd})^{1/2} \langle a | a' \rangle \langle b | b' \rangle \langle c | c' \rangle \langle d | d' \rangle \langle c d;J | V | a b; J \rangle_{\mathrm{NAS}}.
\label{eqn-chap2-two-body-interaction-transformation-nas}
\end{multline}
The overlap bracket is given by 
\begin{equation}
\langle a | a' \rangle = \langle R_{n_{a}l_{a}} | R_{n_{a'} l_{a'}} \rangle \delta_{(l_{a}j_{a})(l_{a'}j_{a'})}, 
\label{eqn-chap2-overlap-bracket}
\end{equation}
where 
\begin{equation}
\langle R_{n_{a}l_{a}} | R_{n_{a'}l_{a}} \rangle = \int_{0}^{\infty} dr R_{n_{a}l_{a}}(b_{\mathrm{HO}};r) R_{n_{a'}l_{a}}(b_{a'};r), 
\label{eqn-chap2-overlap-integral}
\end{equation}
and $b_{\mathrm{HO}}$ and $b_{a'}$ are the characteristic lengths of the harmonic oscillator basis and the general basis respectively. The transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) [or (\ref{eqn-chap2-two-body-interaction-transformation-nas})] involves an infinite quadruple sum over orbitals. The sum must be truncated, e.g., according to a one-body shell cutoff $\Ncut$ which must be selected in a way which ensures that NCCI calculations in the general basis are $\Ncut$ independent.


In principle, the two-body transformation~(\ref{eqn-chap2-two-body-interaction-transformation}) can be used to obtain the two-body matrix elements of the relative kinetic energy operator in the general basis (provided that the matrix elements in the harmonic oscillator or some other single-particle basis are known). However, in Ref.~\cite{caprio2012:csbasis} the transformation was found to yield calculated results which are highly sensitive to the $N_{\mathrm{cut}}$ truncation. Therefore, the two-body matrix elements of the relative kinetic energy operator were calculated directly in the general single-particle basis~\cite{caprio2012:csbasis}. Recall that the relative kinetic energy operator separates into one and two-body parts. Specifically, rearranging (\ref{eqn-chap2-kinetic-energy-decomposition}) we get
\begin{equation}
T_{\mathrm{rel}}  = \frac{1}{4 A m_{\mathrm{N}}} \sum_{i \neq j}^{A} (\mathbf{p}_{i}-\mathbf{p}_{j})^{2} = \frac{1}{2 A m_{\mathrm{N}}} \left[ (A-1) \sum_{i=1}^{A} p_{i}^{2} - \sum_{i \neq j}^{A} \mathbf{p}_{i} \cdot \mathbf{p}_{j} \right].
\label{eqn-chap2-kinetic-energy-decomposition-matrix-elements}
\end{equation}
The first term is a one-body operator the matrix elements of which can be calculated using the momentum space representation of the general single-particle basis. The second term is a two-body operator the matrix elements of which factorize according to Racah's reduction formula~\cite{suhonen2007:nucleons-nucleus}
\begin{equation}
\langle c'd';J | \mathbf{p}_{1} \cdot \mathbf{p}_{2} | a'b'; J \rangle = (-1)^{j_{d'}+j_{a'}+J} \Gj{j_{c'}}{j_{d'}}{J}{j_{b'}}{j_{a'}}{1} \langle c' || \mathbf{p}_{1} || a' \rangle \langle d' || \mathbf{p}_{2} || b' \rangle,
\label{eqn-chap2-kinetic-energy-two-body-matrix-elements}
\end{equation}
where $\langle c' || \mathbf{p} || a' \rangle \propto [\int_{0}^{\infty} dk \tilde{R}_{n_{c'}l_{c'}}(b;k) k \tilde{R}_{n_{a'}l_{a'}}(b;k)] \langle l_{c'} j_{c'} || Y_{1} || l_{a'} j_{a'} \rangle$, $\tilde{R}_{n'l'}(b;k)$ is the momentum space representation of the general single-particle states, and $\mathbf{p} \equiv \hbar \mathbf{k}$.













